Measurement of the top-quark production cross-section and charge asymmetry at LHCb

The first measurements of the top- and antitop-quark differential production cross-sections and the top-quark charge asymmetry in the forward region are presented, using proton-proton collision data collected by the LHCb experiment at a centre-of-mass energy of 13 TeV corresponding to an integrated luminosity of 5.4 $fb^{-1}$. The total production cross-sections of top and antitop quarks are also determined. Measurements are performed using the $\mu+b\text{-jet}$ final state within a fiducial region defined by a $b\text{-jet}$ $p_{\text{T, jet}}>50$ GeV and pseudorapidity $2.2<\eta_{\text{jet}}<4.0$,, with the muon from the $W$-boson decay required to have $p_{\text{T},\mu}>25$ GeV and pseudorapidity $2.0<\eta_{\mu}<4.5$. The muon and $b$-jet system must satisfy $p_{T}(\mu+\text{jet}) > 20$ GeV. The measured integrated production cross-sections for the top and antitop quarks are $\sigma_{t} = 0.95 \pm 0.04 \pm 0.08 \pm 0.02$ pb, $\sigma_{\bar{t}} = 0.81 \pm 0.03 \pm 0.07 \pm 0.02$ pb, where the first uncertainty is statistical, the second systematic, and the third accounts for the luminosity uncertainty. The top-quark charge asymmetry is measured to be $A_C^{t} = 0.08 \pm 0.03 \pm 0.01$, where the first uncertainty is statistical and the second is systematic. These results are consistent with next-to-leading-order Standard Model predictions.

==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	BUILDCOMMANDUPRIGHT=rm -f upright.aux && $(LATEX) upright && bibtex upright && $(LATEX) upright && $(LATEX) upright
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDUPRIGHT=rm -f upright.aux && $(LATEX) upright && bibtex upright && $(LATEX) upright && $(LATEX) upright && dvips -z -o upright.ps upright && ps2pdf upright.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib) $(wildcard *.bst)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prl.pdf

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 

# Make the upright version
upright: 
	$(BUILDCOMMANDUPRIGHT)



==> body.tex <==
% Introduction
In the Standard Model (SM), the top quark (\tquark) is the most massive fundamental particle~\cite{PDG2024}. Owing to its large Yukawa coupling, it plays a central role in electroweak symmetry breaking and in interactions of the Higgs boson. Moreover, the top quark provides a sensitive probe of physics beyond the SM, including scenarios with modified Higgs couplings or new heavy states~\cite{Kagan:2011pnt,Gauld:2013aja,Gauld:2014pxa}.  At the Large Hadron Collider (\lhc), top quarks are mainly produced in pairs with their antiquarks (\ttbar) via the strong interaction, with a smaller contribution from single-top processes mediated by the electroweak interaction~\cite{PDG2024}. In the forward region, the SM predicts that about $80\%$ of $\tquark\to Wb$ decays originate from $\ttbar$ production, with the remaining $20\%$ dominated by $t$-channel single-top production~\cite{ttbar,ST_sch,Wt}.
The top-quark production cross-section is particularly sensitive to the gluon parton distribution function (PDF), especially in the high-Bjorken-$x$ region where current constraints remain weak~\cite{gluonpdf,Alekhin:2024bhs,Ablat:2023tiy}. 
With its unique forward acceptance, the \lhcb detector can probe kinematic regimes inaccessible to \atlas and \cms experiments, providing complementary measurements. In particular, forward top production has been suggested as a probe to constrain the gluon PDF at high $x$ at the level of $20\%$~\cite{Gauld:2014pxa}. 

Within the SM, \ttbar production is intrinsically charge symmetric at leading order, and the $gg\to \ttbar$ contribution is charge symmetric to all orders. However, next-to-leading-order (NLO) quantum chromodynamics (QCD) effects, driven by quark-antiquark annihilation, induce a small asymmetry. 
These effects arise from interference between initial- and final-state radiation, as well as between the Born and box diagrams~\cite{Bernreuther:2012sx}. 
Although single-top production has a small cross-section, its intrinsic asymmetry is enhanced in proton-proton ($pp$) collisions, where the larger \uquark-quark parton density relative to \dquark quarks leads to a net positive charge asymmetry; the single-top process itself yields a charge asymmetry at the level of about $40\%$~\cite{ST_sch,Wt}.
The charge-asymmetry observable is defined as
\begin{equation}
\label{eq:asy}
\asy = \left( \frac{\sigma_t - \sigma_{\bar{t}}}{\sigma_t + \sigma_{\bar{t}}} \right)_{\eta_{\mu}},
\end{equation}
where $\sigma_t$ and $\sigma_{\bar{t}}$ respectively represent the production cross-sections of \tquark and \tquarkbar quarks in bins of muon pseudorapidity, $\mueta$, 
measured in the \lhcb laboratory frame.
At the \lhc, where gluon fusion dominates, the charge asymmetry in \ttbar production is significantly diluted. Nevertheless, in the forward region accessible to \lhcb, this dilution is reduced, enhancing sensitivity to the charge asymmetry~\cite{Gauld:2014pxa}. Theoretical predictions suggest that \lhcb may provide the first significant observation of the top-quark charge asymmetry at the \lhc~\cite{Kagan:2011pnt,Gauld:2014pxa}. 

The \ttbar and single-top production cross-sections have been extensively measured by the \atlas and \cms collaborations at center-of-mass energies of $\sqs=5.02$, 7, 8, 13, and 13.6\tev~\cite{CMS:2012hcu,CMS:2012xhh,CMS:2013yjt,ATLAS:2014sxe,CMS:2014mgj,ATLAS:2014nxi,CMS:2015auz,ATLAS:2016qhd,CMS:2016yys,CMS:2016csa,ATLAS:2017jkf,ATLAS:2017wvi,ATLAS:2017rso,CMS:2018fks,CMS:2018lgn,CMS:2019snc,ATLAS:2020ccu,CMS:2021gwv,CMS:2021vhb,ATLAS:2022aof,ATLAS:2022jbj,ATLAS:2022opp,ATLAS:2023gsl,ATLAS:2023slx,CMS:2023qyl,CMS:2024ghc}. 
At \lhcb, previous studies have so far been limited to total cross-section measurements at 7, 8, and 13\tev~\cite{LHCb-PAPER-2015-022,LHCb-PAPER-2016-038,LHCb-PAPER-2017-050}.
Measurements of $\asy$ were first performed at the \tevatron by the \cdf and \dzero experiments~\cite{CDF:2011xdt,D0:2015alu,CDF:2012ctl}, where initial tensions with theoretical predictions were later reduced by improved calculations and updated measurements~\cite{Czakon:2014xsa,D0:2014cda,Kidonakis:2015ona,CDF:2017cvy}. At the \lhc, results from \atlas~\cite{ATLAS:2013buu,ATLAS:2015ysm,ATLAS:2015jgj,ATLAS:2015sex,ATLAS:2022wec,ATLAS:2022waa} and \cms~\cite{CMS:2012oht,CMS:2014rdf,CMS:2015fvy,CMS:2015pob,CMS:2016ypc} collaborations have achieved increasing precision.
While the most recent ATLAS measurement~\cite{ATLAS:2022waa} reports a 4.7$\sigma$ deviation from zero, the extracted asymmetry remains numerically small and consistent with the SM.


This Letter presents the first measurements of the differential production cross-sections of the \tquark and \tquarkbar quarks as a function of the muon pseudorapidity in the forward region, the corresponding $\asy$ observable, and the integrated production cross-sections.
The measurement is performed in the \decay{t}{W^{+}(\to\mu^{+}\nu_{\mu})\, b} decay channel,\footnote{Charge-conjugate states are implied throughout this Letter.} using $pp$ collision data collected with the \lhcb detector at $\sqs=13\tev$, corresponding to an integrated luminosity of 5.4\invfb.
The measurement is performed in the fiducial phase space defined by the presence of a muon with transverse momentum (defined with respect to the beam axis) $\mupt>25\gev$ in the pseudorapidity range $2.0<\mueta<4.5$.\footnote{Natural units with $\hbar = c = 1$ are used throughout.}
Jets are reconstructed using the anti-$k_\textrm{T}$ algorithm~\cite{antiKt} with radius parameter $R=0.5$, and are required to satisfy $\jetpt>50\gev$ and $2.2 < \jeteta < 4.0$. The inputs to the jet‑clustering algorithm are charged and neutral particles, which are obtained by combining information from all detector subsystems through a particle-flow approach~\cite{LHCb-PAPER-2013-058}.

%  top xsec determination
The top charge asymmetry, $\asy$, is measured via Eq.~\ref{eq:asy}, while the differential cross-section for each charge of the final-state muon and each bin in $\eta_{\mu}$ is determined as
\begin{equation}
\label{eq:xsec}
\frac{d\sigma_{t}^{}}{d\eta_{\mu}} = 
\frac{\left( N - N_{\text{bkg}} \right) \cdot \mathcal{A} \cdot P}
{\Delta \eta_{\mu} \cdot \lum \cdot \varepsilon_{\text{sel}} \cdot \varepsilon_{\text{rec}} \cdot \varepsilon_{\text{btag}} \cdot \epsilon_{\text{true}} }, 
\end{equation}
where $N$ is the total number of selected candidates, $N_{\text{bkg}}$ is the estimated background contribution, and $\Delta \eta_{\mu}$ is the width of the bin in $\eta_{\mu}$. The integrated luminosity is denoted by \lum, and the  reconstruction, selection, and \bquark-tagging efficiencies are represented by $\varepsilon_{\text{rec}}$, $\varepsilon_{\text{sel}}$, and $\varepsilon_{\text{btag}}$, respectively. The acceptance factor, $\mathcal{A}$, accounts for migrations into and out of the fiducial region, including non-negligible contributions from the $\decay{t}{W^+(\to\tau^+\nu_{\tau})\, b}$ decay mode. The jet reconstruction purity, $P$, is defined as the fraction of reconstructed jets within the fiducial region that originate from truth-level jets also contained in the same region.  
The term $\epsilon_{\text{true}}$ denotes the truth-level jet reconstruction efficiency, defined as the fraction of truth-level jets within the fiducial region that are successfully reconstructed in the same region.  

%% LHCb detector 
The \lhcb detector~\cite{LHCb-DP-2008-001,LHCb-DP-2014-002} is a single-arm forward spectrometer covering $2<\eta <5$, designed for the study of particles containing \bquark or \cquark quarks. 
The detector used to collect data for this analysis includes a high-precision tracking system consisting of a silicon-strip vertex detector surrounding the $pp$ interaction region~\cite{LHCb-DP-2014-001}, a large-area silicon-strip detector located upstream of a dipole magnet with a bending power of about $4{\mathrm{\,T\,m}}$, and three stations of silicon-strip detectors and straw drift tubes~\cite{LHCb-DP-2017-001} placed downstream of the magnet.
The tracking system provides a measurement of the momentum, \ptot, of charged particles with a relative uncertainty that varies from 0.5\% at low momentum to 1.0\% at 200\gev. The minimum distance of a track to a primary $pp$ collision vertex (PV), the impact parameter (IP), is measured with a resolution of $(15+29/\pt)\mum$, where \pt is measured in\,\gev.
Different types of charged hadrons are distinguished using information from two ring-imaging Cherenkov detectors~\cite{LHCb-DP-2012-003}. 
Photons, electrons and hadrons are identified by a calorimeter system consisting of scintillating-pad and preshower detectors, an electromagnetic and a hadronic calorimeter.
Muons are identified by a system composed of alternating layers of iron and multiwire proportional chambers~\cite{LHCb-DP-2012-002}.
Approximately half of the data were collected with the magnet in each of the two polarity configurations. The online event selection is performed by a trigger system~\cite{LHCb-DP-2012-004,LHCb-DP-2019-001}. This analysis uses events selected by trigger algorithms that require at least one identified muon with high \pt.

Simulation samples are generated using \pythia~\cite{Sjostrand:2007gs,*Sjostrand:2006za} with a specific \lhcb configuration~\cite{LHCb-PROC-2010-056}. Final-state radiation is simulated with \photos~\cite{davidson2015photos}. The interaction of the generated particles with the detector, and its response, are modeled using the \geant toolkit~\cite{Allison:2006ve, *Agostinelli:2002hh} as described in Ref.~\cite{LHCb-PROC-2011-006}. 
Auxiliary signal samples without detector simulation are produced using the ‌\powheg-BOX framework~\cite{Nason:2004rx,Frixione:2007vw,Alioli:2010xd} at NLO, and interfaced with \pythia for parton showering and hadronization.
Alternative NLO predictions produced with the {\sc MadGraph}~\cite{Mg5} framework are employed for cross-checks. 



Candidate \decay{t}{W^{+}(\to\mu^{+}\nu_{\mu})\, b} decays are formed from a well-separated muon-jet pair with $\Delta R(\mu, \jet) > 0.5$, where $\Delta R \equiv \sqrt{(\Delta \eta)^2 + (\Delta \phi)^2}$, and $\Delta \eta$ ($\Delta \phi$) is the difference in pseudorapidity (azimuthal angle) between the muon and the jet axis. 
To suppress semileptonic heavy-flavor backgrounds, the muon IP is required to be less than 0.04\mm~\cite{LHCb-PAPER-2016-011}. 
Hadrons misidentified as muons are suppressed by requiring the energy deposit in the electromagnetic $(E_{\rm{ECAL}})$ and hadronic $(E_{\rm{HCAL}})$ calorimeters to be small, $(E_{\rm ECAL}+E_{\rm HCAL})/p < 4\%$, where $p$ is the muon momentum.
The relative momentum uncertainty of the muon track, $\sigma_{p}/p$, is required to be less than 10\%.
Events containing a second, oppositely charged, high-\pt muon with $M(\mu^{+}\mu^{-})>40\gev$ are rejected to suppress $\Z/\gamma^{*}(\to\mu^+\mu^-)+\jet$ contamination.


The jet flavor is identified using a dedicated deep neural network (DNN) classifier, inspired by the DeepJet algorithm~\cite{deepjet}, and trained using simulated \bquark-, \cquark-, and light-flavor jet samples~\cite{LHCb-PAPER-2025-034}. The network uses more than 400 input features related to jet properties, including those associated with charged and neutral jet constituents, secondary vertex variables, and global features. 
The classifier's outputs are three probabilities, $P_b$, $P_c$, and $P_q$, which sum to unity and represent the likelihood of a jet originating from a $\bquark$-, $\cquark$-, or light-flavor parton, respectively.
To suppress contamination from \cquark-jets and light-flavor jets while maximizing the \bquark-jet signal significance, the optimal selection thresholds on the DNN outputs are determined by maximizing the expected signal significance, $S = N_\text{sim}/\sqrt{N_\text{data}}$, where $N_\text{sim}$ and $N_\text{data}$ denote the expected number of simulated top signal and data candidates passing the selection, respectively. 
The simulated yields are normalized using the theoretical predictions for the production cross-section and integrated luminosity.
The working point is chosen as $P_b > 0.65$ and $P_q < 0.05$.
Despite the tight $P_b$ requirement, residual contamination from misidentified \cquark-jets and light-flavor jets remains. To account for this, a template fit to the $P_b$ distribution in data is performed to extract the \bquark-jet fraction, using simulated templates for each jet flavor. The fit yields a \bquark-jet purity of approximately 74\%, which is applied as a bin-by-bin weight in $\eta_\mu$ to remove the contributions from \cquark-jets and light-flavor jets.

One of the dominant background contributions in this analysis arises from QCD multijet production, particularly from heavy-flavor decays or in-flight hadron decays producing high-\pt muons.  
In signal events such as \decay{t}{W^{+}(\to\mu^{+}\nu_{\mu})\, b}, the undetected neutrino carries a significant fraction of the \W-boson \pt, 
resulting in a strong momentum imbalance between the muon and the accompanying jet.  
In contrast, QCD events usually have the muon produced inside or near a jet, 
leading to a more balanced configuration where the muon and jet \pt are similar and the muon is less isolated. 
To suppress this background, candidates are required to satisfy two further kinematic criteria. 
First, the \pt of the $\mu + \bquark$-jet system, $\pttot = p_{\mathrm{T}}(j + j_{\mu})$, must be greater than 20\gev, where $j$ denotes the reconstructed jet and $j_{\mu}$ denotes the jet which contains the muon.  
Secondly, the muon isolation, defined as $\imu = \mupt /p_{\mathrm{T,}\, j_{\mu}}$, must exceed 0.9.
The residual QCD background is estimated using a data-driven \texttt{ABCD} method~\cite{ABCD_ATLAS} in the ($\pttot$, $\imu$) plane. In this analysis, the \texttt{ABCD} regions are defined as: region \texttt{A} with $\pttot < 15\gev$ and $\imu < 0.9$; region \texttt{B} with $\pttot < 15\gev$ and $\imu > 0.9$; region \texttt{C} with $\pttot > 20\gev$ and $\imu < 0.9$; and region \texttt{D} (the signal region) with $\pttot > 20\gev$ and $\imu > 0.9$, containing 2278 $\mu^+$+\bjet and 1799 $\mu^-$+\bjet events.
The estimated signal yield in region \texttt{D}, $N_{D}^{\text{sig}}$, is calculated using the generalized \texttt{ABCD} relation.

Electroweak backgrounds are also considered. The \Z + \bjet background contribution is estimated using $Z(\to \mumu)+ b$-jet data candidates together with an acceptance correction factor, taken from the ratio of yields in simulation. 
Here, the $Z(\to \mumu) + \bjet$ category corresponds to partially reconstructed $Z(\to \mumu) + \bjet$ decays where one muon falls outside the geometrical acceptance of the \lhcb detector.
This correction is applied in bins of $\eta_{\mu}$ and separately for each muon charge. After subtracting the QCD and $\Z+ \jet$ backgrounds, the yield of the remaining $\W+\bjet$ background contribution is estimated. The relative normalization between $\W+\bjet$ and $\W+\jet$ events is taken from the \powheg prediction and cross-checked with {\sc MadGraph}, with corrections for the \bquark-tagging efficiency applied to match the observed yields.

%% corrections
After background subtraction, the observed signal yields of 1458 (\tquark) and 1231 (\tquarkbar) are corrected for detector and selection effects. These include the muon reconstruction efficiency, the efficiency of the muon selection criteria, the jet reconstruction efficiency, the \bquark-tagging efficiency and mistag rates, possible bin-to-bin migrations due to the detector resolution, and finally the acceptance difference between the fiducial and signal definitions and a small contamination from $W$ bosons that decay via a $\tau$ lepton subsequently producing a muon. The muon reconstruction efficiency, encompassing track reconstruction, identification, and trigger requirements, is estimated with a tag-and-probe method using \Zmm data, following the procedures used in published \W- and \Z-boson cross-section measurements at \lhcb~\cite{LHCB-PAPER-2021-037,LHCB-PAPER-2014-033,LHCB-PAPER-2015-001,LHCB-PAPER-2015-049}. The muon reconstruction efficiency varies across the muon pseudorapidity region, ranging from 64\% to 77\%. The selection efficiencies are evaluated using simulated \ttbar and single-top samples, and vary across the muon pseudorapidity region, ranging from 68\% to 75\%.
The jet reconstruction efficiency is determined from simulated $\Z(\to\mu^+\mu^-)+\jet$ samples, and is found to be about 96\%. The \bquark-tagging efficiency, based on DNN discriminators, is evaluated using simulated \ttbar and single-top samples, and corrected with a data-driven tag-and-probe method in a dijet sample enriched in $b$-jets. The number of $b$-jets before applying the DNN requirement is determined from a fit to the $P_b$ template distribution. After the DNN selection, the mistag fraction, arising from $c$- and light-flavor jets, is subtracted to obtain the final $b$-jets yield. The mistag probability is evaluated as the fraction of simulated $c$-jets and light-flavor jets passing the same DNN selection under the same tag-and-probe conditions~\cite{LHCb-PAPER-2025-034}. 
After applying weights based on the ratio of data to simulation, found to vary between 0.94 and 1.04, the resulting \bquark-tagging efficiency is approximately 56\%. 

% detector resolution effects
To account for detector-resolution effects, migration corrections for events with a reconstructed jet inside the fiducial region while the truth-level jet is outside, or vice versa, are evaluated with simulations.
The corrections from these effects are below 1\%. Bin-to-bin migrations in $\eta_\mu$ are found to be negligible, owing to the excellent resolution. 

Beyond detector-resolution effects, differences between the definitions of the fiducial region and of the signal region \texttt{D} (in the \texttt{ABCD} method) are taken into account. In the fiducial region, the \pt requirement is applied to the vector sum of the muon and the \bjet, while in the signal region it is applied to the muon-containing jet combined with the \bjet. This mismatch is corrected by using an acceptance factor defined as $\mathcal{A}_{j_{\mu}} =\frac{N\left( p_{\mathrm{T}}(\mu + j) > 20\,\gev \right)}{N\left( p_{\mathrm{T}}(j_{\mu} + j) > 20\,\gev \right)}$, which is evaluated from simulated top-quark events.
The data sample includes background contributions from muons originating in intermediate $\tau$ decays, in addition to those produced directly in \decay{W}{\mu\nu} decays. To ensure that the reported cross-sections correspond exclusively to prompt muons from \W decays, a correction factor, defined as the fraction of such muons relative to the total, is derived from simulation and applied to the yields measured in data. 
The effect of the acceptance factor is found to be below 2\%.


%% uncertainties 
The sources of systematic uncertainties considered in the cross-section measurements are summarized in Table~\ref{tab:uncertainty}. 
The dominant contribution arises from \bquark-jet tagging, which comprises uncertainties from both the mistag fraction and the \bquark-tagging efficiency. These are affected by common factors such as the choice of the parton-shower model (comparing {\sc MadGraph} interfaced with \pythia and with {\sc Herwig}, with kinematic weighting applied), variations in the simulated flavor composition (achieved by altering the fractions of light-flavor and \cquark-jets in the fit), and the jet energy scale and resolution effects (evaluated through smearing and scaling). For the mistag fraction, an additional contribution arises from the statistical precision of the template fits. For the \bquark-tagging efficiency, the dominant statistical contribution comes from data-driven corrections, including the template fits and the weights based on the ratio of data to simulation.
The second-largest systematic uncertainty originates from the jet energy scale and resolution. The efficiency of the $\jetpt > 50\gev$ requirement is evaluated in simulation. A control sample of $Z+\jet$ events is used to assess the energy scale and resolution as done in Ref.~\cite{LHCb-PAPER-2020-018}, which are then propagated to the top-quark simulation to evaluate the impact.

\begin{table}
\begin{center}
\caption{Relative systematic uncertainties in the \tquark and \tquarkbar total cross-section measurements, in percent. The total uncertainties are obtained by summing in quadrature the statistical, total systematic, and luminosity components.}
\begin{tabular}{l|c|c}
\hline
 Source               & $\Delta\sigma_{\tquark}/\sigma_{\tquark}$ [\%]  & $\Delta\sigma_{\tquarkbar}/\sigma_{\tquarkbar}$ [\%] \\
\hline
\textit{b}-jet tagging & 6.5 & 6.2 \\
Jet energy scale and resolution & 5.0 & 5.0 \\ 
\texttt{ABCD} method  & 2.0 & 2.1 \\ 
$\Z+\bjet$ background & 0.2 & 0.2 \\ 
$\W+\bjet$ background & 0.9 & 1.3 \\ 
Selection efficiency & 0.2 & 0.2 \\ 
Muon reconstruction efficiency & 0.2 & 0.2 \\ 
Jet reconstruction efficiency & 0.3 & 0.3 \\ 
\hline
Total systematic (excl. lumi.) & 8.5 & 8.3 \\ 
Luminosity   & 2.0 & 2.0 \\ 
Statistical & 3.8 & 4.0 \\ 
Total  & 9.5 & 9.4 \\  \hline
\end{tabular}
\label{tab:uncertainty}
\end{center}
\end{table}

The uncertainty associated with the \texttt{ABCD} background estimation method receives contributions from several effects. The method assumes that the two discriminating variables are uncorrelated. To reduce possible correlations, the ratio $N_{C}/N_{A}$ in the region $\imu<0.9$ is calculated as a function of $\pt^{j_{\mu}}$, and used to weight both the \texttt{A} and \texttt{B} samples following the strategy of Ref.~\cite{LHCb-PAPER-2015-021}. The impact of this weighting is quantified by assessing the signal yield variations, with the difference assigned as the corresponding systematic uncertainty.
In addition, the impact of the uncertainties on the correction coefficients is evaluated by varying each coefficient independently by $\pm10\%$. The resulting variation in the extracted signal yield is taken as its systematic uncertainty.

The systematic uncertainty on the $\Z+\bjet$ background arises from the statistical uncertainty of the acceptance correction factor.
The uncertainty of the $\W+\bjet$ background originates from uncertainties in the theoretical prediction of the NLO cross-section ratio $\sigma(\W+\bjet)/\sigma(\W +\jet)$.
The effect of PDF uncertainties is determined using the technique of Monte Carlo PDF replicas, while the scale uncertainty is obtained from the envelope of variations where both the factorization and renormalization scales are independently varied up and down by a factor of two, as well as from the variation of the strong-coupling constant $\alpha_s$~\cite{theoryerr}.

Muon reconstruction uncertainties are derived from data-driven efficiency measurements using \Zmm events and applied to the simulated \tquark-quark samples. 
The jet reconstruction uncertainty is similarly evaluated using $\Z(\to\mu^{+}\mu^{-})+\jet$ control samples. The uncertainty from the selection efficiency accounts for the limited size of the simulated \tquark-quark samples. A 2\% uncertainty is assigned to the integrated luminosity, as determined in Ref.~\cite{lumi}.
The results obtained separately for the two magnet polarities are compatible within statistical uncertainties, and no additional systematic uncertainty is assigned.

The integrated production cross-sections for \tquark and \tquarkbar are measured using Eq.~\ref{eq:xsec} to be
\begin{equation*}
\begin{split}
 \sigma_{\tquark} = \xs \pm \xsstat  \stat \pm \xssyst \syst \pm \xslumi \ (\rm{lumi})  \pb, \\
 \sigma_{\tquarkbar} = \tbarxs \pm \tbarxsstat \stat \pm \tbarxssyst \syst \pm \tbarxslumi \ (\rm{lumi})  \pb,
 \end{split}
\end{equation*}
where the quoted uncertainties are statistical, systematic, and from the luminosity determination, respectively. The systematic uncertainties of the \tquark and \tquarkbar cross-sections are correlated at the level of 96\%. 
The inclusive charge asymmetry is measured as
\begin{equation*}
 \asy = \ay \pm \aystat \stat \pm \aysyst \syst.
\end{equation*}

Differential cross-sections and charge asymmetries as a function of $\eta_\mu$ are shown in Figs.~\ref{fig:xsec} and \ref{fig:asy}, and summarized in Tables~\ref{tab:xsec_table} and \ref{tab:asymmetry_table}.
The measurements are compared with NLO predictions from \powheg-BOX~\cite{POWHEG} using CT18~\cite{Hou:2019efy} and NNPDF31~\cite{Ball2017} PDFs and {\sc MadGraph}~\cite{Mg5} using NNPDF31, and good agreement is observed.
Theoretical uncertainties contain the PDF, scale, and $\alpha_s$ uncertainties~\cite{bourilkov2006}. 

% summary
In summary, the first measurement of the top-quark charge asymmetry and the differential \tquark- and \tquarkbar-quark production cross-sections in the forward region is presented, using $pp$ collisions collected with the \lhcb detector between 2015 and 2018 at $\sqs=13\tev$, corresponding to an integrated luminosity of 5.4\invfb.
The results represent the most precise top-quark production cross-section measurements in the forward region to date.

For the charge asymmetry measurement, the $\mu+\bjet$ final state receives contributions from both $\ttbar$ and single-top production. In future analyses with larger data sets, the measured asymmetry should be decomposed through a fit incorporating the expected asymmetries from both processes. 

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.49\linewidth]{figs/xsec_mup_adjusted_bins.pdf}
    \includegraphics[width=0.49\linewidth]{figs/xsec_mum_adjusted_bins.pdf}
    \caption{Differential cross-sections for the (left) \tquark and (right) \tquarkbar production as a function of the muon pseudorapidity compared with theoretical predictions at NLO.}
    \label{fig:xsec}
\end{figure}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.49\linewidth]{figs/asy.pdf}
    \caption{Measured \tquark-quark charge asymmetry as a function of the muon pseudorapidity compared with theoretical predictions at NLO.}
    \label{fig:asy}
\end{figure}

\begin{table}[!htbp]
    \centering
    \caption{Measured \tquark- and \tquarkbar-quark differential cross-sections as a function of $\eta_{\mu}$. Uncertainties are statistical, systematic, and from the luminosity, respectively.}
\begin{tabular}{ccc}
    \toprule
    $\eta_{\mu}$ interval & $\sigma_{\tquark}$ (pb) & $\sigma_{\tquarkbar}$ (pb) \\
    \midrule
    2.000--2.625 & $0.722 \pm 0.040 \pm 0.063 \pm 0.014$ & $0.653 \pm 0.035 \pm 0.055 \pm 0.013$ \\
    2.625--3.250 & $0.507 \pm 0.033 \pm 0.043 \pm 0.010$ & $0.437 \pm 0.030 \pm 0.037 \pm 0.009$ \\
    3.250--3.875 & $0.234 \pm 0.022 \pm 0.019 \pm 0.005$ & $0.173 \pm 0.020 \pm 0.016 \pm 0.003$ \\
    3.875--4.500 & $0.061 \pm 0.014 \pm 0.008 \pm 0.001$ & $0.044 \pm 0.012 \pm 0.007 \pm 0.001$ \\

    \bottomrule
\end{tabular}
    \label{tab:xsec_table}
\end{table}

\begin{table}[!htbp]
    \centering
    \caption{Measured \tquark-quark charge asymmetry as a function of $\eta_{\mu}$. Uncertainties are statistical and systematic, respectively. The significance quantifies the deviation from zero.}
\begin{tabular}{cccc}
    \toprule
    $\eta_{\mu}$ range & $\asy$ & significance  \\
    \midrule

    2.000--2.625 & $0.05 \pm 0.04 \pm 0.02$ & $1.22$ \\
    2.625--3.250 & $0.07 \pm 0.05 \pm 0.02$ & $1.44$ \\
    3.250--3.875 & $0.15 \pm 0.07 \pm 0.03$ & $1.91$ \\
    3.875--4.500 & $0.17 \pm 0.18 \pm 0.09$ & $0.85$ \\ \hline

    2.0--4.5\;\;(\text{combined}) 
      & $\ay \pm \aystat \pm \aysyst$ 
      & \TotalAsySigma \\

    \bottomrule
\end{tabular}
    \label{tab:asymmetry_table}
\end{table}



==> lhcb_text/Authorship_LHCb-PAPER-2025-057-arXiv.tex <==
LHCb collaboration:
R. Aaij,
A.S.W. Abdelmotteleb,
C. Abellan Beteta,
F. Abudin{\'e}n,
T. Ackernley,
A. A.  Adefisoye,
B. Adeva,
M. Adinolfi,
P. Adlarson,
C. Agapopoulou,
C.A. Aidala,
Z. Ajaltouni,
S. Akar,
K. Akiba,
M.  Akthar,
P. Albicocco,
J. Albrecht,
R.  Aleksiejunas,
F. Alessio,
P. Alvarez Cartelle,
R. Amalric,
S. Amato,
J.L. Amey,
Y. Amhis,
L. An,
L. Anderlini,
M. Andersson,
P. Andreola,
M. Andreotti,
S.  Andres Estrada,
A. Anelli,
D. Ao,
C. Arata,
F. Archilli,
Z. Areg,
M. Argenton,
S. Arguedas Cuendis,
L.  Arnone,
A. Artamonov,
M. Artuso,
E. Aslanides,
R. Ata\'{i}de Da Silva,
M. Atzeni,
B. Audurier,
J. A.  Authier,
D. Bacher,
I. Bachiller Perea,
S. Bachmann,
M. Bachmayer,
J.J. Back,
P. Baladron Rodriguez,
V. Balagura,
A.  Balboni,
W. Baldini,
Z. Baldwin,
L. Balzani,
H.  Bao,
J. Baptista de Souza Leite,
C. Barbero Pretel,
M. Barbetti,
I. R. Barbosa,
R.J. Barlow,
M. Barnyakov,
S. Barsuk,
W. Barter,
J. Bartz,
S. Bashir,
B. Batsukh,
P. B.  Battista,
A.  Bavarchee,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I.B. Bediaga,
N. A.  Behling,
S. Belin,
A.  Bellavista,
K. Belous,
I. Belov,
I. Belyaev,
G. Benane,
G. Bencivenni,
E. Ben-Haim,
A. Berezhnoy,
R. Bernet,
S. Bernet Andres,
A. Bertolin,
F. Betti,
J.  Bex,
O. Bezshyyko,
S.  Bhattacharya,
M.S. Bieker,
N.V. Biesuz,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
T. Blake,
F. Blanc,
J.E. Blank,
S. Blusk,
V. Bocharnikov,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A.  Bohare,
A. Boldyrev,
C. Bolognani,
R. Bolzonella,
R. B.  Bonacci,
N. Bondar,
A. Bordelius,
F. Borgato,
S. Borghi,
M. Borsato,
J.T. Borsuk,
E.  Bottalico,
S.A. Bouchiba,
M.  Bovill,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
J. D. Brandenburg,
A. Brea Rodriguez,
N. Breer,
J. Brodzicka,
J. Brown,
D. Brundu,
E. Buchanan,
M.  Burgos Marcos,
C. Burr,
C.  Buti,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
Y.  Cai,
A. Caillet,
R. Calabrese,
L. Calefice,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
J. I. Cambon Bouzas,
P. Campana,
A. C. Campos,
A.F. Campoverde Quezada,
S. Capelli,
M.  Caporale,
L. Capriotti,
R. Caravaca-Mora,
A. Carbone,
L. Carcedo Salgado,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carus,
A. Casais Vidal,
R. Caspary,
G. Casse,
M. Cattaneo,
G. Cavallero,
V. Cavallini,
S. Celani,
I.  Celestino,
S.  Cesare,
A.J. Chadwick,
I. Chahrour,
H.  Chang,
M. Charles,
Ph. Charpentier,
E.  Chatzianagnostou,
R.  Cheaib,
M. Chefdeville,
C. Chen,
J.  Chen,
S. Chen,
Z. Chen,
A.  Chen Hu,
M.  Cherif,
A. Chernov,
S. Chernyshenko,
X.  Chiotopoulos,
V. Chobanova,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
X. Cid Vidal,
G. Ciezarek,
P. Cifra,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
C. Cocha Toapaxi,
V. Coco,
J. Cogan,
E. Cogneras,
L. Cojocariu,
S.  Collaviti,
P. Collins,
T. Colombo,
M. Colonna,
A. Comerma-Montells,
L. Congedo,
J.  Connaughton,
A. Contu,
N. Cooke,
G. Cordova,
C.  Coronel,
I. Corredoira ,
A. Correia,
G. Corti,
J. Cottee Meldrum,
B. Couturier,
D.C. Craik,
M. Cruz Torres,
M.  Cubero Campos,
E. Curras Rivera,
R. Currie,
C.L. Da Silva,
S. Dadabaev,
X. Dai,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
J. Daniel,
G. Darze,
A.  Davidson,
J.E. Davies,
O. De Aguiar Francisco,
C. De Angelis,
F. De Benedetti,
J. de Boer,
K. De Bruyn,
S. De Capua,
M. De Cian,
U. De Freitas Carneiro Da Graca,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
F. De Vellis,
J.A. de Vries,
F. Debernardis,
D. Decamp,
S.  Dekkers,
L. Del Buono,
B. Delaney,
J. Deng,
V. Denysenko,
O. Deschamps,
F. Dettori,
B. Dey,
P. Di Nezza,
I. Diachkov,
S. Didenko,
S. Ding,
Y.  Ding,
L. Dittmann,
V. Dobishuk,
A. D.  Docheva,
A.  Doheny,
C. Dong,
F. Dordei,
A.C. dos Reis,
A. D.  Dowling,
L. Dreyfus,
W. Duan,
P. Duda,
L. Dufour,
V. Duk,
P. Durante,
M. M. Duras,
J.M. Durham,
O. D.  Durmus,
A. Dziurda,
A. Dzyuba,
S. Easo,
E. Eckstein,
U. Egede,
A. Egorychev,
V. Egorychev,
S. Eisenhardt,
E. Ejopu,
L. Eklund,
M. Elashri,
D.  Elizondo Blanco,
J. Ellbracht,
S. Ely,
A. Ene,
J. Eschle,
T. Evans,
F. Fabiano,
S.  Faghih,
L.N. Falcao,
B. Fang,
R. Fantechi,
L. Fantini,
M. Faria,
K.   Farmer,
F.  Fassin,
D. Fazzini,
L. Felkowski,
M. Feng,
A. Fernandez Casani,
M. Fernandez Gomez,
A.D. Fernez,
F. Ferrari,
F. Ferreira Rodrigues,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
K.L. Fischer,
D.S. Fitzgerald,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
A.  Fomin,
M. Fontana,
L. A.  Foreman,
R. Forty,
D. Foulds-Holt,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Q. F{\"u}hring,
T. Fulghesu,
G. Galati,
M.D. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
M. Gandelman,
P. Gandini,
B.  Ganie,
H. Gao,
R. Gao,
T.Q. Gao,
Y. Gao,
Y. Gao,
Y. Gao,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc{\'\i}a Pardi{\~n}as,
P.  Gardner,
L. Garrido,
C. Gaspar,
A.  Gavrikov,
L.L. Gerken,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
S. Ghizzo,
Z. Ghorbanimoghaddam,
F. I. Giasemis,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent{\`u},
L. Girardey,
M.A. Giza,
F.C. Glaser,
V.V. Gligorov,
C. G{\"o}bel,
L.  Golinka-Bezshyyko,
E. Golobardes,
D. Golubkov,
A. Golutvin,
S. Gomez Fernandez,
W.  Gomulka,
I. Gonçales Vaz,
F. Goncalves Abrantes,
M. Goncerz,
G. Gong,
J. A. Gooding,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
L. Grazette,
G. Graziani,
A. T. Grecu,
N.A. Grieser,
L. Grillo,
S. Gromov,
C.  Gu,
M. Guarise,
L.  Guerry,
A.-K. Guseinov,
E. Gushchin,
Y. Guz,
T. Gys,
K. Habermann,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
S.  Haken,
G.  Hallett,
P.M. Hamilton,
J. Hammerich,
Q. Han,
X. Han,
S. Hansmann-Menzemer,
L. Hao,
N. Harnew,
T. H.  Harris,
M. Hartmann,
S. Hashmi,
J. He,
N.  Heatley,
A.  Hedes,
F. Hemmer,
C. Henderson,
R. Henderson,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Herd,
P. Herrero Gascon,
J. Heuel,
A.  Heyn,
A. Hicheur,
G. Hijano Mendizabal,
J. Horswill,
R. Hou,
Y. Hou,
D.C. Houston,
N. Howarth,
W. Hu,
X. Hu,
W. Hulsbergen,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
M. Idzik,
D. Ilin,
P. Ilten,
A. Iniukhin,
A.  Iohner,
A. Ishteev,
K. Ivshin,
H. Jage,
S.J. Jaimes Elles,
S. Jakobsen,
T. Jakoubek,
E. Jans,
B.K. Jashal,
A. Jawahery,
C.  Jayaweera,
A.  Jelavic,
V. Jevtic,
Z.  Jia,
E. Jiang,
X. Jiang,
Y. Jiang,
Y. J.  Jiang,
E. Jimenez Moya,
N.  Jindal,
M. John,
A.  John Rubesh Rajan,
D. Johnson,
C.R. Jones,
S. Joshi,
B. Jost,
J.  Juan Castella,
N. Jurik,
I. Juszczak,
K.  Kalecinska,
D. Kaminaris,
S. Kandybei,
M.  Kane,
Y. Kang,
C. Kar,
M. Karacson,
A. Kauniskangas,
J.W. Kautz,
M.K. Kazanecki,
F. Keizer,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
G. Khreich,
F.  Kiraz,
T. Kirn,
V.S. Kirsebom,
S. Klaver,
N. Kleijne,
A. Kleimenova,
D. K.  Klekots,
K. Klimaszewski,
M.R. Kmiec,
T.  Knospe,
R.  Kolb,
S. Koliiev,
L. Kolk,
A. Konoplyannikov,
P. Kopciewicz,
P. Koppenburg,
A.  Korchin,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
E.  Kowalczyk,
A. Kozachuk,
P. Kravchenko,
L. Kravchuk,
O.  Kravcov,
M. Kreps,
P. Krokovny,
W. Krupa,
W. Krzemien,
O. Kshyvanskyi,
S. Kubis,
M. Kucharczyk,
V. Kudryavtsev,
E. Kulikova,
A. Kupsc,
V. Kushnir,
B. Kutsenko,
J. Kvapil,
I.  Kyryllin,
D. Lacarrere,
P.  Laguarta Gonzalez,
A. Lai,
A. Lampis,
D. Lancierini,
C. Landesa Gomez,
J.J. Lane,
G. Lanfranchi,
C. Langenbruch,
J. Langer,
T. Latham,
F. Lazzari,
C. Lazzeroni,
R. Le Gac,
H.  Lee,
R. Lef{\`e}vre,
A. Leflat,
S. Legotin,
M. Lehuraux,
E. Lemos Cid,
O. Leroy,
T. Lesiak,
E. D. Lesser,
B. Leverington,
A. Li,
C.  Li,
C.  Li,
H. Li,
J. Li,
K. Li,
L. Li,
P. Li,
P.-R. Li,
Q.  Li,
T. Li,
T. Li,
Y. Li,
Y. Li,
Y.  Li,
Z. Lian,
Q.  Liang,
X. Liang,
Z.  Liang,
S. Libralon,
A.  Lightbody,
C. Lin,
T. Lin,
R. Lindner,
H.  Linton,
R. Litvinov,
D. Liu,
F. L.  Liu,
G. Liu,
K. Liu,
S. Liu,
W.  Liu,
Y. Liu,
Y. Liu,
Y. L.  Liu,
G. Loachamin Ordonez,
I.  Lobo,
A. Lobo Salvia,
A. Loi,
T. Long,
F. C. L. Lopes,
J.H. Lopes,
A. Lopez Huertas,
C.  Lopez Iribarnegaray,
S. L{\'o}pez Soli{\~n}o,
Q. Lu,
C. Lucarelli,
D. Lucchesi,
M. Lucio Martinez,
Y. Luo,
A. Lupato,
E. Luppi,
K. Lynch,
X.-R. Lyu,
G. M.  Ma,
H.  Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
B.  Mack,
I. Mackay,
L. M.  Mackey,
L.R. Madhan Mohan,
M. J.  Madurai,
D. Magdalinski,
D. Maisuzenko,
J.J. Malczewski,
S. Malde,
L. Malentacca,
A. Malinin,
T. Maltsev,
G. Manca,
G. Mancinelli,
C. Mancuso,
R. Manera Escalero,
F. M.  Manganella,
D. Manuzzi,
D. Marangotto,
J.F. Marchand,
R. Marchevski,
U. Marconi,
E. Mariani,
S. Mariani,
C. Marin Benito,
J. Marks,
A.M. Marshall,
L.  Martel,
G. Martelli,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D.  Martinez Gomez,
D. Martinez Santos,
F. Martinez Vidal,
A.  Martorell i Granollers,
A. Massafferri,
R. Matev,
A. Mathad,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
J. Mauricio,
P. Mayencourt,
J. Mazorra de Cos,
M. Mazurek,
D.  Mazzanti Tarancon,
M. McCann,
N.T. McHugh,
A. McNab,
R. McNulty,
B. Meadows,
D. Melnychuk,
D. Mendoza Granada,
P.  Menendez Valdes Perez,
F. M.  Meng,
M. Merk,
A. Merli,
L. Meyer Garcia,
D. Miao,
H. Miao,
M. Mikhasenko,
D.A. Milanes,
A. Minotti,
E. Minucci,
T. Miralles,
B. Mitreska,
D.S. Mitzel,
R.  Mocanu,
A. Modak,
L. Moeser,
R.D. Moise,
E. F. Molina Cardenas,
T. Momb{\"a}cher,
M. Monk,
T. Monnard,
S. Monteil,
A. Morcillo Gomez,
G. Morello,
M.J. Morello,
M.P. Morgenthaler,
A.  Moro,
J. Moron,
W.  Morren,
A.B. Morris,
A.G. Morris,
R. Mountain,
Z. M.  Mu,
E. Muhammad,
F. Muheim,
M. Mulder,
K. M{\"u}ller,
F. Mu{\~n}oz-Rojas,
V.  Mytrochenko,
P. Naik,
T. Nakada,
R. Nandakumar,
G.  Napoletano,
I. Nasteva,
M. Needham,
E.  Nekrasova,
N. Neri,
S. Neubert,
N. Neufeld,
P. Neustroev,
J. Nicolini,
D. Nicotra,
E.M. Niel,
N. Nikitin,
L.  Nisi,
Q. Niu,
B. K. Njoki,
P. Nogarolli,
P. Nogga,
C. Normand,
J. Novoa Fernandez,
G. Nowak,
C. Nunez,
H. N.  Nur,
A. Oblakowska-Mucha,
V. Obraztsov,
T. Oeser,
A. Okhotnikov,
O. Okhrimenko,
R. Oldeman,
F. Oliva,
E.  Olivart Pino,
M. Olocco,
R.H. O'Neil,
J.S. Ordonez Soto,
D. Osthues,
J.M. Otalora Goicochea,
P. Owen,
A. Oyanguren,
O. Ozcelik,
F. Paciolla,
A.  Padee,
K.O. Padeken,
B. Pagare,
T. Pajero,
A. Palano,
L.  Palini,
M. Palutan,
C.  Pan,
X.  Pan,
S. Panebianco,
S. Paniskaki,
G. Panshin,
L. Paolucci,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
C. Parkes,
D.  Parmar,
G. Passaleva,
D. Passaro,
A. Pastore,
M. Patel,
J. Patoc,
C. Patrignani,
A.  Paul,
C.J. Pawley,
A. Pellegrino,
J.  Peng,
X.  Peng,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
H.  Pereira Da Costa,
M.  Pereira Martinez,
A. Pereiro Castro,
C.  Perez,
P. Perret,
A.  Perrevoort,
A. Perro,
M.J. Peters,
K. Petridis,
A. Petrolini,
S.  Pezzulo,
J. P.  Pfaller,
H. Pham,
L. Pica,
M. Piccini,
L.  Piccolo,
B. Pietrzyk,
G. Pietrzyk,
R. N. Pilato,
D. Pinci,
F. Pisani,
M. Pizzichemi,
V. M. Placinta,
M. Plo Casasus,
T. Poeschl,
F. Polci,
M. Poli Lener,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
S. Ponce,
D. Popov,
K. Popp,
S. Poslavskii,
K. Prasanth,
C. Prouve,
D. Provenzano,
V. Pugatch,
A.  Puicercus Gomez,
G. Punzi,
J.R. Pybus,
Q. Q.  Qian,
W. Qian,
N. Qin,
R. Quagliani,
R.I. Rabadan Trejo,
R.  Racz,
J.H. Rademacker,
M. Rama,
M.  Ram\'{i}rez Garc\'{i}a,
V. Ramos De Oliveira,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Rebollo De Miguel,
F. Redi,
J. Reich,
F. Reiss,
Z. Ren,
P.K. Resmi,
M.  Ribalda Galvez,
R. Ribatti,
G. Ricart,
D. Riccardi,
S. Ricciardi,
K. Richardson,
M. Richardson-Slipper,
F.  Riehn,
K. Rinnert,
P. Robbe,
G. Robertson,
E. Rodrigues,
A. Rodriguez Alvarez,
E. Rodriguez Fernandez,
J.A. Rodriguez Lopez,
E. Rodriguez Rodriguez,
J. Roensch,
A. Rogachev,
A. Rogovskiy,
D.L. Rolf,
P. Roloff,
V. Romanovskiy,
A. Romero Vidal,
G. Romolini,
F. Ronchetti,
T. Rong,
M. Rotondo,
M.S. Rudolph,
M. Ruiz Diaz,
R.A. Ruiz Fernandez,
J. Ruiz Vidal,
J. J. Saavedra-Arias,
J.J. Saborido Silva,
S. E. R. Sacha Emile R.,
N. Sagidova,
D. Sahoo,
N. Sahoo,
B. Saitta,
M. Salomoni,
I. Sanderswood,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
L. Santoro ,
E. Santovetti,
A. Saputi,
D. Saranin,
A. Sarnatskiy,
G. Sarpis,
M. Sarpis,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
F. Sborzacchi,
A. Scarabotto,
S. Schael,
S. Scherl,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
N. Schmidt,
S. Schmitt,
H. Schmitz,
O. Schneider,
A. Schopper,
N. Schulte,
M.H. Schune,
G. Schwering,
B. Sciascia,
A. Sciuccati,
G.  Scriven,
I. Segal,
S. Sellam,
A. Semennikov,
T. Senger,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
B.  Sevilla Sanjuan,
Y. Shang,
D.M. Shangase,
M. Shapkin,
R. S.  Sharma,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
Z. Shen,
S. Sheng,
V. Shevchenko,
B. Shi,
J.  Shi,
Q. Shi,
W. S.  Shi,
Y. Shimizu,
E. Shmanin,
R. Shorkin,
R. Silva Coutinho,
G. Simi,
S. Simone,
M.  Singha,
I. Siral,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
E. Smith,
M. Smith,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solomin,
A. Solovev,
K.  Solovieva,
N. S.  Sommerfeld,
R. Song,
Y. Song,
Y. Song,
Y. S.  Song,
F.L. Souza De Almeida,
B. Souza De Paula,
K.M. Sowa,
E. Spadaro Norella,
E. Spedicato,
J.G. Speer,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
M.  Stefaniak,
O. Steinkamp,
D. Strekalina,
Y. Su,
F. Suljik,
J. Sun,
J.  Sun,
L. Sun,
D. Sundfeld,
W. Sutcliffe,
P. Svihra,
V. Svintozelskyi,
K. Swientek,
F. Swystun,
A. Szabelski,
T. Szumlak,
Y. Tan,
Y. Tang,
Y. T.  Tang,
M.D. Tat,
J. A. Teijeiro Jimenez,
A. Terentev,
F. Terzuoli,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
A. R.  Thomson-Strong,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
T. T.  Todorov,
L. Tomassetti,
G. Tonani,
X. Tong,
T. Tork,
L. Toscano,
D.Y. Tou,
C. Trippl,
G. Tuci,
N. Tuning,
L.H. Uecker,
A. Ukleja,
D.J. Unverzagt,
A.  Upadhyay,
B.  Urbach,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
V. Vagnoni,
A.  Vaitkevicius,
V.  Valcarce Cadenas,
G. Valenti,
N. Valls Canudas,
J. van Eldik,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
R. Van Laak,
M. van Veghel,
G. Vasquez,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.  Velilla Serna,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Verdoglia,
M. Vesterinen,
W. Vetens,
D.  Vico Benet,
P.  Vidrier Villalba,
M. Vieites Diaz,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
B. Vivacqua,
F.C. Volle,
D. vom Bruch,
N. Voropaev,
K. Vos,
C. Vrahas,
J. Wagner,
J. Walsh,
E.J. Walton,
G. Wan,
A.  Wang,
B.  Wang,
C. Wang,
G. Wang,
H. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
N. W.  Wang,
R. Wang,
X. Wang,
X. Wang,
X. W.  Wang,
Y. Wang,
Y. Wang,
Y. H.  Wang,
Z. Wang,
Z. Wang,
J.A. Ward,
M. Waterlaat,
N.K. Watson,
D. Websdale,
Y. Wei,
Z.  Weida,
J. Wendel,
B.D.C. Westhenry,
C. White,
M. Whitehead,
E. Whiter,
A.R. Wiederhold,
D. Wiedner,
M. A. Wiegertjes,
C.  Wild,
G. Wilkinson,
M.K. Wilkinson,
M. Williams,
M. J. Williams,
M.R.J. Williams,
R. Williams,
S.  Williams,
Z.  Williams,
F.F. Wilson,
M. Winn,
W. Wislicki,
M. Witek,
L. Witola,
T. Wolf,
E.  Wood,
G. Wormser,
S.A. Wotton,
H. Wu,
J. Wu,
X. Wu,
Y. Wu,
Z. Wu,
K. Wyllie,
S. Xian,
Z. Xiang,
Y. Xie,
T. X.  Xing,
A. Xu,
L. Xu,
M. Xu,
Z. Xu,
Z. Xu,
Z. Xu,
S.  Yadav,
K.  Yang,
X. Yang,
Y. Yang,
Y.  Yang,
Z. Yang,
H. Yeung,
H. Yin,
X.  Yin,
C. Y.  Yu,
J. Yu,
X. Yuan,
Y Yuan,
J. A. Zamora Saa,
M. Zavertyaev,
M. Zdybal,
F. Zenesini,
C.  Zeng,
M. Zeng,
C. Zhang,
D. Zhang,
J. Zhang,
L. Zhang,
R. Zhang,
S. Zhang,
S.~L.~  Zhang,
Y. Zhang,
Y. Z.  Zhang,
Z. Zhang,
Y. Zhao,
A. Zhelezov,
S. Z.  Zheng,
X. Z.  Zheng,
Y. Zheng,
T. Zhou,
X. Zhou,
V. Zhovkovska,
L. Z.  Zhu,
X. Zhu,
X. Zhu,
Y.  Zhu,
V. Zhukov,
J. Zhuo,
D. Zuliani,
G. Zunica

==> lhcb_text/Authorship_LHCb-PAPER-2025-057.tex <==
% LHCb collaboration author list
% Data extracted on December 2nd, 2025 at 3:56pm for paper reference LHCb-PAPER-2025-057
\centerline
{\large\bf LHCb collaboration}
\begin
{flushleft}
\small
R.~Aaij$^{38}$\lhcborcid{0000-0003-0533-1952},
A.S.W.~Abdelmotteleb$^{58}$\lhcborcid{0000-0001-7905-0542},
C.~Abellan~Beteta$^{52}$\lhcborcid{0009-0009-0869-6798},
F.~Abudin{\'e}n$^{60}$\lhcborcid{0000-0002-6737-3528},
T.~Ackernley$^{62}$\lhcborcid{0000-0002-5951-3498},
A. A. ~Adefisoye$^{70}$\lhcborcid{0000-0003-2448-1550},
B.~Adeva$^{48}$\lhcborcid{0000-0001-9756-3712},
M.~Adinolfi$^{56}$\lhcborcid{0000-0002-1326-1264},
P.~Adlarson$^{86}$\lhcborcid{0000-0001-6280-3851},
C.~Agapopoulou$^{14}$\lhcborcid{0000-0002-2368-0147},
C.A.~Aidala$^{88}$\lhcborcid{0000-0001-9540-4988},
Z.~Ajaltouni$^{11}$,
S.~Akar$^{11}$\lhcborcid{0000-0003-0288-9694},
K.~Akiba$^{38}$\lhcborcid{0000-0002-6736-471X},
M. ~Akthar$^{40}$\lhcborcid{0009-0003-3172-2997},
P.~Albicocco$^{28}$\lhcborcid{0000-0001-6430-1038},
J.~Albrecht$^{19,g}$\lhcborcid{0000-0001-8636-1621},
R. ~Aleksiejunas$^{82}$\lhcborcid{0000-0002-9093-2252},
F.~Alessio$^{50}$\lhcborcid{0000-0001-5317-1098},
P.~Alvarez~Cartelle$^{57,48}$\lhcborcid{0000-0003-1652-2834},
R.~Amalric$^{16}$\lhcborcid{0000-0003-4595-2729},
S.~Amato$^{3}$\lhcborcid{0000-0002-3277-0662},
J.L.~Amey$^{56}$\lhcborcid{0000-0002-2597-3808},
Y.~Amhis$^{14}$\lhcborcid{0000-0003-4282-1512},
L.~An$^{6}$\lhcborcid{0000-0002-3274-5627},
L.~Anderlini$^{27}$\lhcborcid{0000-0001-6808-2418},
M.~Andersson$^{52}$\lhcborcid{0000-0003-3594-9163},
P.~Andreola$^{52}$\lhcborcid{0000-0002-3923-431X},
M.~Andreotti$^{26}$\lhcborcid{0000-0003-2918-1311},
S. ~Andres~Estrada$^{45}$\lhcborcid{0009-0004-1572-0964},
A.~Anelli$^{31,p}$\lhcborcid{0000-0002-6191-934X},
D.~Ao$^{7}$\lhcborcid{0000-0003-1647-4238},
C.~Arata$^{12}$\lhcborcid{0009-0002-1990-7289},
F.~Archilli$^{37}$\lhcborcid{0000-0002-1779-6813},
Z.~Areg$^{70}$\lhcborcid{0009-0001-8618-2305},
M.~Argenton$^{26}$\lhcborcid{0009-0006-3169-0077},
S.~Arguedas~Cuendis$^{9,50}$\lhcborcid{0000-0003-4234-7005},
L. ~Arnone$^{31,p}$\lhcborcid{0009-0008-2154-8493},
A.~Artamonov$^{44}$\lhcborcid{0000-0002-2785-2233},
M.~Artuso$^{70}$\lhcborcid{0000-0002-5991-7273},
E.~Aslanides$^{13}$\lhcborcid{0000-0003-3286-683X},
R.~Ata\'{i}de~Da~Silva$^{51}$\lhcborcid{0009-0005-1667-2666},
M.~Atzeni$^{66}$\lhcborcid{0000-0002-3208-3336},
B.~Audurier$^{12}$\lhcborcid{0000-0001-9090-4254},
J. A. ~Authier$^{15}$\lhcborcid{0009-0000-4716-5097},
D.~Bacher$^{65}$\lhcborcid{0000-0002-1249-367X},
I.~Bachiller~Perea$^{51}$\lhcborcid{0000-0002-3721-4876},
S.~Bachmann$^{22}$\lhcborcid{0000-0002-1186-3894},
M.~Bachmayer$^{51}$\lhcborcid{0000-0001-5996-2747},
J.J.~Back$^{58}$\lhcborcid{0000-0001-7791-4490},
P.~Baladron~Rodriguez$^{48}$\lhcborcid{0000-0003-4240-2094},
V.~Balagura$^{15}$\lhcborcid{0000-0002-1611-7188},
A. ~Balboni$^{26}$\lhcborcid{0009-0003-8872-976X},
W.~Baldini$^{26}$\lhcborcid{0000-0001-7658-8777},
Z.~Baldwin$^{80}$\lhcborcid{0000-0002-8534-0922},
L.~Balzani$^{19}$\lhcborcid{0009-0006-5241-1452},
H. ~Bao$^{7}$\lhcborcid{0009-0002-7027-021X},
J.~Baptista~de~Souza~Leite$^{2}$\lhcborcid{0000-0002-4442-5372},
C.~Barbero~Pretel$^{48,12}$\lhcborcid{0009-0001-1805-6219},
M.~Barbetti$^{27}$\lhcborcid{0000-0002-6704-6914},
I. R.~Barbosa$^{71}$\lhcborcid{0000-0002-3226-8672},
R.J.~Barlow$^{64}$\lhcborcid{0000-0002-8295-8612},
M.~Barnyakov$^{25}$\lhcborcid{0009-0000-0102-0482},
S.~Barsuk$^{14}$\lhcborcid{0000-0002-0898-6551},
W.~Barter$^{60}$\lhcborcid{0000-0002-9264-4799},
J.~Bartz$^{70}$\lhcborcid{0000-0002-2646-4124},
S.~Bashir$^{40}$\lhcborcid{0000-0001-9861-8922},
B.~Batsukh$^{5}$\lhcborcid{0000-0003-1020-2549},
P. B. ~Battista$^{14}$\lhcborcid{0009-0005-5095-0439},
A. ~Bavarchee$^{81}$\lhcborcid{0000-0001-7880-4525},
A.~Bay$^{51}$\lhcborcid{0000-0002-4862-9399},
A.~Beck$^{66}$\lhcborcid{0000-0003-4872-1213},
M.~Becker$^{19}$\lhcborcid{0000-0002-7972-8760},
F.~Bedeschi$^{35}$\lhcborcid{0000-0002-8315-2119},
I.B.~Bediaga$^{2}$\lhcborcid{0000-0001-7806-5283},
N. A. ~Behling$^{19}$\lhcborcid{0000-0003-4750-7872},
S.~Belin$^{48}$\lhcborcid{0000-0001-7154-1304},
A. ~Bellavista$^{25}$\lhcborcid{0009-0009-3723-834X},
K.~Belous$^{44}$\lhcborcid{0000-0003-0014-2589},
I.~Belov$^{29}$\lhcborcid{0000-0003-1699-9202},
I.~Belyaev$^{36}$\lhcborcid{0000-0002-7458-7030},
G.~Benane$^{13}$\lhcborcid{0000-0002-8176-8315},
G.~Bencivenni$^{28}$\lhcborcid{0000-0002-5107-0610},
E.~Ben-Haim$^{16}$\lhcborcid{0000-0002-9510-8414},
A.~Berezhnoy$^{44}$\lhcborcid{0000-0002-4431-7582},
R.~Bernet$^{52}$\lhcborcid{0000-0002-4856-8063},
S.~Bernet~Andres$^{47}$\lhcborcid{0000-0002-4515-7541},
A.~Bertolin$^{33}$\lhcborcid{0000-0003-1393-4315},
F.~Betti$^{60}$\lhcborcid{0000-0002-2395-235X},
J. ~Bex$^{57}$\lhcborcid{0000-0002-2856-8074},
O.~Bezshyyko$^{87}$\lhcborcid{0000-0001-7106-5213},
S. ~Bhattacharya$^{81}$\lhcborcid{0009-0007-8372-6008},
M.S.~Bieker$^{18}$\lhcborcid{0000-0001-7113-7862},
N.V.~Biesuz$^{26}$\lhcborcid{0000-0003-3004-0946},
A.~Biolchini$^{38}$\lhcborcid{0000-0001-6064-9993},
M.~Birch$^{63}$\lhcborcid{0000-0001-9157-4461},
F.C.R.~Bishop$^{10}$\lhcborcid{0000-0002-0023-3897},
A.~Bitadze$^{64}$\lhcborcid{0000-0001-7979-1092},
A.~Bizzeti$^{27,q}$\lhcborcid{0000-0001-5729-5530},
T.~Blake$^{58,c}$\lhcborcid{0000-0002-0259-5891},
F.~Blanc$^{51}$\lhcborcid{0000-0001-5775-3132},
J.E.~Blank$^{19}$\lhcborcid{0000-0002-6546-5605},
S.~Blusk$^{70}$\lhcborcid{0000-0001-9170-684X},
V.~Bocharnikov$^{44}$\lhcborcid{0000-0003-1048-7732},
J.A.~Boelhauve$^{19}$\lhcborcid{0000-0002-3543-9959},
O.~Boente~Garcia$^{50}$\lhcborcid{0000-0003-0261-8085},
T.~Boettcher$^{89}$\lhcborcid{0000-0002-2439-9955},
A. ~Bohare$^{60}$\lhcborcid{0000-0003-1077-8046},
A.~Boldyrev$^{44}$\lhcborcid{0000-0002-7872-6819},
C.~Bolognani$^{84}$\lhcborcid{0000-0003-3752-6789},
R.~Bolzonella$^{26,m}$\lhcborcid{0000-0002-0055-0577},
R. B. ~Bonacci$^{1}$\lhcborcid{0009-0004-1871-2417},
N.~Bondar$^{44,50}$\lhcborcid{0000-0003-2714-9879},
A.~Bordelius$^{50}$\lhcborcid{0009-0002-3529-8524},
F.~Borgato$^{33,50}$\lhcborcid{0000-0002-3149-6710},
S.~Borghi$^{64}$\lhcborcid{0000-0001-5135-1511},
M.~Borsato$^{31,p}$\lhcborcid{0000-0001-5760-2924},
J.T.~Borsuk$^{85}$\lhcborcid{0000-0002-9065-9030},
E. ~Bottalico$^{62}$\lhcborcid{0000-0003-2238-8803},
S.A.~Bouchiba$^{51}$\lhcborcid{0000-0002-0044-6470},
M. ~Bovill$^{65}$\lhcborcid{0009-0006-2494-8287},
T.J.V.~Bowcock$^{62}$\lhcborcid{0000-0002-3505-6915},
A.~Boyer$^{50}$\lhcborcid{0000-0002-9909-0186},
C.~Bozzi$^{26}$\lhcborcid{0000-0001-6782-3982},
J. D.~Brandenburg$^{90}$\lhcborcid{0000-0002-6327-5947},
A.~Brea~Rodriguez$^{51}$\lhcborcid{0000-0001-5650-445X},
N.~Breer$^{19}$\lhcborcid{0000-0003-0307-3662},
J.~Brodzicka$^{41}$\lhcborcid{0000-0002-8556-0597},
J.~Brown$^{62}$\lhcborcid{0000-0001-9846-9672},
D.~Brundu$^{32}$\lhcborcid{0000-0003-4457-5896},
E.~Buchanan$^{60}$\lhcborcid{0009-0008-3263-1823},
M. ~Burgos~Marcos$^{84}$\lhcborcid{0009-0001-9716-0793},
C.~Burr$^{50}$\lhcborcid{0000-0002-5155-1094},
C. ~Buti$^{27}$\lhcborcid{0009-0009-2488-5548},
J.S.~Butter$^{57}$\lhcborcid{0000-0002-1816-536X},
J.~Buytaert$^{50}$\lhcborcid{0000-0002-7958-6790},
W.~Byczynski$^{50}$\lhcborcid{0009-0008-0187-3395},
S.~Cadeddu$^{32}$\lhcborcid{0000-0002-7763-500X},
H.~Cai$^{76}$\lhcborcid{0000-0003-0898-3673},
Y. ~Cai$^{5}$\lhcborcid{0009-0004-5445-9404},
A.~Caillet$^{16}$\lhcborcid{0009-0001-8340-3870},
R.~Calabrese$^{26,m}$\lhcborcid{0000-0002-1354-5400},
L.~Calefice$^{46}$\lhcborcid{0000-0001-6401-1583},
M.~Calvi$^{31,p}$\lhcborcid{0000-0002-8797-1357},
M.~Calvo~Gomez$^{47}$\lhcborcid{0000-0001-5588-1448},
P.~Camargo~Magalhaes$^{2,a}$\lhcborcid{0000-0003-3641-8110},
J. I.~Cambon~Bouzas$^{48}$\lhcborcid{0000-0002-2952-3118},
P.~Campana$^{28}$\lhcborcid{0000-0001-8233-1951},
A. C.~Campos$^{3}$\lhcborcid{0009-0000-0785-8163},
A.F.~Campoverde~Quezada$^{7}$\lhcborcid{0000-0003-1968-1216},
S.~Capelli$^{31}$\lhcborcid{0000-0002-8444-4498},
M. ~Caporale$^{25}$\lhcborcid{0009-0008-9395-8723},
L.~Capriotti$^{26}$\lhcborcid{0000-0003-4899-0587},
R.~Caravaca-Mora$^{9}$\lhcborcid{0000-0001-8010-0447},
A.~Carbone$^{25,k}$\lhcborcid{0000-0002-7045-2243},
L.~Carcedo~Salgado$^{48}$\lhcborcid{0000-0003-3101-3528},
R.~Cardinale$^{29,n}$\lhcborcid{0000-0002-7835-7638},
A.~Cardini$^{32}$\lhcborcid{0000-0002-6649-0298},
P.~Carniti$^{31}$\lhcborcid{0000-0002-7820-2732},
L.~Carus$^{22}$\lhcborcid{0009-0009-5251-2474},
A.~Casais~Vidal$^{66}$\lhcborcid{0000-0003-0469-2588},
R.~Caspary$^{22}$\lhcborcid{0000-0002-1449-1619},
G.~Casse$^{62}$\lhcborcid{0000-0002-8516-237X},
M.~Cattaneo$^{50}$\lhcborcid{0000-0001-7707-169X},
G.~Cavallero$^{26}$\lhcborcid{0000-0002-8342-7047},
V.~Cavallini$^{26,m}$\lhcborcid{0000-0001-7601-129X},
S.~Celani$^{50}$\lhcborcid{0000-0003-4715-7622},
I. ~Celestino$^{35,t}$\lhcborcid{0009-0008-0215-0308},
S. ~Cesare$^{50,o}$\lhcborcid{0000-0003-0886-7111},
A.J.~Chadwick$^{62}$\lhcborcid{0000-0003-3537-9404},
I.~Chahrour$^{88}$\lhcborcid{0000-0002-1472-0987},
H. ~Chang$^{4,d}$\lhcborcid{0009-0002-8662-1918},
M.~Charles$^{16}$\lhcborcid{0000-0003-4795-498X},
Ph.~Charpentier$^{50}$\lhcborcid{0000-0001-9295-8635},
E. ~Chatzianagnostou$^{38}$\lhcborcid{0009-0009-3781-1820},
R. ~Cheaib$^{81}$\lhcborcid{0000-0002-6292-3068},
M.~Chefdeville$^{10}$\lhcborcid{0000-0002-6553-6493},
C.~Chen$^{57}$\lhcborcid{0000-0002-3400-5489},
J. ~Chen$^{51}$\lhcborcid{0009-0006-1819-4271},
S.~Chen$^{5}$\lhcborcid{0000-0002-8647-1828},
Z.~Chen$^{7}$\lhcborcid{0000-0002-0215-7269},
A. ~Chen~Hu$^{63}$\lhcborcid{0009-0002-3626-8909 },
M. ~Cherif$^{12}$\lhcborcid{0009-0004-4839-7139},
A.~Chernov$^{41}$\lhcborcid{0000-0003-0232-6808},
S.~Chernyshenko$^{54}$\lhcborcid{0000-0002-2546-6080},
X. ~Chiotopoulos$^{84}$\lhcborcid{0009-0006-5762-6559},
V.~Chobanova$^{45}$\lhcborcid{0000-0002-1353-6002},
M.~Chrzaszcz$^{41}$\lhcborcid{0000-0001-7901-8710},
A.~Chubykin$^{44}$\lhcborcid{0000-0003-1061-9643},
V.~Chulikov$^{28,36,50}$\lhcborcid{0000-0002-7767-9117},
P.~Ciambrone$^{28}$\lhcborcid{0000-0003-0253-9846},
X.~Cid~Vidal$^{48}$\lhcborcid{0000-0002-0468-541X},
G.~Ciezarek$^{50}$\lhcborcid{0000-0003-1002-8368},
P.~Cifra$^{38}$\lhcborcid{0000-0003-3068-7029},
P.E.L.~Clarke$^{60}$\lhcborcid{0000-0003-3746-0732},
M.~Clemencic$^{50}$\lhcborcid{0000-0003-1710-6824},
H.V.~Cliff$^{57}$\lhcborcid{0000-0003-0531-0916},
J.~Closier$^{50}$\lhcborcid{0000-0002-0228-9130},
C.~Cocha~Toapaxi$^{22}$\lhcborcid{0000-0001-5812-8611},
V.~Coco$^{50}$\lhcborcid{0000-0002-5310-6808},
J.~Cogan$^{13}$\lhcborcid{0000-0001-7194-7566},
E.~Cogneras$^{11}$\lhcborcid{0000-0002-8933-9427},
L.~Cojocariu$^{43}$\lhcborcid{0000-0002-1281-5923},
S. ~Collaviti$^{51}$\lhcborcid{0009-0003-7280-8236},
P.~Collins$^{50}$\lhcborcid{0000-0003-1437-4022},
T.~Colombo$^{50}$\lhcborcid{0000-0002-9617-9687},
M.~Colonna$^{19}$\lhcborcid{0009-0000-1704-4139},
A.~Comerma-Montells$^{46}$\lhcborcid{0000-0002-8980-6048},
L.~Congedo$^{24}$\lhcborcid{0000-0003-4536-4644},
J. ~Connaughton$^{58}$\lhcborcid{0000-0003-2557-4361},
A.~Contu$^{32}$\lhcborcid{0000-0002-3545-2969},
N.~Cooke$^{61}$\lhcborcid{0000-0002-4179-3700},
G.~Cordova$^{35,t}$\lhcborcid{0009-0003-8308-4798},
C. ~Coronel$^{67}$\lhcborcid{0009-0006-9231-4024},
I.~Corredoira~$^{12}$\lhcborcid{0000-0002-6089-0899},
A.~Correia$^{16}$\lhcborcid{0000-0002-6483-8596},
G.~Corti$^{50}$\lhcborcid{0000-0003-2857-4471},
J.~Cottee~Meldrum$^{56}$\lhcborcid{0009-0009-3900-6905},
B.~Couturier$^{50}$\lhcborcid{0000-0001-6749-1033},
D.C.~Craik$^{52}$\lhcborcid{0000-0002-3684-1560},
M.~Cruz~Torres$^{2,h}$\lhcborcid{0000-0003-2607-131X},
M. ~Cubero~Campos$^{9}$\lhcborcid{0000-0002-5183-4668},
E.~Curras~Rivera$^{51}$\lhcborcid{0000-0002-6555-0340},
R.~Currie$^{60}$\lhcborcid{0000-0002-0166-9529},
C.L.~Da~Silva$^{69}$\lhcborcid{0000-0003-4106-8258},
S.~Dadabaev$^{44}$\lhcborcid{0000-0002-0093-3244},
X.~Dai$^{4}$\lhcborcid{0000-0003-3395-7151},
E.~Dall'Occo$^{50}$\lhcborcid{0000-0001-9313-4021},
J.~Dalseno$^{45}$\lhcborcid{0000-0003-3288-4683},
C.~D'Ambrosio$^{63}$\lhcborcid{0000-0003-4344-9994},
J.~Daniel$^{11}$\lhcborcid{0000-0002-9022-4264},
G.~Darze$^{3}$\lhcborcid{0000-0002-7666-6533},
A. ~Davidson$^{58}$\lhcborcid{0009-0002-0647-2028},
J.E.~Davies$^{64}$\lhcborcid{0000-0002-5382-8683},
O.~De~Aguiar~Francisco$^{64}$\lhcborcid{0000-0003-2735-678X},
C.~De~Angelis$^{32,l}$\lhcborcid{0009-0005-5033-5866},
F.~De~Benedetti$^{50}$\lhcborcid{0000-0002-7960-3116},
J.~de~Boer$^{38}$\lhcborcid{0000-0002-6084-4294},
K.~De~Bruyn$^{83}$\lhcborcid{0000-0002-0615-4399},
S.~De~Capua$^{64}$\lhcborcid{0000-0002-6285-9596},
M.~De~Cian$^{64,50}$\lhcborcid{0000-0002-1268-9621},
U.~De~Freitas~Carneiro~Da~Graca$^{2,b}$\lhcborcid{0000-0003-0451-4028},
E.~De~Lucia$^{28}$\lhcborcid{0000-0003-0793-0844},
J.M.~De~Miranda$^{2}$\lhcborcid{0009-0003-2505-7337},
L.~De~Paula$^{3}$\lhcborcid{0000-0002-4984-7734},
M.~De~Serio$^{24,i}$\lhcborcid{0000-0003-4915-7933},
P.~De~Simone$^{28}$\lhcborcid{0000-0001-9392-2079},
F.~De~Vellis$^{19}$\lhcborcid{0000-0001-7596-5091},
J.A.~de~Vries$^{84}$\lhcborcid{0000-0003-4712-9816},
F.~Debernardis$^{24}$\lhcborcid{0009-0001-5383-4899},
D.~Decamp$^{10}$\lhcborcid{0000-0001-9643-6762},
S. ~Dekkers$^{1}$\lhcborcid{0000-0001-9598-875X},
L.~Del~Buono$^{16}$\lhcborcid{0000-0003-4774-2194},
B.~Delaney$^{66}$\lhcborcid{0009-0007-6371-8035},
J.~Deng$^{8}$\lhcborcid{0000-0002-4395-3616},
V.~Denysenko$^{52}$\lhcborcid{0000-0002-0455-5404},
O.~Deschamps$^{11}$\lhcborcid{0000-0002-7047-6042},
F.~Dettori$^{32,l}$\lhcborcid{0000-0003-0256-8663},
B.~Dey$^{81}$\lhcborcid{0000-0002-4563-5806},
P.~Di~Nezza$^{28}$\lhcborcid{0000-0003-4894-6762},
I.~Diachkov$^{44}$\lhcborcid{0000-0001-5222-5293},
S.~Didenko$^{44}$\lhcborcid{0000-0001-5671-5863},
S.~Ding$^{70}$\lhcborcid{0000-0002-5946-581X},
Y. ~Ding$^{51}$\lhcborcid{0009-0008-2518-8392},
L.~Dittmann$^{22}$\lhcborcid{0009-0000-0510-0252},
V.~Dobishuk$^{54}$\lhcborcid{0000-0001-9004-3255},
A. D. ~Docheva$^{61}$\lhcborcid{0000-0002-7680-4043},
A. ~Doheny$^{58}$\lhcborcid{0009-0006-2410-6282},
C.~Dong$^{d,4}$\lhcborcid{0000-0003-3259-6323},
F.~Dordei$^{32}$\lhcborcid{0000-0002-2571-5067},
A.C.~dos~Reis$^{2}$\lhcborcid{0000-0001-7517-8418},
A. D. ~Dowling$^{70}$\lhcborcid{0009-0007-1406-3343},
L.~Dreyfus$^{13}$\lhcborcid{0009-0000-2823-5141},
W.~Duan$^{74}$\lhcborcid{0000-0003-1765-9939},
P.~Duda$^{85}$\lhcborcid{0000-0003-4043-7963},
L.~Dufour$^{51}$\lhcborcid{0000-0002-3924-2774},
V.~Duk$^{34}$\lhcborcid{0000-0001-6440-0087},
P.~Durante$^{50}$\lhcborcid{0000-0002-1204-2270},
M. M.~Duras$^{85}$\lhcborcid{0000-0002-4153-5293},
J.M.~Durham$^{69}$\lhcborcid{0000-0002-5831-3398},
O. D. ~Durmus$^{81}$\lhcborcid{0000-0002-8161-7832},
A.~Dziurda$^{41}$\lhcborcid{0000-0003-4338-7156},
A.~Dzyuba$^{44}$\lhcborcid{0000-0003-3612-3195},
S.~Easo$^{59}$\lhcborcid{0000-0002-4027-7333},
E.~Eckstein$^{18}$\lhcborcid{0009-0009-5267-5177},
U.~Egede$^{1}$\lhcborcid{0000-0001-5493-0762},
A.~Egorychev$^{44}$\lhcborcid{0000-0001-5555-8982},
V.~Egorychev$^{44}$\lhcborcid{0000-0002-2539-673X},
S.~Eisenhardt$^{60}$\lhcborcid{0000-0002-4860-6779},
E.~Ejopu$^{62}$\lhcborcid{0000-0003-3711-7547},
L.~Eklund$^{86}$\lhcborcid{0000-0002-2014-3864},
M.~Elashri$^{67}$\lhcborcid{0000-0001-9398-953X},
D. ~Elizondo~Blanco$^{9}$\lhcborcid{0009-0007-4950-0822},
J.~Ellbracht$^{19}$\lhcborcid{0000-0003-1231-6347},
S.~Ely$^{63}$\lhcborcid{0000-0003-1618-3617},
A.~Ene$^{43}$\lhcborcid{0000-0001-5513-0927},
J.~Eschle$^{70}$\lhcborcid{0000-0002-7312-3699},
T.~Evans$^{38}$\lhcborcid{0000-0003-3016-1879},
F.~Fabiano$^{14}$\lhcborcid{0000-0001-6915-9923},
S. ~Faghih$^{67}$\lhcborcid{0009-0008-3848-4967},
L.N.~Falcao$^{31,p}$\lhcborcid{0000-0003-3441-583X},
B.~Fang$^{7}$\lhcborcid{0000-0003-0030-3813},
R.~Fantechi$^{35}$\lhcborcid{0000-0002-6243-5726},
L.~Fantini$^{34,s}$\lhcborcid{0000-0002-2351-3998},
M.~Faria$^{51}$\lhcborcid{0000-0002-4675-4209},
K.  ~Farmer$^{60}$\lhcborcid{0000-0003-2364-2877},
F. ~Fassin$^{83,38}$\lhcborcid{0009-0002-9804-5364},
D.~Fazzini$^{31,p}$\lhcborcid{0000-0002-5938-4286},
L.~Felkowski$^{85}$\lhcborcid{0000-0002-0196-910X},
M.~Feng$^{5,7}$\lhcborcid{0000-0002-6308-5078},
A.~Fernandez~Casani$^{49}$\lhcborcid{0000-0003-1394-509X},
M.~Fernandez~Gomez$^{48}$\lhcborcid{0000-0003-1984-4759},
A.D.~Fernez$^{68}$\lhcborcid{0000-0001-9900-6514},
F.~Ferrari$^{25,k}$\lhcborcid{0000-0002-3721-4585},
F.~Ferreira~Rodrigues$^{3}$\lhcborcid{0000-0002-4274-5583},
M.~Ferrillo$^{52}$\lhcborcid{0000-0003-1052-2198},
M.~Ferro-Luzzi$^{50}$\lhcborcid{0009-0008-1868-2165},
S.~Filippov$^{44}$\lhcborcid{0000-0003-3900-3914},
R.A.~Fini$^{24}$\lhcborcid{0000-0002-3821-3998},
M.~Fiorini$^{26,m}$\lhcborcid{0000-0001-6559-2084},
M.~Firlej$^{40}$\lhcborcid{0000-0002-1084-0084},
K.L.~Fischer$^{65}$\lhcborcid{0009-0000-8700-9910},
D.S.~Fitzgerald$^{88}$\lhcborcid{0000-0001-6862-6876},
C.~Fitzpatrick$^{64}$\lhcborcid{0000-0003-3674-0812},
T.~Fiutowski$^{40}$\lhcborcid{0000-0003-2342-8854},
F.~Fleuret$^{15}$\lhcborcid{0000-0002-2430-782X},
A. ~Fomin$^{53}$\lhcborcid{0000-0002-3631-0604},
M.~Fontana$^{25,50}$\lhcborcid{0000-0003-4727-831X},
L. A. ~Foreman$^{64}$\lhcborcid{0000-0002-2741-9966},
R.~Forty$^{50}$\lhcborcid{0000-0003-2103-7577},
D.~Foulds-Holt$^{60}$\lhcborcid{0000-0001-9921-687X},
V.~Franco~Lima$^{3}$\lhcborcid{0000-0002-3761-209X},
M.~Franco~Sevilla$^{68}$\lhcborcid{0000-0002-5250-2948},
M.~Frank$^{50}$\lhcborcid{0000-0002-4625-559X},
E.~Franzoso$^{26,m}$\lhcborcid{0000-0003-2130-1593},
G.~Frau$^{64}$\lhcborcid{0000-0003-3160-482X},
C.~Frei$^{50}$\lhcborcid{0000-0001-5501-5611},
D.A.~Friday$^{64,50}$\lhcborcid{0000-0001-9400-3322},
J.~Fu$^{7}$\lhcborcid{0000-0003-3177-2700},
Q.~F{\"u}hring$^{19,g,57}$\lhcborcid{0000-0003-3179-2525},
T.~Fulghesu$^{13}$\lhcborcid{0000-0001-9391-8619},
G.~Galati$^{24,i}$\lhcborcid{0000-0001-7348-3312},
M.D.~Galati$^{38}$\lhcborcid{0000-0002-8716-4440},
A.~Gallas~Torreira$^{48}$\lhcborcid{0000-0002-2745-7954},
D.~Galli$^{25,k}$\lhcborcid{0000-0003-2375-6030},
S.~Gambetta$^{60}$\lhcborcid{0000-0003-2420-0501},
M.~Gandelman$^{3}$\lhcborcid{0000-0001-8192-8377},
P.~Gandini$^{30}$\lhcborcid{0000-0001-7267-6008},
B. ~Ganie$^{64}$\lhcborcid{0009-0008-7115-3940},
H.~Gao$^{7}$\lhcborcid{0000-0002-6025-6193},
R.~Gao$^{65}$\lhcborcid{0009-0004-1782-7642},
T.Q.~Gao$^{57}$\lhcborcid{0000-0001-7933-0835},
Y.~Gao$^{8}$\lhcborcid{0000-0002-6069-8995},
Y.~Gao$^{6}$\lhcborcid{0000-0003-1484-0943},
Y.~Gao$^{8}$\lhcborcid{0009-0002-5342-4475},
L.M.~Garcia~Martin$^{51}$\lhcborcid{0000-0003-0714-8991},
P.~Garcia~Moreno$^{46}$\lhcborcid{0000-0002-3612-1651},
J.~Garc{\'\i}a~Pardi{\~n}as$^{66}$\lhcborcid{0000-0003-2316-8829},
P. ~Gardner$^{68}$\lhcborcid{0000-0002-8090-563X},
L.~Garrido$^{46}$\lhcborcid{0000-0001-8883-6539},
C.~Gaspar$^{50}$\lhcborcid{0000-0002-8009-1509},
A. ~Gavrikov$^{33}$\lhcborcid{0000-0002-6741-5409},
L.L.~Gerken$^{19}$\lhcborcid{0000-0002-6769-3679},
E.~Gersabeck$^{20}$\lhcborcid{0000-0002-2860-6528},
M.~Gersabeck$^{20}$\lhcborcid{0000-0002-0075-8669},
T.~Gershon$^{58}$\lhcborcid{0000-0002-3183-5065},
S.~Ghizzo$^{29,n}$\lhcborcid{0009-0001-5178-9385},
Z.~Ghorbanimoghaddam$^{56}$\lhcborcid{0000-0002-4410-9505},
F. I.~Giasemis$^{16,f}$\lhcborcid{0000-0003-0622-1069},
V.~Gibson$^{57}$\lhcborcid{0000-0002-6661-1192},
H.K.~Giemza$^{42}$\lhcborcid{0000-0003-2597-8796},
A.L.~Gilman$^{67}$\lhcborcid{0000-0001-5934-7541},
M.~Giovannetti$^{28}$\lhcborcid{0000-0003-2135-9568},
A.~Giovent{\`u}$^{46}$\lhcborcid{0000-0001-5399-326X},
L.~Girardey$^{64,59}$\lhcborcid{0000-0002-8254-7274},
M.A.~Giza$^{41}$\lhcborcid{0000-0002-0805-1561},
F.C.~Glaser$^{22,14}$\lhcborcid{0000-0001-8416-5416},
V.V.~Gligorov$^{16}$\lhcborcid{0000-0002-8189-8267},
C.~G{\"o}bel$^{71}$\lhcborcid{0000-0003-0523-495X},
L. ~Golinka-Bezshyyko$^{87}$\lhcborcid{0000-0002-0613-5374},
E.~Golobardes$^{47}$\lhcborcid{0000-0001-8080-0769},
D.~Golubkov$^{44}$\lhcborcid{0000-0001-6216-1596},
A.~Golutvin$^{63,50}$\lhcborcid{0000-0003-2500-8247},
S.~Gomez~Fernandez$^{46}$\lhcborcid{0000-0002-3064-9834},
W. ~Gomulka$^{40}$\lhcborcid{0009-0003-2873-425X},
I.~Gonçales~Vaz$^{50}$\lhcborcid{0009-0006-4585-2882},
F.~Goncalves~Abrantes$^{65}$\lhcborcid{0000-0002-7318-482X},
M.~Goncerz$^{41}$\lhcborcid{0000-0002-9224-914X},
G.~Gong$^{4,d}$\lhcborcid{0000-0002-7822-3947},
J. A.~Gooding$^{19}$\lhcborcid{0000-0003-3353-9750},
I.V.~Gorelov$^{44}$\lhcborcid{0000-0001-5570-0133},
C.~Gotti$^{31}$\lhcborcid{0000-0003-2501-9608},
E.~Govorkova$^{66}$\lhcborcid{0000-0003-1920-6618},
J.P.~Grabowski$^{30}$\lhcborcid{0000-0001-8461-8382},
L.A.~Granado~Cardoso$^{50}$\lhcborcid{0000-0003-2868-2173},
E.~Graug{\'e}s$^{46}$\lhcborcid{0000-0001-6571-4096},
E.~Graverini$^{35,51}$\lhcborcid{0000-0003-4647-6429},
L.~Grazette$^{58}$\lhcborcid{0000-0001-7907-4261},
G.~Graziani$^{27}$\lhcborcid{0000-0001-8212-846X},
A. T.~Grecu$^{43}$\lhcborcid{0000-0002-7770-1839},
N.A.~Grieser$^{67}$\lhcborcid{0000-0003-0386-4923},
L.~Grillo$^{61}$\lhcborcid{0000-0001-5360-0091},
S.~Gromov$^{44}$\lhcborcid{0000-0002-8967-3644},
C. ~Gu$^{15}$\lhcborcid{0000-0001-5635-6063},
M.~Guarise$^{26}$\lhcborcid{0000-0001-8829-9681},
L. ~Guerry$^{11}$\lhcborcid{0009-0004-8932-4024},
A.-K.~Guseinov$^{51}$\lhcborcid{0000-0002-5115-0581},
E.~Gushchin$^{44}$\lhcborcid{0000-0001-8857-1665},
Y.~Guz$^{6,50}$\lhcborcid{0000-0001-7552-400X},
T.~Gys$^{50}$\lhcborcid{0000-0002-6825-6497},
K.~Habermann$^{18}$\lhcborcid{0009-0002-6342-5965},
T.~Hadavizadeh$^{1}$\lhcborcid{0000-0001-5730-8434},
C.~Hadjivasiliou$^{68}$\lhcborcid{0000-0002-2234-0001},
G.~Haefeli$^{51}$\lhcborcid{0000-0002-9257-839X},
C.~Haen$^{50}$\lhcborcid{0000-0002-4947-2928},
S. ~Haken$^{57}$\lhcborcid{0009-0007-9578-2197},
G. ~Hallett$^{58}$\lhcborcid{0009-0005-1427-6520},
P.M.~Hamilton$^{68}$\lhcborcid{0000-0002-2231-1374},
J.~Hammerich$^{62}$\lhcborcid{0000-0002-5556-1775},
Q.~Han$^{33}$\lhcborcid{0000-0002-7958-2917},
X.~Han$^{22,50}$\lhcborcid{0000-0001-7641-7505},
S.~Hansmann-Menzemer$^{22}$\lhcborcid{0000-0002-3804-8734},
L.~Hao$^{7}$\lhcborcid{0000-0001-8162-4277},
N.~Harnew$^{65}$\lhcborcid{0000-0001-9616-6651},
T. H. ~Harris$^{1}$\lhcborcid{0009-0000-1763-6759},
M.~Hartmann$^{14}$\lhcborcid{0009-0005-8756-0960},
S.~Hashmi$^{40}$\lhcborcid{0000-0003-2714-2706},
J.~He$^{7,e}$\lhcborcid{0000-0002-1465-0077},
N. ~Heatley$^{14}$\lhcborcid{0000-0003-2204-4779},
A. ~Hedes$^{64}$\lhcborcid{0009-0005-2308-4002},
F.~Hemmer$^{50}$\lhcborcid{0000-0001-8177-0856},
C.~Henderson$^{67}$\lhcborcid{0000-0002-6986-9404},
R.~Henderson$^{14}$\lhcborcid{0009-0006-3405-5888},
R.D.L.~Henderson$^{1}$\lhcborcid{0000-0001-6445-4907},
A.M.~Hennequin$^{50}$\lhcborcid{0009-0008-7974-3785},
K.~Hennessy$^{62}$\lhcborcid{0000-0002-1529-8087},
L.~Henry$^{51}$\lhcborcid{0000-0003-3605-832X},
J.~Herd$^{63}$\lhcborcid{0000-0001-7828-3694},
P.~Herrero~Gascon$^{22}$\lhcborcid{0000-0001-6265-8412},
J.~Heuel$^{17}$\lhcborcid{0000-0001-9384-6926},
A. ~Heyn$^{13}$\lhcborcid{0009-0009-2864-9569},
A.~Hicheur$^{3}$\lhcborcid{0000-0002-3712-7318},
G.~Hijano~Mendizabal$^{52}$\lhcborcid{0009-0002-1307-1759},
J.~Horswill$^{64}$\lhcborcid{0000-0002-9199-8616},
R.~Hou$^{8}$\lhcborcid{0000-0002-3139-3332},
Y.~Hou$^{11}$\lhcborcid{0000-0001-6454-278X},
D.C.~Houston$^{61}$\lhcborcid{0009-0003-7753-9565},
N.~Howarth$^{62}$\lhcborcid{0009-0001-7370-061X},
W.~Hu$^{7}$\lhcborcid{0000-0002-2855-0544},
X.~Hu$^{4}$\lhcborcid{0000-0002-5924-2683},
W.~Hulsbergen$^{38}$\lhcborcid{0000-0003-3018-5707},
R.J.~Hunter$^{58}$\lhcborcid{0000-0001-7894-8799},
M.~Hushchyn$^{44}$\lhcborcid{0000-0002-8894-6292},
D.~Hutchcroft$^{62}$\lhcborcid{0000-0002-4174-6509},
M.~Idzik$^{40}$\lhcborcid{0000-0001-6349-0033},
D.~Ilin$^{44}$\lhcborcid{0000-0001-8771-3115},
P.~Ilten$^{67}$\lhcborcid{0000-0001-5534-1732},
A.~Iniukhin$^{44}$\lhcborcid{0000-0002-1940-6276},
A. ~Iohner$^{10}$\lhcborcid{0009-0003-1506-7427},
A.~Ishteev$^{44}$\lhcborcid{0000-0003-1409-1428},
K.~Ivshin$^{44}$\lhcborcid{0000-0001-8403-0706},
H.~Jage$^{17}$\lhcborcid{0000-0002-8096-3792},
S.J.~Jaimes~Elles$^{78,49,50}$\lhcborcid{0000-0003-0182-8638},
S.~Jakobsen$^{50}$\lhcborcid{0000-0002-6564-040X},
T.~Jakoubek$^{79}$\lhcborcid{0000-0001-7038-0369},
E.~Jans$^{38}$\lhcborcid{0000-0002-5438-9176},
B.K.~Jashal$^{49}$\lhcborcid{0000-0002-0025-4663},
A.~Jawahery$^{68}$\lhcborcid{0000-0003-3719-119X},
C. ~Jayaweera$^{55}$\lhcborcid{ 0009-0004-2328-658X},
A. ~Jelavic$^{1}$\lhcborcid{0009-0005-0826-999X},
V.~Jevtic$^{19}$\lhcborcid{0000-0001-6427-4746},
Z. ~Jia$^{16}$\lhcborcid{0000-0002-4774-5961},
E.~Jiang$^{68}$\lhcborcid{0000-0003-1728-8525},
X.~Jiang$^{5,7}$\lhcborcid{0000-0001-8120-3296},
Y.~Jiang$^{7}$\lhcborcid{0000-0002-8964-5109},
Y. J. ~Jiang$^{6}$\lhcborcid{0000-0002-0656-8647},
E.~Jimenez~Moya$^{9}$\lhcborcid{0000-0001-7712-3197},
N. ~Jindal$^{90}$\lhcborcid{0000-0002-2092-3545},
M.~John$^{65}$\lhcborcid{0000-0002-8579-844X},
A. ~John~Rubesh~Rajan$^{23}$\lhcborcid{0000-0002-9850-4965},
D.~Johnson$^{55}$\lhcborcid{0000-0003-3272-6001},
C.R.~Jones$^{57}$\lhcborcid{0000-0003-1699-8816},
S.~Joshi$^{42}$\lhcborcid{0000-0002-5821-1674},
B.~Jost$^{50}$\lhcborcid{0009-0005-4053-1222},
J. ~Juan~Castella$^{57}$\lhcborcid{0009-0009-5577-1308},
N.~Jurik$^{50}$\lhcborcid{0000-0002-6066-7232},
I.~Juszczak$^{41}$\lhcborcid{0000-0002-1285-3911},
K. ~Kalecinska$^{40}$,
D.~Kaminaris$^{51}$\lhcborcid{0000-0002-8912-4653},
S.~Kandybei$^{53}$\lhcborcid{0000-0003-3598-0427},
M. ~Kane$^{60}$\lhcborcid{ 0009-0006-5064-966X},
Y.~Kang$^{4,d}$\lhcborcid{0000-0002-6528-8178},
C.~Kar$^{11}$\lhcborcid{0000-0002-6407-6974},
M.~Karacson$^{50}$\lhcborcid{0009-0006-1867-9674},
A.~Kauniskangas$^{51}$\lhcborcid{0000-0002-4285-8027},
J.W.~Kautz$^{67}$\lhcborcid{0000-0001-8482-5576},
M.K.~Kazanecki$^{41}$\lhcborcid{0009-0009-3480-5724},
F.~Keizer$^{50}$\lhcborcid{0000-0002-1290-6737},
M.~Kenzie$^{57}$\lhcborcid{0000-0001-7910-4109},
T.~Ketel$^{38}$\lhcborcid{0000-0002-9652-1964},
B.~Khanji$^{70}$\lhcborcid{0000-0003-3838-281X},
A.~Kharisova$^{44}$\lhcborcid{0000-0002-5291-9583},
S.~Kholodenko$^{63,50}$\lhcborcid{0000-0002-0260-6570},
G.~Khreich$^{14}$\lhcborcid{0000-0002-6520-8203},
F. ~Kiraz$^{14}$,
T.~Kirn$^{17}$\lhcborcid{0000-0002-0253-8619},
V.S.~Kirsebom$^{31,p}$\lhcborcid{0009-0005-4421-9025},
S.~Klaver$^{39}$\lhcborcid{0000-0001-7909-1272},
N.~Kleijne$^{35,t}$\lhcborcid{0000-0003-0828-0943},
A.~Kleimenova$^{51}$\lhcborcid{0000-0002-9129-4985},
D. K. ~Klekots$^{87}$\lhcborcid{0000-0002-4251-2958},
K.~Klimaszewski$^{42}$\lhcborcid{0000-0003-0741-5922},
M.R.~Kmiec$^{42}$\lhcborcid{0000-0002-1821-1848},
T. ~Knospe$^{19}$\lhcborcid{ 0009-0003-8343-3767},
R. ~Kolb$^{22}$\lhcborcid{0009-0005-5214-0202},
S.~Koliiev$^{54}$\lhcborcid{0009-0002-3680-1224},
L.~Kolk$^{19}$\lhcborcid{0000-0003-2589-5130},
A.~Konoplyannikov$^{6}$\lhcborcid{0009-0005-2645-8364},
P.~Kopciewicz$^{50}$\lhcborcid{0000-0001-9092-3527},
P.~Koppenburg$^{38}$\lhcborcid{0000-0001-8614-7203},
A. ~Korchin$^{53}$\lhcborcid{0000-0001-7947-170X},
I.~Kostiuk$^{38}$\lhcborcid{0000-0002-8767-7289},
O.~Kot$^{54}$\lhcborcid{0009-0005-5473-6050},
S.~Kotriakhova$^{}$\lhcborcid{0000-0002-1495-0053},
E. ~Kowalczyk$^{68}$\lhcborcid{0009-0006-0206-2784},
A.~Kozachuk$^{44}$\lhcborcid{0000-0001-6805-0395},
P.~Kravchenko$^{44}$\lhcborcid{0000-0002-4036-2060},
L.~Kravchuk$^{44}$\lhcborcid{0000-0001-8631-4200},
O. ~Kravcov$^{82}$\lhcborcid{0000-0001-7148-3335},
M.~Kreps$^{58}$\lhcborcid{0000-0002-6133-486X},
P.~Krokovny$^{44}$\lhcborcid{0000-0002-1236-4667},
W.~Krupa$^{70}$\lhcborcid{0000-0002-7947-465X},
W.~Krzemien$^{42}$\lhcborcid{0000-0002-9546-358X},
O.~Kshyvanskyi$^{54}$\lhcborcid{0009-0003-6637-841X},
S.~Kubis$^{85}$\lhcborcid{0000-0001-8774-8270},
M.~Kucharczyk$^{41}$\lhcborcid{0000-0003-4688-0050},
V.~Kudryavtsev$^{44}$\lhcborcid{0009-0000-2192-995X},
E.~Kulikova$^{44}$\lhcborcid{0009-0002-8059-5325},
A.~Kupsc$^{86}$\lhcborcid{0000-0003-4937-2270},
V.~Kushnir$^{53}$\lhcborcid{0000-0003-2907-1323},
B.~Kutsenko$^{13}$\lhcborcid{0000-0002-8366-1167},
J.~Kvapil$^{69}$\lhcborcid{0000-0002-0298-9073},
I. ~Kyryllin$^{53}$\lhcborcid{0000-0003-3625-7521},
D.~Lacarrere$^{50}$\lhcborcid{0009-0005-6974-140X},
P. ~Laguarta~Gonzalez$^{46}$\lhcborcid{0009-0005-3844-0778},
A.~Lai$^{32}$\lhcborcid{0000-0003-1633-0496},
A.~Lampis$^{32}$\lhcborcid{0000-0002-5443-4870},
D.~Lancierini$^{63}$\lhcborcid{0000-0003-1587-4555},
C.~Landesa~Gomez$^{48}$\lhcborcid{0000-0001-5241-8642},
J.J.~Lane$^{1}$\lhcborcid{0000-0002-5816-9488},
G.~Lanfranchi$^{28}$\lhcborcid{0000-0002-9467-8001},
C.~Langenbruch$^{22}$\lhcborcid{0000-0002-3454-7261},
J.~Langer$^{19}$\lhcborcid{0000-0002-0322-5550},
T.~Latham$^{58}$\lhcborcid{0000-0002-7195-8537},
F.~Lazzari$^{35,u}$\lhcborcid{0000-0002-3151-3453},
C.~Lazzeroni$^{55}$\lhcborcid{0000-0003-4074-4787},
R.~Le~Gac$^{13}$\lhcborcid{0000-0002-7551-6971},
H. ~Lee$^{62}$\lhcborcid{0009-0003-3006-2149},
R.~Lef{\`e}vre$^{11}$\lhcborcid{0000-0002-6917-6210},
A.~Leflat$^{44}$\lhcborcid{0000-0001-9619-6666},
S.~Legotin$^{44}$\lhcborcid{0000-0003-3192-6175},
M.~Lehuraux$^{58}$\lhcborcid{0000-0001-7600-7039},
E.~Lemos~Cid$^{50}$\lhcborcid{0000-0003-3001-6268},
O.~Leroy$^{13}$\lhcborcid{0000-0002-2589-240X},
T.~Lesiak$^{41}$\lhcborcid{0000-0002-3966-2998},
E. D.~Lesser$^{50}$\lhcborcid{0000-0001-8367-8703},
B.~Leverington$^{22}$\lhcborcid{0000-0001-6640-7274},
A.~Li$^{4,d}$\lhcborcid{0000-0001-5012-6013},
C. ~Li$^{4}$\lhcborcid{0009-0002-3366-2871},
C. ~Li$^{13}$\lhcborcid{0000-0002-3554-5479},
H.~Li$^{74}$\lhcborcid{0000-0002-2366-9554},
J.~Li$^{8}$\lhcborcid{0009-0003-8145-0643},
K.~Li$^{77}$\lhcborcid{0000-0002-2243-8412},
L.~Li$^{64}$\lhcborcid{0000-0003-4625-6880},
P.~Li$^{7}$\lhcborcid{0000-0003-2740-9765},
P.-R.~Li$^{75}$\lhcborcid{0000-0002-1603-3646},
Q. ~Li$^{5,7}$\lhcborcid{0009-0004-1932-8580},
T.~Li$^{73}$\lhcborcid{0000-0002-5241-2555},
T.~Li$^{74}$\lhcborcid{0000-0002-5723-0961},
Y.~Li$^{8}$\lhcborcid{0009-0004-0130-6121},
Y.~Li$^{5}$\lhcborcid{0000-0003-2043-4669},
Y. ~Li$^{4}$\lhcborcid{0009-0007-6670-7016},
Z.~Lian$^{4,d}$\lhcborcid{0000-0003-4602-6946},
Q. ~Liang$^{8}$,
X.~Liang$^{70}$\lhcborcid{0000-0002-5277-9103},
Z. ~Liang$^{32}$\lhcborcid{0000-0001-6027-6883},
S.~Libralon$^{49}$\lhcborcid{0009-0002-5841-9624},
A. ~Lightbody$^{12}$\lhcborcid{0009-0008-9092-582X},
C.~Lin$^{7}$\lhcborcid{0000-0001-7587-3365},
T.~Lin$^{59}$\lhcborcid{0000-0001-6052-8243},
R.~Lindner$^{50}$\lhcborcid{0000-0002-5541-6500},
H. ~Linton$^{63}$\lhcborcid{0009-0000-3693-1972},
R.~Litvinov$^{32}$\lhcborcid{0000-0002-4234-435X},
D.~Liu$^{8}$\lhcborcid{0009-0002-8107-5452},
F. L. ~Liu$^{1}$\lhcborcid{0009-0002-2387-8150},
G.~Liu$^{74}$\lhcborcid{0000-0001-5961-6588},
K.~Liu$^{75}$\lhcborcid{0000-0003-4529-3356},
S.~Liu$^{5}$\lhcborcid{0000-0002-6919-227X},
W. ~Liu$^{8}$\lhcborcid{0009-0005-0734-2753},
Y.~Liu$^{60}$\lhcborcid{0000-0003-3257-9240},
Y.~Liu$^{75}$\lhcborcid{0009-0002-0885-5145},
Y. L. ~Liu$^{63}$\lhcborcid{0000-0001-9617-6067},
G.~Loachamin~Ordonez$^{71}$\lhcborcid{0009-0001-3549-3939},
I. ~Lobo$^{1}$\lhcborcid{0009-0003-3915-4146},
A.~Lobo~Salvia$^{10}$\lhcborcid{0000-0002-2375-9509},
A.~Loi$^{32}$\lhcborcid{0000-0003-4176-1503},
T.~Long$^{57}$\lhcborcid{0000-0001-7292-848X},
F. C. L.~Lopes$^{2,a}$\lhcborcid{0009-0006-1335-3595},
J.H.~Lopes$^{3}$\lhcborcid{0000-0003-1168-9547},
A.~Lopez~Huertas$^{46}$\lhcborcid{0000-0002-6323-5582},
C. ~Lopez~Iribarnegaray$^{48}$\lhcborcid{0009-0004-3953-6694},
S.~L{\'o}pez~Soli{\~n}o$^{48}$\lhcborcid{0000-0001-9892-5113},
Q.~Lu$^{15}$\lhcborcid{0000-0002-6598-1941},
C.~Lucarelli$^{50}$\lhcborcid{0000-0002-8196-1828},
D.~Lucchesi$^{33,r}$\lhcborcid{0000-0003-4937-7637},
M.~Lucio~Martinez$^{49}$\lhcborcid{0000-0001-6823-2607},
Y.~Luo$^{6}$\lhcborcid{0009-0001-8755-2937},
A.~Lupato$^{33,j}$\lhcborcid{0000-0003-0312-3914},
E.~Luppi$^{26,m}$\lhcborcid{0000-0002-1072-5633},
K.~Lynch$^{23}$\lhcborcid{0000-0002-7053-4951},
X.-R.~Lyu$^{7}$\lhcborcid{0000-0001-5689-9578},
G. M. ~Ma$^{4,d}$\lhcborcid{0000-0001-8838-5205},
H. ~Ma$^{73}$\lhcborcid{0009-0001-0655-6494},
S.~Maccolini$^{19}$\lhcborcid{0000-0002-9571-7535},
F.~Machefert$^{14}$\lhcborcid{0000-0002-4644-5916},
F.~Maciuc$^{43}$\lhcborcid{0000-0001-6651-9436},
B. ~Mack$^{70}$\lhcborcid{0000-0001-8323-6454},
I.~Mackay$^{65}$\lhcborcid{0000-0003-0171-7890},
L. M. ~Mackey$^{70}$\lhcborcid{0000-0002-8285-3589},
L.R.~Madhan~Mohan$^{57}$\lhcborcid{0000-0002-9390-8821},
M. J. ~Madurai$^{55}$\lhcborcid{0000-0002-6503-0759},
D.~Magdalinski$^{38}$\lhcborcid{0000-0001-6267-7314},
D.~Maisuzenko$^{44}$\lhcborcid{0000-0001-5704-3499},
J.J.~Malczewski$^{41}$\lhcborcid{0000-0003-2744-3656},
S.~Malde$^{65}$\lhcborcid{0000-0002-8179-0707},
L.~Malentacca$^{50}$\lhcborcid{0000-0001-6717-2980},
A.~Malinin$^{44}$\lhcborcid{0000-0002-3731-9977},
T.~Maltsev$^{44}$\lhcborcid{0000-0002-2120-5633},
G.~Manca$^{32,l}$\lhcborcid{0000-0003-1960-4413},
G.~Mancinelli$^{13}$\lhcborcid{0000-0003-1144-3678},
C.~Mancuso$^{14}$\lhcborcid{0000-0002-2490-435X},
R.~Manera~Escalero$^{46}$\lhcborcid{0000-0003-4981-6847},
F. M. ~Manganella$^{37}$\lhcborcid{0009-0003-1124-0974},
D.~Manuzzi$^{25}$\lhcborcid{0000-0002-9915-6587},
D.~Marangotto$^{30,o}$\lhcborcid{0000-0001-9099-4878},
J.F.~Marchand$^{10}$\lhcborcid{0000-0002-4111-0797},
R.~Marchevski$^{51}$\lhcborcid{0000-0003-3410-0918},
U.~Marconi$^{25}$\lhcborcid{0000-0002-5055-7224},
E.~Mariani$^{16}$\lhcborcid{0009-0002-3683-2709},
S.~Mariani$^{50}$\lhcborcid{0000-0002-7298-3101},
C.~Marin~Benito$^{46}$\lhcborcid{0000-0003-0529-6982},
J.~Marks$^{22}$\lhcborcid{0000-0002-2867-722X},
A.M.~Marshall$^{56}$\lhcborcid{0000-0002-9863-4954},
L. ~Martel$^{65}$\lhcborcid{0000-0001-8562-0038},
G.~Martelli$^{34}$\lhcborcid{0000-0002-6150-3168},
G.~Martellotti$^{36}$\lhcborcid{0000-0002-8663-9037},
L.~Martinazzoli$^{50}$\lhcborcid{0000-0002-8996-795X},
M.~Martinelli$^{31,p}$\lhcborcid{0000-0003-4792-9178},
D. ~Martinez~Gomez$^{83}$\lhcborcid{0009-0001-2684-9139},
D.~Martinez~Santos$^{45}$\lhcborcid{0000-0002-6438-4483},
F.~Martinez~Vidal$^{49}$\lhcborcid{0000-0001-6841-6035},
A. ~Martorell~i~Granollers$^{47}$\lhcborcid{0009-0005-6982-9006},
A.~Massafferri$^{2}$\lhcborcid{0000-0002-3264-3401},
R.~Matev$^{50}$\lhcborcid{0000-0001-8713-6119},
A.~Mathad$^{50}$\lhcborcid{0000-0002-9428-4715},
V.~Matiunin$^{44}$\lhcborcid{0000-0003-4665-5451},
C.~Matteuzzi$^{70}$\lhcborcid{0000-0002-4047-4521},
K.R.~Mattioli$^{15}$\lhcborcid{0000-0003-2222-7727},
A.~Mauri$^{63}$\lhcborcid{0000-0003-1664-8963},
E.~Maurice$^{15}$\lhcborcid{0000-0002-7366-4364},
J.~Mauricio$^{46}$\lhcborcid{0000-0002-9331-1363},
P.~Mayencourt$^{51}$\lhcborcid{0000-0002-8210-1256},
J.~Mazorra~de~Cos$^{49}$\lhcborcid{0000-0003-0525-2736},
M.~Mazurek$^{42}$\lhcborcid{0000-0002-3687-9630},
D. ~Mazzanti~Tarancon$^{46}$\lhcborcid{0009-0003-9319-777X},
M.~McCann$^{63}$\lhcborcid{0000-0002-3038-7301},
N.T.~McHugh$^{61}$\lhcborcid{0000-0002-5477-3995},
A.~McNab$^{64}$\lhcborcid{0000-0001-5023-2086},
R.~McNulty$^{23}$\lhcborcid{0000-0001-7144-0175},
B.~Meadows$^{67}$\lhcborcid{0000-0002-1947-8034},
D.~Melnychuk$^{42}$\lhcborcid{0000-0003-1667-7115},
D.~Mendoza~Granada$^{16}$\lhcborcid{0000-0002-6459-5408},
P. ~Menendez~Valdes~Perez$^{48}$\lhcborcid{0009-0003-0406-8141},
F. M. ~Meng$^{4,d}$\lhcborcid{0009-0004-1533-6014},
M.~Merk$^{38,84}$\lhcborcid{0000-0003-0818-4695},
A.~Merli$^{51,30}$\lhcborcid{0000-0002-0374-5310},
L.~Meyer~Garcia$^{68}$\lhcborcid{0000-0002-2622-8551},
D.~Miao$^{5,7}$\lhcborcid{0000-0003-4232-5615},
H.~Miao$^{7}$\lhcborcid{0000-0002-1936-5400},
M.~Mikhasenko$^{80}$\lhcborcid{0000-0002-6969-2063},
D.A.~Milanes$^{78,x}$\lhcborcid{0000-0001-7450-1121},
A.~Minotti$^{31,p}$\lhcborcid{0000-0002-0091-5177},
E.~Minucci$^{28}$\lhcborcid{0000-0002-3972-6824},
T.~Miralles$^{11}$\lhcborcid{0000-0002-4018-1454},
B.~Mitreska$^{64}$\lhcborcid{0000-0002-1697-4999},
D.S.~Mitzel$^{19}$\lhcborcid{0000-0003-3650-2689},
R. ~Mocanu$^{43}$\lhcborcid{0009-0005-5391-7255},
A.~Modak$^{59}$\lhcborcid{0000-0003-1198-1441},
L.~Moeser$^{19}$\lhcborcid{0009-0007-2494-8241},
R.D.~Moise$^{17}$\lhcborcid{0000-0002-5662-8804},
E. F.~Molina~Cardenas$^{88}$\lhcborcid{0009-0002-0674-5305},
T.~Momb{\"a}cher$^{67}$\lhcborcid{0000-0002-5612-979X},
M.~Monk$^{57}$\lhcborcid{0000-0003-0484-0157},
T.~Monnard$^{51}$\lhcborcid{0009-0005-7171-7775},
S.~Monteil$^{11}$\lhcborcid{0000-0001-5015-3353},
A.~Morcillo~Gomez$^{48}$\lhcborcid{0000-0001-9165-7080},
G.~Morello$^{28}$\lhcborcid{0000-0002-6180-3697},
M.J.~Morello$^{35,t}$\lhcborcid{0000-0003-4190-1078},
M.P.~Morgenthaler$^{22}$\lhcborcid{0000-0002-7699-5724},
A. ~Moro$^{31,p}$\lhcborcid{0009-0007-8141-2486},
J.~Moron$^{40}$\lhcborcid{0000-0002-1857-1675},
W. ~Morren$^{38}$\lhcborcid{0009-0004-1863-9344},
A.B.~Morris$^{82,50}$\lhcborcid{0000-0002-0832-9199},
A.G.~Morris$^{13}$\lhcborcid{0000-0001-6644-9888},
R.~Mountain$^{70}$\lhcborcid{0000-0003-1908-4219},
Z. M. ~Mu$^{6}$\lhcborcid{0000-0001-9291-2231},
E.~Muhammad$^{58}$\lhcborcid{0000-0001-7413-5862},
F.~Muheim$^{60}$\lhcborcid{0000-0002-1131-8909},
M.~Mulder$^{38}$\lhcborcid{0000-0001-6867-8166},
K.~M{\"u}ller$^{52}$\lhcborcid{0000-0002-5105-1305},
F.~Mu{\~n}oz-Rojas$^{9}$\lhcborcid{0000-0002-4978-602X},
V. ~Mytrochenko$^{53}$\lhcborcid{ 0000-0002-3002-7402},
P.~Naik$^{62}$\lhcborcid{0000-0001-6977-2971},
T.~Nakada$^{51}$\lhcborcid{0009-0000-6210-6861},
R.~Nandakumar$^{59}$\lhcborcid{0000-0002-6813-6794},
G. ~Napoletano$^{51}$\lhcborcid{0009-0008-9225-8653},
I.~Nasteva$^{3}$\lhcborcid{0000-0001-7115-7214},
M.~Needham$^{60}$\lhcborcid{0000-0002-8297-6714},
E. ~Nekrasova$^{44}$\lhcborcid{0009-0009-5725-2405},
N.~Neri$^{30,o}$\lhcborcid{0000-0002-6106-3756},
S.~Neubert$^{18}$\lhcborcid{0000-0002-0706-1944},
N.~Neufeld$^{50}$\lhcborcid{0000-0003-2298-0102},
P.~Neustroev$^{44}$,
J.~Nicolini$^{50}$\lhcborcid{0000-0001-9034-3637},
D.~Nicotra$^{84}$\lhcborcid{0000-0001-7513-3033},
E.M.~Niel$^{15}$\lhcborcid{0000-0002-6587-4695},
N.~Nikitin$^{44}$\lhcborcid{0000-0003-0215-1091},
L. ~Nisi$^{19}$\lhcborcid{0009-0006-8445-8968},
Q.~Niu$^{75}$\lhcborcid{0009-0004-3290-2444},
B. K.~Njoki$^{50}$\lhcborcid{0000-0002-5321-4227},
P.~Nogarolli$^{3}$\lhcborcid{0009-0001-4635-1055},
P.~Nogga$^{18}$\lhcborcid{0009-0006-2269-4666},
C.~Normand$^{48}$\lhcborcid{0000-0001-5055-7710},
J.~Novoa~Fernandez$^{48}$\lhcborcid{0000-0002-1819-1381},
G.~Nowak$^{67}$\lhcborcid{0000-0003-4864-7164},
C.~Nunez$^{88}$\lhcborcid{0000-0002-2521-9346},
H. N. ~Nur$^{61}$\lhcborcid{0000-0002-7822-523X},
A.~Oblakowska-Mucha$^{40}$\lhcborcid{0000-0003-1328-0534},
V.~Obraztsov$^{44}$\lhcborcid{0000-0002-0994-3641},
T.~Oeser$^{17}$\lhcborcid{0000-0001-7792-4082},
A.~Okhotnikov$^{44}$,
O.~Okhrimenko$^{54}$\lhcborcid{0000-0002-0657-6962},
R.~Oldeman$^{32,l}$\lhcborcid{0000-0001-6902-0710},
F.~Oliva$^{60,50}$\lhcborcid{0000-0001-7025-3407},
E. ~Olivart~Pino$^{46}$\lhcborcid{0009-0001-9398-8614},
M.~Olocco$^{19}$\lhcborcid{0000-0002-6968-1217},
R.H.~O'Neil$^{50}$\lhcborcid{0000-0002-9797-8464},
J.S.~Ordonez~Soto$^{11}$\lhcborcid{0009-0009-0613-4871},
D.~Osthues$^{19}$\lhcborcid{0009-0004-8234-513X},
J.M.~Otalora~Goicochea$^{3}$\lhcborcid{0000-0002-9584-8500},
P.~Owen$^{52}$\lhcborcid{0000-0002-4161-9147},
A.~Oyanguren$^{49}$\lhcborcid{0000-0002-8240-7300},
O.~Ozcelik$^{50}$\lhcborcid{0000-0003-3227-9248},
F.~Paciolla$^{35,v}$\lhcborcid{0000-0002-6001-600X},
A. ~Padee$^{42}$\lhcborcid{0000-0002-5017-7168},
K.O.~Padeken$^{18}$\lhcborcid{0000-0001-7251-9125},
B.~Pagare$^{48}$\lhcborcid{0000-0003-3184-1622},
T.~Pajero$^{50}$\lhcborcid{0000-0001-9630-2000},
A.~Palano$^{24}$\lhcborcid{0000-0002-6095-9593},
L. ~Palini$^{30}$\lhcborcid{0009-0004-4010-2172},
M.~Palutan$^{28}$\lhcborcid{0000-0001-7052-1360},
C. ~Pan$^{76}$\lhcborcid{0009-0009-9985-9950},
X. ~Pan$^{4,d}$\lhcborcid{0000-0002-7439-6621},
S.~Panebianco$^{12}$\lhcborcid{0000-0002-0343-2082},
S.~Paniskaki$^{50,33}$\lhcborcid{0009-0004-4947-954X},
G.~Panshin$^{5}$\lhcborcid{0000-0001-9163-2051},
L.~Paolucci$^{64}$\lhcborcid{0000-0003-0465-2893},
A.~Papanestis$^{59}$\lhcborcid{0000-0002-5405-2901},
M.~Pappagallo$^{24,i}$\lhcborcid{0000-0001-7601-5602},
L.L.~Pappalardo$^{26}$\lhcborcid{0000-0002-0876-3163},
C.~Pappenheimer$^{67}$\lhcborcid{0000-0003-0738-3668},
C.~Parkes$^{64}$\lhcborcid{0000-0003-4174-1334},
D. ~Parmar$^{80}$\lhcborcid{0009-0004-8530-7630},
G.~Passaleva$^{27}$\lhcborcid{0000-0002-8077-8378},
D.~Passaro$^{35,t}$\lhcborcid{0000-0002-8601-2197},
A.~Pastore$^{24}$\lhcborcid{0000-0002-5024-3495},
M.~Patel$^{63}$\lhcborcid{0000-0003-3871-5602},
J.~Patoc$^{65}$\lhcborcid{0009-0000-1201-4918},
C.~Patrignani$^{25,k}$\lhcborcid{0000-0002-5882-1747},
A. ~Paul$^{70}$\lhcborcid{0009-0006-7202-0811},
C.J.~Pawley$^{84}$\lhcborcid{0000-0001-9112-3724},
A.~Pellegrino$^{38}$\lhcborcid{0000-0002-7884-345X},
J. ~Peng$^{5,7}$\lhcborcid{0009-0005-4236-4667},
X. ~Peng$^{75}$,
M.~Pepe~Altarelli$^{28}$\lhcborcid{0000-0002-1642-4030},
S.~Perazzini$^{25}$\lhcborcid{0000-0002-1862-7122},
D.~Pereima$^{44}$\lhcborcid{0000-0002-7008-8082},
H. ~Pereira~Da~Costa$^{69}$\lhcborcid{0000-0002-3863-352X},
M. ~Pereira~Martinez$^{48}$\lhcborcid{0009-0006-8577-9560},
A.~Pereiro~Castro$^{48}$\lhcborcid{0000-0001-9721-3325},
C. ~Perez$^{47}$\lhcborcid{0000-0002-6861-2674},
P.~Perret$^{11}$\lhcborcid{0000-0002-5732-4343},
A. ~Perrevoort$^{83}$\lhcborcid{0000-0001-6343-447X},
A.~Perro$^{50}$\lhcborcid{0000-0002-1996-0496},
M.J.~Peters$^{67}$\lhcborcid{0009-0008-9089-1287},
K.~Petridis$^{56}$\lhcborcid{0000-0001-7871-5119},
A.~Petrolini$^{29,n}$\lhcborcid{0000-0003-0222-7594},
S. ~Pezzulo$^{29,n}$\lhcborcid{0009-0004-4119-4881},
J. P. ~Pfaller$^{67}$\lhcborcid{0009-0009-8578-3078},
H.~Pham$^{70}$\lhcborcid{0000-0003-2995-1953},
L.~Pica$^{35,t}$\lhcborcid{0000-0001-9837-6556},
M.~Piccini$^{34}$\lhcborcid{0000-0001-8659-4409},
L. ~Piccolo$^{32}$\lhcborcid{0000-0003-1896-2892},
B.~Pietrzyk$^{10}$\lhcborcid{0000-0003-1836-7233},
G.~Pietrzyk$^{14}$\lhcborcid{0000-0001-9622-820X},
R. N.~Pilato$^{62}$\lhcborcid{0000-0002-4325-7530},
D.~Pinci$^{36}$\lhcborcid{0000-0002-7224-9708},
F.~Pisani$^{50}$\lhcborcid{0000-0002-7763-252X},
M.~Pizzichemi$^{31,p,50}$\lhcborcid{0000-0001-5189-230X},
V. M.~Placinta$^{43}$\lhcborcid{0000-0003-4465-2441},
M.~Plo~Casasus$^{48}$\lhcborcid{0000-0002-2289-918X},
T.~Poeschl$^{50}$\lhcborcid{0000-0003-3754-7221},
F.~Polci$^{16}$\lhcborcid{0000-0001-8058-0436},
M.~Poli~Lener$^{28}$\lhcborcid{0000-0001-7867-1232},
A.~Poluektov$^{13}$\lhcborcid{0000-0003-2222-9925},
N.~Polukhina$^{44}$\lhcborcid{0000-0001-5942-1772},
I.~Polyakov$^{64}$\lhcborcid{0000-0002-6855-7783},
E.~Polycarpo$^{3}$\lhcborcid{0000-0002-4298-5309},
S.~Ponce$^{50}$\lhcborcid{0000-0002-1476-7056},
D.~Popov$^{7,50}$\lhcborcid{0000-0002-8293-2922},
K.~Popp$^{19}$\lhcborcid{0009-0002-6372-2767},
S.~Poslavskii$^{44}$\lhcborcid{0000-0003-3236-1452},
K.~Prasanth$^{60}$\lhcborcid{0000-0001-9923-0938},
C.~Prouve$^{45}$\lhcborcid{0000-0003-2000-6306},
D.~Provenzano$^{32,l,50}$\lhcborcid{0009-0005-9992-9761},
V.~Pugatch$^{54}$\lhcborcid{0000-0002-5204-9821},
A. ~Puicercus~Gomez$^{50}$\lhcborcid{0009-0005-9982-6383},
G.~Punzi$^{35,u}$\lhcborcid{0000-0002-8346-9052},
J.R.~Pybus$^{69}$\lhcborcid{0000-0001-8951-2317},
Q. Q. ~Qian$^{6}$\lhcborcid{0000-0001-6453-4691},
W.~Qian$^{7}$\lhcborcid{0000-0003-3932-7556},
N.~Qin$^{4,d}$\lhcborcid{0000-0001-8453-658X},
R.~Quagliani$^{50}$\lhcborcid{0000-0002-3632-2453},
R.I.~Rabadan~Trejo$^{58}$\lhcborcid{0000-0002-9787-3910},
R. ~Racz$^{82}$\lhcborcid{0009-0003-3834-8184},
J.H.~Rademacker$^{56}$\lhcborcid{0000-0003-2599-7209},
M.~Rama$^{35}$\lhcborcid{0000-0003-3002-4719},
M. ~Ram\'{i}rez~Garc\'{i}a$^{88}$\lhcborcid{0000-0001-7956-763X},
V.~Ramos~De~Oliveira$^{71}$\lhcborcid{0000-0003-3049-7866},
M.~Ramos~Pernas$^{58}$\lhcborcid{0000-0003-1600-9432},
M.S.~Rangel$^{3}$\lhcborcid{0000-0002-8690-5198},
F.~Ratnikov$^{44}$\lhcborcid{0000-0003-0762-5583},
G.~Raven$^{39}$\lhcborcid{0000-0002-2897-5323},
M.~Rebollo~De~Miguel$^{49}$\lhcborcid{0000-0002-4522-4863},
F.~Redi$^{30,j}$\lhcborcid{0000-0001-9728-8984},
J.~Reich$^{56}$\lhcborcid{0000-0002-2657-4040},
F.~Reiss$^{20}$\lhcborcid{0000-0002-8395-7654},
Z.~Ren$^{7}$\lhcborcid{0000-0001-9974-9350},
P.K.~Resmi$^{65}$\lhcborcid{0000-0001-9025-2225},
M. ~Ribalda~Galvez$^{46}$\lhcborcid{0009-0006-0309-7639},
R.~Ribatti$^{51}$\lhcborcid{0000-0003-1778-1213},
G.~Ricart$^{12}$\lhcborcid{0000-0002-9292-2066},
D.~Riccardi$^{35,t}$\lhcborcid{0009-0009-8397-572X},
S.~Ricciardi$^{59}$\lhcborcid{0000-0002-4254-3658},
K.~Richardson$^{66}$\lhcborcid{0000-0002-6847-2835},
M.~Richardson-Slipper$^{57}$\lhcborcid{0000-0002-2752-001X},
F. ~Riehn$^{19}$\lhcborcid{ 0000-0001-8434-7500},
K.~Rinnert$^{62}$\lhcborcid{0000-0001-9802-1122},
P.~Robbe$^{14,50}$\lhcborcid{0000-0002-0656-9033},
G.~Robertson$^{61}$\lhcborcid{0000-0002-7026-1383},
E.~Rodrigues$^{62}$\lhcborcid{0000-0003-2846-7625},
A.~Rodriguez~Alvarez$^{46}$\lhcborcid{0009-0006-1758-936X},
E.~Rodriguez~Fernandez$^{48}$\lhcborcid{0000-0002-3040-065X},
J.A.~Rodriguez~Lopez$^{78}$\lhcborcid{0000-0003-1895-9319},
E.~Rodriguez~Rodriguez$^{50}$\lhcborcid{0000-0002-7973-8061},
J.~Roensch$^{19}$\lhcborcid{0009-0001-7628-6063},
A.~Rogachev$^{44}$\lhcborcid{0000-0002-7548-6530},
A.~Rogovskiy$^{59}$\lhcborcid{0000-0002-1034-1058},
D.L.~Rolf$^{19}$\lhcborcid{0000-0001-7908-7214},
P.~Roloff$^{50}$\lhcborcid{0000-0001-7378-4350},
V.~Romanovskiy$^{67}$\lhcborcid{0000-0003-0939-4272},
A.~Romero~Vidal$^{48}$\lhcborcid{0000-0002-8830-1486},
G.~Romolini$^{26,50}$\lhcborcid{0000-0002-0118-4214},
F.~Ronchetti$^{51}$\lhcborcid{0000-0003-3438-9774},
T.~Rong$^{6}$\lhcborcid{0000-0002-5479-9212},
M.~Rotondo$^{28}$\lhcborcid{0000-0001-5704-6163},
M.S.~Rudolph$^{70}$\lhcborcid{0000-0002-0050-575X},
M.~Ruiz~Diaz$^{22}$\lhcborcid{0000-0001-6367-6815},
R.A.~Ruiz~Fernandez$^{48}$\lhcborcid{0000-0002-5727-4454},
J.~Ruiz~Vidal$^{84}$\lhcborcid{0000-0001-8362-7164},
J. J.~Saavedra-Arias$^{9}$\lhcborcid{0000-0002-2510-8929},
J.J.~Saborido~Silva$^{48}$\lhcborcid{0000-0002-6270-130X},
S. E. R.~Sacha~Emile~R.$^{50}$\lhcborcid{0000-0002-1432-2858},
N.~Sagidova$^{44}$\lhcborcid{0000-0002-2640-3794},
D.~Sahoo$^{81}$\lhcborcid{0000-0002-5600-9413},
N.~Sahoo$^{55}$\lhcborcid{0000-0001-9539-8370},
B.~Saitta$^{32}$\lhcborcid{0000-0003-3491-0232},
M.~Salomoni$^{31,50,p}$\lhcborcid{0009-0007-9229-653X},
I.~Sanderswood$^{49}$\lhcborcid{0000-0001-7731-6757},
R.~Santacesaria$^{36}$\lhcborcid{0000-0003-3826-0329},
C.~Santamarina~Rios$^{48}$\lhcborcid{0000-0002-9810-1816},
M.~Santimaria$^{28}$\lhcborcid{0000-0002-8776-6759},
L.~Santoro~$^{2}$\lhcborcid{0000-0002-2146-2648},
E.~Santovetti$^{37}$\lhcborcid{0000-0002-5605-1662},
A.~Saputi$^{26,50}$\lhcborcid{0000-0001-6067-7863},
D.~Saranin$^{44}$\lhcborcid{0000-0002-9617-9986},
A.~Sarnatskiy$^{83}$\lhcborcid{0009-0007-2159-3633},
G.~Sarpis$^{50}$\lhcborcid{0000-0003-1711-2044},
M.~Sarpis$^{82}$\lhcborcid{0000-0002-6402-1674},
C.~Satriano$^{36}$\lhcborcid{0000-0002-4976-0460},
A.~Satta$^{37}$\lhcborcid{0000-0003-2462-913X},
M.~Saur$^{75}$\lhcborcid{0000-0001-8752-4293},
D.~Savrina$^{44}$\lhcborcid{0000-0001-8372-6031},
H.~Sazak$^{17}$\lhcborcid{0000-0003-2689-1123},
F.~Sborzacchi$^{50,28}$\lhcborcid{0009-0004-7916-2682},
A.~Scarabotto$^{19}$\lhcborcid{0000-0003-2290-9672},
S.~Schael$^{17}$\lhcborcid{0000-0003-4013-3468},
S.~Scherl$^{62}$\lhcborcid{0000-0003-0528-2724},
M.~Schiller$^{22}$\lhcborcid{0000-0001-8750-863X},
H.~Schindler$^{50}$\lhcborcid{0000-0002-1468-0479},
M.~Schmelling$^{21}$\lhcborcid{0000-0003-3305-0576},
B.~Schmidt$^{50}$\lhcborcid{0000-0002-8400-1566},
N.~Schmidt$^{69}$\lhcborcid{0000-0002-5795-4871},
S.~Schmitt$^{66}$\lhcborcid{0000-0002-6394-1081},
H.~Schmitz$^{18}$,
O.~Schneider$^{51}$\lhcborcid{0000-0002-6014-7552},
A.~Schopper$^{63}$\lhcborcid{0000-0002-8581-3312},
N.~Schulte$^{19}$\lhcborcid{0000-0003-0166-2105},
M.H.~Schune$^{14}$\lhcborcid{0000-0002-3648-0830},
G.~Schwering$^{17}$\lhcborcid{0000-0003-1731-7939},
B.~Sciascia$^{28}$\lhcborcid{0000-0003-0670-006X},
A.~Sciuccati$^{50}$\lhcborcid{0000-0002-8568-1487},
G. ~Scriven$^{84}$\lhcborcid{0009-0004-9997-1647},
I.~Segal$^{80}$\lhcborcid{0000-0001-8605-3020},
S.~Sellam$^{48}$\lhcborcid{0000-0003-0383-1451},
A.~Semennikov$^{44}$\lhcborcid{0000-0003-1130-2197},
T.~Senger$^{52}$\lhcborcid{0009-0006-2212-6431},
M.~Senghi~Soares$^{39}$\lhcborcid{0000-0001-9676-6059},
A.~Sergi$^{29,n}$\lhcborcid{0000-0001-9495-6115},
N.~Serra$^{52}$\lhcborcid{0000-0002-5033-0580},
L.~Sestini$^{27}$\lhcborcid{0000-0002-1127-5144},
B. ~Sevilla~Sanjuan$^{47}$\lhcborcid{0009-0002-5108-4112},
Y.~Shang$^{6}$\lhcborcid{0000-0001-7987-7558},
D.M.~Shangase$^{88}$\lhcborcid{0000-0002-0287-6124},
M.~Shapkin$^{44}$\lhcborcid{0000-0002-4098-9592},
R. S. ~Sharma$^{70}$\lhcborcid{0000-0003-1331-1791},
I.~Shchemerov$^{44}$\lhcborcid{0000-0001-9193-8106},
L.~Shchutska$^{51}$\lhcborcid{0000-0003-0700-5448},
T.~Shears$^{62}$\lhcborcid{0000-0002-2653-1366},
L.~Shekhtman$^{44}$\lhcborcid{0000-0003-1512-9715},
Z.~Shen$^{38}$\lhcborcid{0000-0003-1391-5384},
S.~Sheng$^{51}$\lhcborcid{0000-0002-1050-5649},
V.~Shevchenko$^{44}$\lhcborcid{0000-0003-3171-9125},
B.~Shi$^{7}$\lhcborcid{0000-0002-5781-8933},
J. ~Shi$^{57}$\lhcborcid{0000-0001-5108-6957},
Q.~Shi$^{7}$\lhcborcid{0000-0001-7915-8211},
W. S. ~Shi$^{74}$\lhcborcid{0009-0003-4186-9191},
Y.~Shimizu$^{14}$\lhcborcid{0000-0002-4936-1152},
E.~Shmanin$^{25}$\lhcborcid{0000-0002-8868-1730},
R.~Shorkin$^{44}$\lhcborcid{0000-0001-8881-3943},
R.~Silva~Coutinho$^{2}$\lhcborcid{0000-0002-1545-959X},
G.~Simi$^{33,r}$\lhcborcid{0000-0001-6741-6199},
S.~Simone$^{24,i}$\lhcborcid{0000-0003-3631-8398},
M. ~Singha$^{81}$\lhcborcid{0009-0005-1271-972X},
I.~Siral$^{51}$\lhcborcid{0000-0003-4554-1831},
N.~Skidmore$^{58}$\lhcborcid{0000-0003-3410-0731},
T.~Skwarnicki$^{70}$\lhcborcid{0000-0002-9897-9506},
M.W.~Slater$^{55}$\lhcborcid{0000-0002-2687-1950},
E.~Smith$^{66}$\lhcborcid{0000-0002-9740-0574},
M.~Smith$^{63}$\lhcborcid{0000-0002-3872-1917},
L.~Soares~Lavra$^{60}$\lhcborcid{0000-0002-2652-123X},
M.D.~Sokoloff$^{67}$\lhcborcid{0000-0001-6181-4583},
F.J.P.~Soler$^{61}$\lhcborcid{0000-0002-4893-3729},
A.~Solomin$^{56}$\lhcborcid{0000-0003-0644-3227},
A.~Solovev$^{44}$\lhcborcid{0000-0002-5355-5996},
K. ~Solovieva$^{20}$\lhcborcid{0000-0003-2168-9137},
N. S. ~Sommerfeld$^{18}$\lhcborcid{0009-0006-7822-2860},
R.~Song$^{1}$\lhcborcid{0000-0002-8854-8905},
Y.~Song$^{51}$\lhcborcid{0000-0003-0256-4320},
Y.~Song$^{4,d}$\lhcborcid{0000-0003-1959-5676},
Y. S. ~Song$^{6}$\lhcborcid{0000-0003-3471-1751},
F.L.~Souza~De~Almeida$^{46}$\lhcborcid{0000-0001-7181-6785},
B.~Souza~De~Paula$^{3}$\lhcborcid{0009-0003-3794-3408},
K.M.~Sowa$^{40}$\lhcborcid{0000-0001-6961-536X},
E.~Spadaro~Norella$^{29,n}$\lhcborcid{0000-0002-1111-5597},
E.~Spedicato$^{25}$\lhcborcid{0000-0002-4950-6665},
J.G.~Speer$^{19}$\lhcborcid{0000-0002-6117-7307},
P.~Spradlin$^{61}$\lhcborcid{0000-0002-5280-9464},
F.~Stagni$^{50}$\lhcborcid{0000-0002-7576-4019},
M.~Stahl$^{80}$\lhcborcid{0000-0001-8476-8188},
S.~Stahl$^{50}$\lhcborcid{0000-0002-8243-400X},
S.~Stanislaus$^{65}$\lhcborcid{0000-0003-1776-0498},
M. ~Stefaniak$^{90}$\lhcborcid{0000-0002-5820-1054},
O.~Steinkamp$^{52}$\lhcborcid{0000-0001-7055-6467},
D.~Strekalina$^{44}$\lhcborcid{0000-0003-3830-4889},
Y.~Su$^{7}$\lhcborcid{0000-0002-2739-7453},
F.~Suljik$^{65}$\lhcborcid{0000-0001-6767-7698},
J.~Sun$^{32}$\lhcborcid{0000-0002-6020-2304},
J. ~Sun$^{64}$\lhcborcid{0009-0008-7253-1237},
L.~Sun$^{76}$\lhcborcid{0000-0002-0034-2567},
D.~Sundfeld$^{2}$\lhcborcid{0000-0002-5147-3698},
W.~Sutcliffe$^{52}$\lhcborcid{0000-0002-9795-3582},
P.~Svihra$^{79}$\lhcborcid{0000-0002-7811-2147},
V.~Svintozelskyi$^{49}$\lhcborcid{0000-0002-0798-5864},
K.~Swientek$^{40}$\lhcborcid{0000-0001-6086-4116},
F.~Swystun$^{57}$\lhcborcid{0009-0006-0672-7771},
A.~Szabelski$^{42}$\lhcborcid{0000-0002-6604-2938},
T.~Szumlak$^{40}$\lhcborcid{0000-0002-2562-7163},
Y.~Tan$^{4}$\lhcborcid{0000-0003-3860-6545},
Y.~Tang$^{76}$\lhcborcid{0000-0002-6558-6730},
Y. T. ~Tang$^{7}$\lhcborcid{0009-0003-9742-3949},
M.D.~Tat$^{22}$\lhcborcid{0000-0002-6866-7085},
J. A.~Teijeiro~Jimenez$^{48}$\lhcborcid{0009-0004-1845-0621},
A.~Terentev$^{44}$\lhcborcid{0000-0003-2574-8560},
F.~Terzuoli$^{35,v}$\lhcborcid{0000-0002-9717-225X},
F.~Teubert$^{50}$\lhcborcid{0000-0003-3277-5268},
E.~Thomas$^{50}$\lhcborcid{0000-0003-0984-7593},
D.J.D.~Thompson$^{55}$\lhcborcid{0000-0003-1196-5943},
A. R. ~Thomson-Strong$^{60}$\lhcborcid{0009-0000-4050-6493},
H.~Tilquin$^{63}$\lhcborcid{0000-0003-4735-2014},
V.~Tisserand$^{11}$\lhcborcid{0000-0003-4916-0446},
S.~T'Jampens$^{10}$\lhcborcid{0000-0003-4249-6641},
M.~Tobin$^{5,50}$\lhcborcid{0000-0002-2047-7020},
T. T. ~Todorov$^{20}$\lhcborcid{0009-0002-0904-4985},
L.~Tomassetti$^{26,m}$\lhcborcid{0000-0003-4184-1335},
G.~Tonani$^{30}$\lhcborcid{0000-0001-7477-1148},
X.~Tong$^{6}$\lhcborcid{0000-0002-5278-1203},
T.~Tork$^{30}$\lhcborcid{0000-0001-9753-329X},
L.~Toscano$^{19}$\lhcborcid{0009-0007-5613-6520},
D.Y.~Tou$^{4,d}$\lhcborcid{0000-0002-4732-2408},
C.~Trippl$^{47}$\lhcborcid{0000-0003-3664-1240},
G.~Tuci$^{22}$\lhcborcid{0000-0002-0364-5758},
N.~Tuning$^{38}$\lhcborcid{0000-0003-2611-7840},
L.H.~Uecker$^{22}$\lhcborcid{0000-0003-3255-9514},
A.~Ukleja$^{40}$\lhcborcid{0000-0003-0480-4850},
D.J.~Unverzagt$^{22}$\lhcborcid{0000-0002-1484-2546},
A. ~Upadhyay$^{50}$\lhcborcid{0009-0000-6052-6889},
B. ~Urbach$^{60}$\lhcborcid{0009-0001-4404-561X},
A.~Usachov$^{38}$\lhcborcid{0000-0002-5829-6284},
A.~Ustyuzhanin$^{44}$\lhcborcid{0000-0001-7865-2357},
U.~Uwer$^{22}$\lhcborcid{0000-0002-8514-3777},
V.~Vagnoni$^{25,50}$\lhcborcid{0000-0003-2206-311X},
A. ~Vaitkevicius$^{82}$\lhcborcid{0000-0003-3625-198X},
V. ~Valcarce~Cadenas$^{48}$\lhcborcid{0009-0006-3241-8964},
G.~Valenti$^{25}$\lhcborcid{0000-0002-6119-7535},
N.~Valls~Canudas$^{50}$\lhcborcid{0000-0001-8748-8448},
J.~van~Eldik$^{50}$\lhcborcid{0000-0002-3221-7664},
H.~Van~Hecke$^{69}$\lhcborcid{0000-0001-7961-7190},
E.~van~Herwijnen$^{63}$\lhcborcid{0000-0001-8807-8811},
C.B.~Van~Hulse$^{48,y}$\lhcborcid{0000-0002-5397-6782},
R.~Van~Laak$^{51}$\lhcborcid{0000-0002-7738-6066},
M.~van~Veghel$^{84}$\lhcborcid{0000-0001-6178-6623},
G.~Vasquez$^{52}$\lhcborcid{0000-0002-3285-7004},
R.~Vazquez~Gomez$^{46}$\lhcborcid{0000-0001-5319-1128},
P.~Vazquez~Regueiro$^{48}$\lhcborcid{0000-0002-0767-9736},
C.~V{\'a}zquez~Sierra$^{45}$\lhcborcid{0000-0002-5865-0677},
S.~Vecchi$^{26}$\lhcborcid{0000-0002-4311-3166},
J. ~Velilla~Serna$^{49}$\lhcborcid{0009-0006-9218-6632},
J.J.~Velthuis$^{56}$\lhcborcid{0000-0002-4649-3221},
M.~Veltri$^{27,w}$\lhcborcid{0000-0001-7917-9661},
A.~Venkateswaran$^{51}$\lhcborcid{0000-0001-6950-1477},
M.~Verdoglia$^{32}$\lhcborcid{0009-0006-3864-8365},
M.~Vesterinen$^{58}$\lhcborcid{0000-0001-7717-2765},
W.~Vetens$^{70}$\lhcborcid{0000-0003-1058-1163},
D. ~Vico~Benet$^{65}$\lhcborcid{0009-0009-3494-2825},
P. ~Vidrier~Villalba$^{46}$\lhcborcid{0009-0005-5503-8334},
M.~Vieites~Diaz$^{48}$\lhcborcid{0000-0002-0944-4340},
X.~Vilasis-Cardona$^{47}$\lhcborcid{0000-0002-1915-9543},
E.~Vilella~Figueras$^{62}$\lhcborcid{0000-0002-7865-2856},
A.~Villa$^{25}$\lhcborcid{0000-0002-9392-6157},
P.~Vincent$^{16}$\lhcborcid{0000-0002-9283-4541},
B.~Vivacqua$^{3}$\lhcborcid{0000-0003-2265-3056},
F.C.~Volle$^{55}$\lhcborcid{0000-0003-1828-3881},
D.~vom~Bruch$^{13}$\lhcborcid{0000-0001-9905-8031},
N.~Voropaev$^{44}$\lhcborcid{0000-0002-2100-0726},
K.~Vos$^{84}$\lhcborcid{0000-0002-4258-4062},
C.~Vrahas$^{60}$\lhcborcid{0000-0001-6104-1496},
J.~Wagner$^{19}$\lhcborcid{0000-0002-9783-5957},
J.~Walsh$^{35}$\lhcborcid{0000-0002-7235-6976},
E.J.~Walton$^{1}$\lhcborcid{0000-0001-6759-2504},
G.~Wan$^{6}$\lhcborcid{0000-0003-0133-1664},
A. ~Wang$^{7}$\lhcborcid{0009-0007-4060-799X},
B. ~Wang$^{5}$\lhcborcid{0009-0008-4908-087X},
C.~Wang$^{22}$\lhcborcid{0000-0002-5909-1379},
G.~Wang$^{8}$\lhcborcid{0000-0001-6041-115X},
H.~Wang$^{75}$\lhcborcid{0009-0008-3130-0600},
J.~Wang$^{7}$\lhcborcid{0000-0001-7542-3073},
J.~Wang$^{5}$\lhcborcid{0000-0002-6391-2205},
J.~Wang$^{4,d}$\lhcborcid{0000-0002-3281-8136},
J.~Wang$^{76}$\lhcborcid{0000-0001-6711-4465},
M.~Wang$^{50}$\lhcborcid{0000-0003-4062-710X},
N. W. ~Wang$^{7}$\lhcborcid{0000-0002-6915-6607},
R.~Wang$^{56}$\lhcborcid{0000-0002-2629-4735},
X.~Wang$^{8}$\lhcborcid{0009-0006-3560-1596},
X.~Wang$^{74}$\lhcborcid{0000-0002-2399-7646},
X. W. ~Wang$^{63}$\lhcborcid{0000-0001-9565-8312},
Y.~Wang$^{77}$\lhcborcid{0000-0003-3979-4330},
Y.~Wang$^{6}$\lhcborcid{0009-0003-2254-7162},
Y. H. ~Wang$^{75}$\lhcborcid{0000-0003-1988-4443},
Z.~Wang$^{14}$\lhcborcid{0000-0002-5041-7651},
Z.~Wang$^{30}$\lhcborcid{0000-0003-4410-6889},
J.A.~Ward$^{58,1}$\lhcborcid{0000-0003-4160-9333},
M.~Waterlaat$^{50}$\lhcborcid{0000-0002-2778-0102},
N.K.~Watson$^{55}$\lhcborcid{0000-0002-8142-4678},
D.~Websdale$^{63}$\lhcborcid{0000-0002-4113-1539},
Y.~Wei$^{6}$\lhcborcid{0000-0001-6116-3944},
Z. ~Weida$^{7}$\lhcborcid{0009-0002-4429-2458},
J.~Wendel$^{45}$\lhcborcid{0000-0003-0652-721X},
B.D.C.~Westhenry$^{56}$\lhcborcid{0000-0002-4589-2626},
C.~White$^{57}$\lhcborcid{0009-0002-6794-9547},
M.~Whitehead$^{61}$\lhcborcid{0000-0002-2142-3673},
E.~Whiter$^{55}$\lhcborcid{0009-0003-3902-8123},
A.R.~Wiederhold$^{64}$\lhcborcid{0000-0002-1023-1086},
D.~Wiedner$^{19}$\lhcborcid{0000-0002-4149-4137},
M. A.~Wiegertjes$^{38}$\lhcborcid{0009-0002-8144-422X},
C. ~Wild$^{65}$\lhcborcid{0009-0008-1106-4153},
G.~Wilkinson$^{65,50}$\lhcborcid{0000-0001-5255-0619},
M.K.~Wilkinson$^{67}$\lhcborcid{0000-0001-6561-2145},
M.~Williams$^{66}$\lhcborcid{0000-0001-8285-3346},
M. J.~Williams$^{50}$\lhcborcid{0000-0001-7765-8941},
M.R.J.~Williams$^{60}$\lhcborcid{0000-0001-5448-4213},
R.~Williams$^{57}$\lhcborcid{0000-0002-2675-3567},
S. ~Williams$^{56}$\lhcborcid{ 0009-0007-1731-8700},
Z. ~Williams$^{56}$\lhcborcid{0009-0009-9224-4160},
F.F.~Wilson$^{59}$\lhcborcid{0000-0002-5552-0842},
M.~Winn$^{12}$\lhcborcid{0000-0002-2207-0101},
W.~Wislicki$^{42}$\lhcborcid{0000-0001-5765-6308},
M.~Witek$^{41}$\lhcborcid{0000-0002-8317-385X},
L.~Witola$^{19}$\lhcborcid{0000-0001-9178-9921},
T.~Wolf$^{22}$\lhcborcid{0009-0002-2681-2739},
E. ~Wood$^{57}$\lhcborcid{0009-0009-9636-7029},
G.~Wormser$^{14}$\lhcborcid{0000-0003-4077-6295},
S.A.~Wotton$^{57}$\lhcborcid{0000-0003-4543-8121},
H.~Wu$^{70}$\lhcborcid{0000-0002-9337-3476},
J.~Wu$^{8}$\lhcborcid{0000-0002-4282-0977},
X.~Wu$^{76}$\lhcborcid{0000-0002-0654-7504},
Y.~Wu$^{6,57}$\lhcborcid{0000-0003-3192-0486},
Z.~Wu$^{7}$\lhcborcid{0000-0001-6756-9021},
K.~Wyllie$^{50}$\lhcborcid{0000-0002-2699-2189},
S.~Xian$^{74}$\lhcborcid{0009-0009-9115-1122},
Z.~Xiang$^{5}$\lhcborcid{0000-0002-9700-3448},
Y.~Xie$^{8}$\lhcborcid{0000-0001-5012-4069},
T. X. ~Xing$^{30}$\lhcborcid{0009-0006-7038-0143},
A.~Xu$^{35,t}$\lhcborcid{0000-0002-8521-1688},
L.~Xu$^{4,d}$\lhcborcid{0000-0002-0241-5184},
M.~Xu$^{50}$\lhcborcid{0000-0001-8885-565X},
Z.~Xu$^{50}$\lhcborcid{0000-0002-7531-6873},
Z.~Xu$^{7}$\lhcborcid{0000-0001-9558-1079},
Z.~Xu$^{5}$\lhcborcid{0000-0001-9602-4901},
S. ~Yadav$^{26}$\lhcborcid{0009-0007-5014-1636},
K. ~Yang$^{63}$\lhcborcid{0000-0001-5146-7311},
X.~Yang$^{6}$\lhcborcid{0000-0002-7481-3149},
Y.~Yang$^{7}$\lhcborcid{0000-0002-8917-2620},
Y. ~Yang$^{81}$\lhcborcid{0009-0009-3430-0558},
Z.~Yang$^{6}$\lhcborcid{0000-0003-2937-9782},
H.~Yeung$^{64}$\lhcborcid{0000-0001-9869-5290},
H.~Yin$^{8}$\lhcborcid{0000-0001-6977-8257},
X. ~Yin$^{7}$\lhcborcid{0009-0003-1647-2942},
C. Y. ~Yu$^{6}$\lhcborcid{0000-0002-4393-2567},
J.~Yu$^{73}$\lhcborcid{0000-0003-1230-3300},
X.~Yuan$^{5}$\lhcborcid{0000-0003-0468-3083},
Y~Yuan$^{5,7}$\lhcborcid{0009-0000-6595-7266},
J. A.~Zamora~Saa$^{72}$\lhcborcid{0000-0002-5030-7516},
M.~Zavertyaev$^{21}$\lhcborcid{0000-0002-4655-715X},
M.~Zdybal$^{41}$\lhcborcid{0000-0002-1701-9619},
F.~Zenesini$^{25}$\lhcborcid{0009-0001-2039-9739},
C. ~Zeng$^{5,7}$\lhcborcid{0009-0007-8273-2692},
M.~Zeng$^{4,d}$\lhcborcid{0000-0001-9717-1751},
C.~Zhang$^{6}$\lhcborcid{0000-0002-9865-8964},
D.~Zhang$^{8}$\lhcborcid{0000-0002-8826-9113},
J.~Zhang$^{7}$\lhcborcid{0000-0001-6010-8556},
L.~Zhang$^{4,d}$\lhcborcid{0000-0003-2279-8837},
R.~Zhang$^{8}$\lhcborcid{0009-0009-9522-8588},
S.~Zhang$^{65}$\lhcborcid{0000-0002-2385-0767},
S.~L.~ ~Zhang$^{73}$\lhcborcid{0000-0002-9794-4088},
Y.~Zhang$^{6}$\lhcborcid{0000-0002-0157-188X},
Y. Z. ~Zhang$^{4,d}$\lhcborcid{0000-0001-6346-8872},
Z.~Zhang$^{4,d}$\lhcborcid{0000-0002-1630-0986},
Y.~Zhao$^{22}$\lhcborcid{0000-0002-8185-3771},
A.~Zhelezov$^{22}$\lhcborcid{0000-0002-2344-9412},
S. Z. ~Zheng$^{6}$\lhcborcid{0009-0001-4723-095X},
X. Z. ~Zheng$^{4,d}$\lhcborcid{0000-0001-7647-7110},
Y.~Zheng$^{7}$\lhcborcid{0000-0003-0322-9858},
T.~Zhou$^{6}$\lhcborcid{0000-0002-3804-9948},
X.~Zhou$^{8}$\lhcborcid{0009-0005-9485-9477},
V.~Zhovkovska$^{58}$\lhcborcid{0000-0002-9812-4508},
L. Z. ~Zhu$^{7}$\lhcborcid{0000-0003-0609-6456},
X.~Zhu$^{4,d}$\lhcborcid{0000-0002-9573-4570},
X.~Zhu$^{8}$\lhcborcid{0000-0002-4485-1478},
Y. ~Zhu$^{17}$\lhcborcid{0009-0004-9621-1028},
V.~Zhukov$^{17}$\lhcborcid{0000-0003-0159-291X},
J.~Zhuo$^{49}$\lhcborcid{0000-0002-6227-3368},
D.~Zuliani$^{33,r}$\lhcborcid{0000-0002-1478-4593},
G.~Zunica$^{28}$\lhcborcid{0000-0002-5972-6290}.\bigskip

{\footnotesize \it

$^{1}$School of Physics and Astronomy, Monash University, Melbourne, Australia\\
$^{2}$Centro Brasileiro de Pesquisas F{\'\i}sicas (CBPF), Rio de Janeiro, Brazil\\
$^{3}$Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil\\
$^{4}$Department of Engineering Physics, Tsinghua University, Beijing, China\\
$^{5}$Institute Of High Energy Physics (IHEP), Beijing, China\\
$^{6}$School of Physics State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing, China\\
$^{7}$University of Chinese Academy of Sciences, Beijing, China\\
$^{8}$Institute of Particle Physics, Central China Normal University, Wuhan, Hubei, China\\
$^{9}$Consejo Nacional de Rectores  (CONARE), San Jose, Costa Rica\\
$^{10}$Universit{\'e} Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France\\
$^{11}$Universit{\'e} Clermont Auvergne, CNRS/IN2P3, LPC, Clermont-Ferrand, France\\
$^{12}$Universit{\'e} Paris-Saclay, Centre d'Etudes de Saclay (CEA), IRFU, Saclay, France, Gif-Sur-Yvette, France\\
$^{13}$Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France\\
$^{14}$Universit{\'e} Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France\\
$^{15}$Laboratoire Leprince-Ringuet, CNRS/IN2P3, Ecole Polytechnique, Institut Polytechnique de Paris, Palaiseau, France\\
$^{16}$Laboratoire de Physique Nucl{\'e}aire et de Hautes {\'E}nergies (LPNHE), Sorbonne Universit{\'e}, CNRS/IN2P3, F-75005 Paris, France, Paris, France\\
$^{17}$I. Physikalisches Institut, RWTH Aachen University, Aachen, Germany\\
$^{18}$Universit{\"a}t Bonn - Helmholtz-Institut f{\"u}r Strahlen und Kernphysik, Bonn, Germany\\
$^{19}$Fakult{\"a}t Physik, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
$^{20}$Physikalisches Institut, Albert-Ludwigs-Universit{\"a}t Freiburg, Freiburg, Germany\\
$^{21}$Max-Planck-Institut f{\"u}r Kernphysik (MPIK), Heidelberg, Germany\\
$^{22}$Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg, Germany\\
$^{23}$School of Physics, University College Dublin, Dublin, Ireland\\
$^{24}$INFN Sezione di Bari, Bari, Italy\\
$^{25}$INFN Sezione di Bologna, Bologna, Italy\\
$^{26}$INFN Sezione di Ferrara, Ferrara, Italy\\
$^{27}$INFN Sezione di Firenze, Firenze, Italy\\
$^{28}$INFN Laboratori Nazionali di Frascati, Frascati, Italy\\
$^{29}$INFN Sezione di Genova, Genova, Italy\\
$^{30}$INFN Sezione di Milano, Milano, Italy\\
$^{31}$INFN Sezione di Milano-Bicocca, Milano, Italy\\
$^{32}$INFN Sezione di Cagliari, Monserrato, Italy\\
$^{33}$INFN Sezione di Padova, Padova, Italy\\
$^{34}$INFN Sezione di Perugia, Perugia, Italy\\
$^{35}$INFN Sezione di Pisa, Pisa, Italy\\
$^{36}$INFN Sezione di Roma La Sapienza, Roma, Italy\\
$^{37}$INFN Sezione di Roma Tor Vergata, Roma, Italy\\
$^{38}$Nikhef National Institute for Subatomic Physics, Amsterdam, Netherlands\\
$^{39}$Nikhef National Institute for Subatomic Physics and VU University Amsterdam, Amsterdam, Netherlands\\
$^{40}$AGH - University of Krakow, Faculty of Physics and Applied Computer Science, Krak{\'o}w, Poland\\
$^{41}$Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak{\'o}w, Poland\\
$^{42}$National Center for Nuclear Research (NCBJ), Warsaw, Poland\\
$^{43}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest-Magurele, Romania\\
$^{44}$Authors affiliated with an institute formerly covered by a cooperation agreement with CERN.\\
$^{45}$Universidade da Coru{\~n}a, A Coru{\~n}a, Spain\\
$^{46}$ICCUB, Universitat de Barcelona, Barcelona, Spain\\
$^{47}$La Salle, Universitat Ramon Llull, Barcelona, Spain\\
$^{48}$Instituto Galego de F{\'\i}sica de Altas Enerx{\'\i}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain\\
$^{49}$Instituto de Fisica Corpuscular, Centro Mixto Universidad de Valencia - CSIC, Valencia, Spain\\
$^{50}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$^{51}$Institute of Physics, Ecole Polytechnique  F{\'e}d{\'e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$^{52}$Physik-Institut, Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland\\
$^{53}$NSC Kharkiv Institute of Physics and Technology (NSC KIPT), Kharkiv, Ukraine\\
$^{54}$Institute for Nuclear Research of the National Academy of Sciences (KINR), Kyiv, Ukraine\\
$^{55}$School of Physics and Astronomy, University of Birmingham, Birmingham, United Kingdom\\
$^{56}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom\\
$^{57}$Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$^{58}$Department of Physics, University of Warwick, Coventry, United Kingdom\\
$^{59}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{60}$School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$^{61}$School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$^{62}$Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$^{63}$Imperial College London, London, United Kingdom\\
$^{64}$Department of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$^{65}$Department of Physics, University of Oxford, Oxford, United Kingdom\\
$^{66}$Massachusetts Institute of Technology, Cambridge, MA, United States\\
$^{67}$University of Cincinnati, Cincinnati, OH, United States\\
$^{68}$University of Maryland, College Park, MD, United States\\
$^{69}$Los Alamos National Laboratory (LANL), Los Alamos, NM, United States\\
$^{70}$Syracuse University, Syracuse, NY, United States\\
$^{71}$Pontif{\'\i}cia Universidade Cat{\'o}lica do Rio de Janeiro (PUC-Rio), Rio de Janeiro, Brazil, associated to $^{3}$\\
$^{72}$Universidad Andres Bello, Santiago, Chile, associated to $^{52}$\\
$^{73}$School of Physics and Electronics, Hunan University, Changsha City, China, associated to $^{8}$\\
$^{74}$State Key Laboratory of Nuclear Physics and Technology, South China Normal University, Guangzhou, China., Guangzhou, China, associated to $^{4}$\\
$^{75}$Lanzhou University, Lanzhou, China, associated to $^{5}$\\
$^{76}$School of Physics and Technology, Wuhan University, Wuhan, China, associated to $^{4}$\\
$^{77}$Henan Normal University, Xinxiang, China, associated to $^{8}$\\
$^{78}$Departamento de Fisica , Universidad Nacional de Colombia, Bogota, Colombia, associated to $^{16}$\\
$^{79}$Institute of Physics of  the Czech Academy of Sciences, Prague, Czech Republic, associated to $^{64}$\\
$^{80}$Ruhr Universitaet Bochum, Fakultaet f. Physik und Astronomie, Bochum, Germany, associated to $^{19}$\\
$^{81}$Eotvos Lorand University, Budapest, Hungary, associated to $^{50}$\\
$^{82}$Faculty of Physics, Vilnius University, Vilnius, Lithuania, associated to $^{20}$\\
$^{83}$Van Swinderen Institute, University of Groningen, Groningen, Netherlands, associated to $^{38}$\\
$^{84}$Universiteit Maastricht, Maastricht, Netherlands, associated to $^{38}$\\
$^{85}$Tadeusz Kosciuszko Cracow University of Technology, Cracow, Poland, associated to $^{41}$\\
$^{86}$Department of Physics and Astronomy, Uppsala University, Uppsala, Sweden, associated to $^{61}$\\
$^{87}$Taras Schevchenko University of Kyiv, Faculty of Physics, Kyiv, Ukraine, associated to $^{14}$\\
$^{88}$University of Michigan, Ann Arbor, MI, United States, associated to $^{70}$\\
$^{89}$Indiana University, Bloomington, United States, associated to $^{69}$\\
$^{90}$Ohio State University, Columbus, United States, associated to $^{69}$\\
\bigskip
$^{a}$Universidade Estadual de Campinas (UNICAMP), Campinas, Brazil\\
$^{b}$Centro Federal de Educac{\~a}o Tecnol{\'o}gica Celso Suckow da Fonseca, Rio De Janeiro, Brazil\\
$^{c}$Department of Physics and Astronomy, University of Victoria, Victoria, Canada\\
$^{d}$Center for High Energy Physics, Tsinghua University, Beijing, China\\
$^{e}$Hangzhou Institute for Advanced Study, UCAS, Hangzhou, China\\
$^{f}$LIP6, Sorbonne Universit{\'e}, Paris, France\\
$^{g}$Lamarr Institute for Machine Learning and Artificial Intelligence, Dortmund, Germany\\
$^{h}$Universidad Nacional Aut{\'o}noma de Honduras, Tegucigalpa, Honduras\\
$^{i}$Universit{\`a} di Bari, Bari, Italy\\
$^{j}$Universit{\`a} di Bergamo, Bergamo, Italy\\
$^{k}$Universit{\`a} di Bologna, Bologna, Italy\\
$^{l}$Universit{\`a} di Cagliari, Cagliari, Italy\\
$^{m}$Universit{\`a} di Ferrara, Ferrara, Italy\\
$^{n}$Universit{\`a} di Genova, Genova, Italy\\
$^{o}$Universit{\`a} degli Studi di Milano, Milano, Italy\\
$^{p}$Universit{\`a} degli Studi di Milano-Bicocca, Milano, Italy\\
$^{q}$Universit{\`a} di Modena e Reggio Emilia, Modena, Italy\\
$^{r}$Universit{\`a} di Padova, Padova, Italy\\
$^{s}$Universit{\`a}  di Perugia, Perugia, Italy\\
$^{t}$Scuola Normale Superiore, Pisa, Italy\\
$^{u}$Universit{\`a} di Pisa, Pisa, Italy\\
$^{v}$Universit{\`a} di Siena, Siena, Italy\\
$^{w}$Universit{\`a} di Urbino, Urbino, Italy\\
$^{x}$Universidad de Ingenier\'{i}a y Tecnolog\'{i}a (UTEC), Lima, Peru\\
$^{y}$Universidad de Alcal{\'a}, Alcal{\'a} de Henares , Spain\\
\medskip
}
\end{flushleft}

==> lhcb_text/acknowledgements.tex <==
\clearpage
\section*{Acknowledgements}
%
% These Acknowledgements valid from 12/09/25
%
\noindent We express our gratitude to our colleagues in the CERN
accelerator departments for the excellent performance of the LHC. We
thank the technical and administrative staff at the LHCb
institutes.
We thank James Vincent Mead and Stephen Farry
for their pioneering work on top-quark production, which has substantially informed
and supported the development of this measurement~\cite{james_paper}.
We acknowledge support from CERN and from the national agencies:
ARC (Australia);
CAPES, CNPq, FAPERJ and FINEP (Brazil); 
MOST and NSFC (China); 
CNRS/IN2P3 (France); 
BMFTR, DFG and MPG (Germany);
INFN (Italy); 
NWO (Netherlands); 
MNiSW and NCN (Poland); 
MCID/IFA (Romania); 
%MSHE (Russia); 
MICIU and AEI (Spain);
SNSF and SER (Switzerland); 
NASU (Ukraine); 
STFC (United Kingdom); 
DOE NP and NSF (USA).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We acknowledge the computing resources that are provided by ARDC (Australia), 
CBPF (Brazil),
CERN, 
IHEP and LZU (China),
IN2P3 (France), 
KIT and DESY (Germany), 
INFN (Italy), 
SURF (Netherlands),
Polish WLCG (Poland),
IFIN-HH (Romania), 
%RRCKI and Yandex LLC (Russia), 
PIC (Spain), CSCS (Switzerland), 
and GridPP (United Kingdom).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We are indebted to the communities behind the multiple open-source
software packages on which we depend.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Individual groups or members have received support from
%ARC and ARDC (Australia); % moved to national 16/01
Key Research Program of Frontier Sciences of CAS, CAS PIFI, CAS CCEPP, 
%Fundamental Research Funds for the Central Universities,  and Sci.\
%\& Tech.\ Program of Guangzhou (China); Removed 24/11/25
Minciencias (Colombia);
EPLANET, Marie Sk\l{}odowska-Curie Actions, ERC and NextGenerationEU (European Union);
A*MIDEX, ANR, IPhU and Labex P2IO, and R\'{e}gion Auvergne-Rh\^{o}ne-Alpes (France);
%RFBR, RSF and Yandex LLC (Russia);
Alexander-von-Humboldt Foundation (Germany);
ICSC (Italy); 
%GVA, XuntaGal, GENCAT, Inditex, InTalent and Prog.~Atracci\'on Talento, CM (Spain);
Severo Ochoa and Mar\'ia de Maeztu Units of Excellence, GVA, XuntaGal, GENCAT, InTalent-Inditex and Prog.~Atracci\'on Talento CM (Spain);
SRC (Sweden);
the Leverhulme Trust, the Royal Society and UKRI (United Kingdom).



==> lhcb_text/lhcb-symbols-def.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                                                                    %
%%% !!!!!!!!!!!!!!!!!!! DO NOT EDIT THIS FILE !!!!!!!!!!!!!!!!!!!!!!!! %
%%%                                                                    %
%%% THE EB MAY OVERWRITE IT TO REFLECT LATEST CHANGES IN THE TEMPLATE  %
%%%                                                                    %
%%% You may define your own macros and packages in main.tex or add     %
%%% additional local files                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% ======================================================================
%%% Purpose: Standard LHCb aliases
%%% Author: Originally Ulrik Egede, adapted by Tomasz Skwarnicki for templates,
%%% rewritten by Chris Parkes
%%% Maintainer : Ulrik Egede (2010 - 2012)
%%% Maintainer : Rolf Oldeman (2012 - 2014)
%%% Maintainer : Patrick Koppenburg (2018--2020)
%%% =======================================================================
%%% To use this file outside the normal LHCb document environment, the
%%% following should be added in a preamble (before \begin{document}
%%%
%%%\usepackage{ifthen} 
%%%\newboolean{uprightparticles}
%%%\setboolean{uprightparticles}{false} %Set true for upright particle symbols
\usepackage{xspace} 
\usepackage{upgreek}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% The following is to ensure that the template automatically can process
%%% this file.
%%%
%%% Add comments with at least three %%% preceding.
%%% Add new sections with one % preceding
%%% Add new subsections with two %% preceding
%%%
%%% For upper greek letters, Xires and Xiresbar will be the particles without the charge
%%% States with charge are called Xiz and Xim  
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%
% Experiments
%%%%%%%%%%%%%
\def\lhcb   {\mbox{LHCb}\xspace}
\def\atlas  {\mbox{ATLAS}\xspace}
\def\cms    {\mbox{CMS}\xspace}
\def\alice  {\mbox{ALICE}\xspace}
\def\babar  {\mbox{BaBar}\xspace}
\def\belle  {\mbox{Belle}\xspace}
\def\belletwo {\mbox{Belle~II}\xspace}
\def\besiii {\mbox{BESIII}\xspace}
\def\cleo   {\mbox{CLEO}\xspace}
\def\cdf    {\mbox{CDF}\xspace}
\def\dzero  {\mbox{D0}\xspace}
\def\aleph  {\mbox{ALEPH}\xspace}
\def\delphi {\mbox{DELPHI}\xspace}
\def\opal   {\mbox{OPAL}\xspace}
\def\lthree {\mbox{L3}\xspace}
\def\sld    {\mbox{SLD}\xspace}
%%%\def\argus  {\mbox{ARGUS}\xspace}
%%%\def\uaone  {\mbox{UA1}\xspace}
%%%\def\uatwo  {\mbox{UA2}\xspace}
%%%\def\ux85 {\mbox{UX85}\xspace}
\def\cern {\mbox{CERN}\xspace}
\def\lhc    {\mbox{LHC}\xspace}
\def\lep    {\mbox{LEP}\xspace}
\def\tevatron {Tevatron\xspace}
\def\bfactories {\mbox{\B Factories}\xspace}
\def\bfactory   {\mbox{\B Factory}\xspace}
\def\upgradeone {\mbox{Upgrade~I}\xspace}
\def\upgradetwo {\mbox{Upgrade~II}\xspace}

%% LHCb sub-detectors and sub-systems

%%%\def\pu     {PU\xspace}
\def\velo   {VELO\xspace}
\def\rich   {RICH\xspace}
\def\richone {RICH1\xspace}
\def\richtwo {RICH2\xspace}
\def\ttracker {TT\xspace}
\def\intr   {IT\xspace}
\def\st     {ST\xspace}
\def\ot     {OT\xspace}
\def\herschel {\mbox{\textsc{HeRSCheL}}\xspace}
%%%\def\Tone   {T1\xspace}
%%%\def\Ttwo   {T2\xspace}
%%%\def\Tthree {T3\xspace}
%%%\def\Mone   {M1\xspace}
%%%\def\Mtwo   {M2\xspace}
%%%\def\Mthree {M3\xspace}
%%%\def\Mfour  {M4\xspace}
%%%\def\Mfive  {M5\xspace}
\def\spd    {SPD\xspace}
\def\presh  {PS\xspace}
\def\ecal   {ECAL\xspace}
\def\hcal   {HCAL\xspace}
%%%\def\bcm    {BCM\xspace}
\def\MagUp {\mbox{\em Mag\kern -0.05em Up}\xspace}
\def\MagDown {\mbox{\em MagDown}\xspace}

\def\ode    {ODE\xspace}
\def\daq    {DAQ\xspace}
\def\tfc    {TFC\xspace}
\def\ecs    {ECS\xspace}
\def\lone   {L0\xspace}
\def\hlt    {HLT\xspace}
\def\hltone {HLT1\xspace}
\def\hlttwo {HLT2\xspace}

%%% Upright (not slanted) Particles

\ifthenelse{\boolean{uprightparticles}}%
{\def\Palpha      {\ensuremath{\upalpha}\xspace}
 \def\Pbeta       {\ensuremath{\upbeta}\xspace}
 \def\Pgamma      {\ensuremath{\upgamma}\xspace}                 
 \def\Pdelta      {\ensuremath{\updelta}\xspace}                 
 \def\Pepsilon    {\ensuremath{\upepsilon}\xspace}                 
 \def\Pvarepsilon {\ensuremath{\upvarepsilon}\xspace}                 
 \def\Pzeta       {\ensuremath{\upzeta}\xspace}                 
 \def\Peta        {\ensuremath{\upeta}\xspace}
 \def\Ptheta      {\ensuremath{\uptheta}\xspace}                 
 \def\Pvartheta   {\ensuremath{\upvartheta}\xspace}                 
 \def\Piota       {\ensuremath{\upiota}\xspace}                 
 \def\Pkappa      {\ensuremath{\upkappa}\xspace}                 
 \def\Plambda     {\ensuremath{\uplambda}\xspace}                 
 \def\Pmu         {\ensuremath{\upmu}\xspace}                 
 \def\Pnu         {\ensuremath{\upnu}\xspace}                 
 \def\Pxi         {\ensuremath{\upxi}\xspace}                 
 \def\Ppi         {\ensuremath{\uppi}\xspace}                 
 \def\Pvarpi      {\ensuremath{\upvarpi}\xspace}                 
 \def\Prho        {\ensuremath{\uprho}\xspace}                 
 \def\Pvarrho     {\ensuremath{\upvarrho}\xspace}                 
 \def\Ptau        {\ensuremath{\uptau}\xspace}                 
 \def\Pupsilon    {\ensuremath{\upupsilon}\xspace}                 
 \def\Pphi        {\ensuremath{\upphi}\xspace}                 
 \def\Pvarphi     {\ensuremath{\upvarphi}\xspace}                 
 \def\Pchi        {\ensuremath{\upchi}\xspace}                 
 \def\Ppsi        {\ensuremath{\uppsi}\xspace}                 
 \def\Pomega      {\ensuremath{\upomega}\xspace}                 

 \def\PDelta      {\ensuremath{\Delta}\xspace}                 
 \def\PXi         {\ensuremath{\Xi}\xspace}                 
 \def\PLambda     {\ensuremath{\Lambda}\xspace}                 
 \def\PSigma      {\ensuremath{\Sigma}\xspace}                 
 \def\POmega      {\ensuremath{\Omega}\xspace}                 
 \def\PUpsilon    {\ensuremath{\Upsilon}\xspace}
 \let\oldPi\Pi
 \def\PPi         {\ensuremath{\oldPi}\xspace}                 
               

 %\def\PA      {\ensuremath{\mathrm{A}}\xspace}                 
 \def\PB      {\ensuremath{\mathrm{B}}\xspace}                 
 %\def\PC      {\ensuremath{\mathrm{C}}\xspace}                 
 \def\PD      {\ensuremath{\mathrm{D}}\xspace}                 
 %\def\PE      {\ensuremath{\mathrm{E}}\xspace}                 
 %\def\PF      {\ensuremath{\mathrm{F}}\xspace}                 
 %\def\PG      {\ensuremath{\mathrm{G}}\xspace}                 
 \def\PH      {\ensuremath{\mathrm{H}}\xspace}                 
 %\def\PI      {\ensuremath{\mathrm{I}}\xspace}                 
 \def\PJ      {\ensuremath{\mathrm{J}}\xspace}                 
 \def\PK      {\ensuremath{\mathrm{K}}\xspace}                 
 %\def\PL      {\ensuremath{\mathrm{L}}\xspace}                 
 %\def\PM      {\ensuremath{\mathrm{M}}\xspace}                 
 %\def\PN      {\ensuremath{\mathrm{N}}\xspace}                 
 %\def\PO      {\ensuremath{\mathrm{O}}\xspace}                 
 %\def\PP      {\ensuremath{\mathrm{P}}\xspace}                 
 %\def\PQ      {\ensuremath{\mathrm{Q}}\xspace}                 
 %\def\PR      {\ensuremath{\mathrm{R}}\xspace}                 
 %\def\PS      {\ensuremath{\mathrm{S}}\xspace}                 
 %\def\PT      {\ensuremath{\mathrm{T}}\xspace}                 
 %\def\PU      {\ensuremath{\mathrm{U}}\xspace}                 
 %\def\PV      {\ensuremath{\mathrm{V}}\xspace}                 
 \def\PW      {\ensuremath{\mathrm{W}}\xspace}                 
 %\def\PX      {\ensuremath{\mathrm{X}}\xspace}                 
 %\def\PY      {\ensuremath{\mathrm{Y}}\xspace}                 
 \def\PZ      {\ensuremath{\mathrm{Z}}\xspace}                 
 %\def\Pa      {\ensuremath{\mathrm{a}}\xspace}                 
 \def\Pb      {\ensuremath{\mathrm{b}}\xspace}                 
 \def\Pc      {\ensuremath{\mathrm{c}}\xspace}                 
 \def\Pd      {\ensuremath{\mathrm{d}}\xspace}                 
 \def\Pe      {\ensuremath{\mathrm{e}}\xspace}                 
 %\def\Pf      {\ensuremath{\mathrm{f}}\xspace}                 
 \def\Pg      {\ensuremath{\mathrm{g}}\xspace}                 
 \def\Ph      {\ensuremath{\mathrm{h}}\xspace}                 
 %\def\Pi      {\ensuremath{\mathrm{i}}\xspace}                 
 %\def\Pj      {\ensuremath{\mathrm{j}}\xspace}                 
 %\def\Pk      {\ensuremath{\mathrm{k}}\xspace}                 
 %\def\Pl      {\ensuremath{\mathrm{l}}\xspace}                 
 %\def\Pm      {\ensuremath{\mathrm{m}}\xspace}                 
 \def\Pn      {\ensuremath{\mathrm{n}}\xspace}                 
 %\def\Po      {\ensuremath{\mathrm{o}}\xspace}                 
 \def\Pp      {\ensuremath{\mathrm{p}}\xspace}                 
 \def\Pq      {\ensuremath{\mathrm{q}}\xspace}                 
 %\def\Pr      {\ensuremath{\mathrm{r}}\xspace}                 
 \def\Ps      {\ensuremath{\mathrm{s}}\xspace}                 
 \def\Pt      {\ensuremath{\mathrm{t}}\xspace}                 
 \def\Pu      {\ensuremath{\mathrm{u}}\xspace}                 
 %\def\Pv      {\ensuremath{\mathrm{v}}\xspace}                 
 %\def\Pw      {\ensuremath{\mathrm{w}}\xspace}                 
 %\def\Px      {\ensuremath{\mathrm{x}}\xspace}                 
 %\def\Py      {\ensuremath{\mathrm{y}}\xspace}                 
 %\def\Pz      {\ensuremath{\mathrm{z}}\xspace}                 
 \def\thebaroffset{0.0em}
}
{\def\Palpha      {\ensuremath{\alpha}\xspace}
 \def\Pbeta       {\ensuremath{\beta}\xspace}
 \def\Pgamma      {\ensuremath{\gamma}\xspace}                 
 \def\Pdelta      {\ensuremath{\delta}\xspace}                 
 \def\Pepsilon    {\ensuremath{\epsilon}\xspace}                 
 \def\Pvarepsilon {\ensuremath{\varepsilon}\xspace}                 
 \def\Pzeta       {\ensuremath{\zeta}\xspace}                 
 \def\Peta        {\ensuremath{\eta}\xspace}                 
 \def\Ptheta      {\ensuremath{\theta}\xspace}                 
 \def\Pvartheta   {\ensuremath{\vartheta}\xspace}                 
 \def\Piota       {\ensuremath{\iota}\xspace}                 
 \def\Pkappa      {\ensuremath{\kappa}\xspace}                 
 \def\Plambda     {\ensuremath{\lambda}\xspace}                 
 \def\Pmu         {\ensuremath{\mu}\xspace}                 
 \def\Pnu         {\ensuremath{\nu}\xspace}                 
 \def\Pxi         {\ensuremath{\xi}\xspace}                 
 \def\Ppi         {\ensuremath{\pi}\xspace}                 
 \def\Pvarpi      {\ensuremath{\varpi}\xspace}                 
 \def\Prho        {\ensuremath{\rho}\xspace}                 
 \def\Pvarrho     {\ensuremath{\varrho}\xspace}                 
 \def\Ptau        {\ensuremath{\tau}\xspace}                 
 \def\Pupsilon    {\ensuremath{\upsilon}\xspace}                 
 \def\Pphi        {\ensuremath{\phi}\xspace}                 
 \def\Pvarphi     {\ensuremath{\varphi}\xspace}                 
 \def\Pchi        {\ensuremath{\chi}\xspace}                 
 \def\Ppsi        {\ensuremath{\psi}\xspace}                 
 \def\Pomega      {\ensuremath{\omega}\xspace}                 
 \mathchardef\PDelta="7101
 \mathchardef\PXi="7104
 \mathchardef\PLambda="7103
 \mathchardef\PSigma="7106
 \mathchardef\POmega="710A
 \mathchardef\PUpsilon="7107
 \mathchardef\PPi="7105
 %\def\PA      {\ensuremath{A}\xspace}                 
 \def\PB      {\ensuremath{B}\xspace}                 
 %\def\PC      {\ensuremath{C}\xspace}                 
 \def\PD      {\ensuremath{D}\xspace}                 
 %\def\PE      {\ensuremath{E}\xspace}                 
 %\def\PF      {\ensuremath{F}\xspace}                 
 %\def\PG      {\ensuremath{G}\xspace}                 
 \def\PH      {\ensuremath{H}\xspace}                 
 %\def\PI      {\ensuremath{I}\xspace}                 
 \def\PJ      {\ensuremath{J}\xspace}                 
 \def\PK      {\ensuremath{K}\xspace}                 
 %\def\PL      {\ensuremath{L}\xspace}                 
 %\def\PM      {\ensuremath{M}\xspace}                 
 %\def\PN      {\ensuremath{N}\xspace}                 
 %\def\PO      {\ensuremath{O}\xspace}                 
 %\def\PP      {\ensuremath{P}\xspace}                 
 %\def\PQ      {\ensuremath{Q}\xspace}                 
 %\def\PR      {\ensuremath{R}\xspace}                 
 %\def\PS      {\ensuremath{S}\xspace}                 
 %\def\PT      {\ensuremath{T}\xspace}                 
 %\def\PU      {\ensuremath{U}\xspace}                 
 %\def\PV      {\ensuremath{V}\xspace}                 
 \def\PW      {\ensuremath{W}\xspace}                 
 %\def\PX      {\ensuremath{X}\xspace}                 
 %\def\PY      {\ensuremath{Y}\xspace}                 
 \def\PZ      {\ensuremath{Z}\xspace}                 
 %\def\Pa      {\ensuremath{a}\xspace}                 
 \def\Pb      {\ensuremath{b}\xspace}                 
 \def\Pc      {\ensuremath{c}\xspace}                 
 \def\Pd      {\ensuremath{d}\xspace}                 
 \def\Pe      {\ensuremath{e}\xspace}                 
 %\def\Pf      {\ensuremath{f}\xspace}                 
 \def\Pg      {\ensuremath{g}\xspace}                 
 \def\Ph      {\ensuremath{h}\xspace}                 
 %\def\Pi      {\ensuremath{i}\xspace}                 
 %\def\Pj      {\ensuremath{j}\xspace}                 
 %\def\Pk      {\ensuremath{k}\xspace}                 
 %\def\Pl      {\ensuremath{l}\xspace}                 
 %\def\Pm      {\ensuremath{m}\xspace}                 
 \def\Pn      {\ensuremath{n}\xspace}                 
 %\def\Po      {\ensuremath{o}\xspace}                 
 \def\Pp      {\ensuremath{p}\xspace}                 
 \def\Pq      {\ensuremath{q}\xspace}                 
 %\def\Pr      {\ensuremath{r}\xspace}                 
 \def\Ps      {\ensuremath{s}\xspace}                 
 \def\Pt      {\ensuremath{t}\xspace}                 
 \def\Pu      {\ensuremath{u}\xspace}                 
 %\def\Pv      {\ensuremath{v}\xspace}                 
 %\def\Pw      {\ensuremath{w}\xspace}                 
 %\def\Px      {\ensuremath{x}\xspace}                 
 %\def\Py      {\ensuremath{y}\xspace}                 
 %\def\Pz      {\ensuremath{z}\xspace}
 \def\thebaroffset{0.18em}
}
\newcommand{\offsetoverline}[2][\thebaroffset]{\kern #1\overline{\kern -#1 #2}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Particles
\makeatletter
\ifcase \@ptsize \relax% 10pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{4}{5}}% \tiny: 5/6
\or% 11pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{5}{6}}% \tiny: 6/7
\or% 12pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{5}{6}}% \tiny: 6/7
\fi
\makeatother


\DeclareRobustCommand{\optbar}[1]{\shortstack{{\miniscule (\rule[.5ex]{1.25em}{.18mm})}
  \\ [-.7ex] $#1$}}


%% Leptons

\let\emi\en
\def\electron   {{\ensuremath{\Pe}}\xspace}
\def\en         {{\ensuremath{\Pe^-}}\xspace}   % electron negative (\em is taken)
\def\ep         {{\ensuremath{\Pe^+}}\xspace}
\def\epm        {{\ensuremath{\Pe^\pm}}\xspace} 
\def\emp        {{\ensuremath{\Pe^\mp}}\xspace} 
\def\epem       {{\ensuremath{\Pe^+\Pe^-}}\xspace}
%%%\def\ee         {\ensuremath{\Pe^-\Pe^-}\xspace}

\def\muon       {{\ensuremath{\Pmu}}\xspace}
\def\mup        {{\ensuremath{\Pmu^+}}\xspace}
\def\mun        {{\ensuremath{\Pmu^-}}\xspace} % muon negative (\mum is taken)
\def\mupm       {{\ensuremath{\Pmu^\pm}}\xspace} 
\def\mump       {{\ensuremath{\Pmu^\mp}}\xspace} 
\def\mumu       {{\ensuremath{\Pmu^+\Pmu^-}}\xspace}

\def\tauon      {{\ensuremath{\Ptau}}\xspace}
\def\taup       {{\ensuremath{\Ptau^+}}\xspace}
\def\taum       {{\ensuremath{\Ptau^-}}\xspace}
\def\taupm      {{\ensuremath{\Ptau^\pm}}\xspace}
\def\taump      {{\ensuremath{\Ptau^\mp}}\xspace}
\def\tautau     {{\ensuremath{\Ptau^+\Ptau^-}}\xspace}

\def\lepton     {{\ensuremath{\ell}}\xspace}
\def\ellm       {{\ensuremath{\ell^-}}\xspace}
\def\ellp       {{\ensuremath{\ell^+}}\xspace}
\def\ellpm      {{\ensuremath{\ell^\pm}}\xspace}
\def\ellmp      {{\ensuremath{\ell^\mp}}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\neu        {{\ensuremath{\Pnu}}\xspace}
\def\neub       {{\ensuremath{\overline{\Pnu}}}\xspace}
%%%\def\nuenueb    {\ensuremath{\neu\neub}\xspace}
\def\neue       {{\ensuremath{\neu_e}}\xspace}
\def\neueb      {{\ensuremath{\neub_e}}\xspace}
%%%\def\neueneueb  {\ensuremath{\neue\neueb}\xspace}
\def\neum       {{\ensuremath{\neu_\mu}}\xspace}
\def\neumb      {{\ensuremath{\neub_\mu}}\xspace}
%%%\def\neumneumb  {\ensuremath{\neum\neumb}\xspace}
\def\neut       {{\ensuremath{\neu_\tau}}\xspace}
\def\neutb      {{\ensuremath{\neub_\tau}}\xspace}
%%%\def\neutneutb  {\ensuremath{\neut\neutb}\xspace}
\def\neul       {{\ensuremath{\neu_\ell}}\xspace}
\def\neulb      {{\ensuremath{\neub_\ell}}\xspace}
%%%\def\neulneulb  {\ensuremath{\neul\neulb}\xspace}

%% Gauge bosons and scalars

\def\g      {{\ensuremath{\Pgamma}}\xspace}
\def\H      {{\ensuremath{\PH^0}}\xspace}
\def\Hp     {{\ensuremath{\PH^+}}\xspace}
\def\Hm     {{\ensuremath{\PH^-}}\xspace}
\def\Hpm    {{\ensuremath{\PH^\pm}}\xspace}
\def\W      {{\ensuremath{\PW}}\xspace}
\def\Wp     {{\ensuremath{\PW^+}}\xspace}
\def\Wm     {{\ensuremath{\PW^-}}\xspace}
\def\Wpm    {{\ensuremath{\PW^\pm}}\xspace}
\def\Z      {{\ensuremath{\PZ}}\xspace}

%% Quarks

\def\quark     {{\ensuremath{\Pq}}\xspace}
\def\quarkbar  {{\ensuremath{\overline \quark}}\xspace}
\def\qqbar     {{\ensuremath{\quark\quarkbar}}\xspace}
\def\uquark    {{\ensuremath{\Pu}}\xspace}
\def\uquarkbar {{\ensuremath{\overline \uquark}}\xspace}
\def\uubar     {{\ensuremath{\uquark\uquarkbar}}\xspace}
\def\dquark    {{\ensuremath{\Pd}}\xspace}
\def\dquarkbar {{\ensuremath{\overline \dquark}}\xspace}
\def\ddbar     {{\ensuremath{\dquark\dquarkbar}}\xspace}
\def\squark    {{\ensuremath{\Ps}}\xspace}
\def\squarkbar {{\ensuremath{\overline \squark}}\xspace}
\def\ssbar     {{\ensuremath{\squark\squarkbar}}\xspace}
\def\cquark    {{\ensuremath{\Pc}}\xspace}
\def\cquarkbar {{\ensuremath{\overline \cquark}}\xspace}
\def\ccbar     {{\ensuremath{\cquark\cquarkbar}}\xspace}
\def\bquark    {{\ensuremath{\Pb}}\xspace}
\def\bquarkbar {{\ensuremath{\overline \bquark}}\xspace}
\def\bbbar     {{\ensuremath{\bquark\bquarkbar}}\xspace}
\def\tquark    {{\ensuremath{\Pt}}\xspace}
\def\tquarkbar {{\ensuremath{\overline \tquark}}\xspace}
\def\ttbar     {{\ensuremath{\tquark\tquarkbar}}\xspace}

%% Light mesons

\def\hadron {{\ensuremath{\Ph}}\xspace}
\def\pion   {{\ensuremath{\Ppi}}\xspace}
\def\piz    {{\ensuremath{\pion^0}}\xspace}
\def\pip    {{\ensuremath{\pion^+}}\xspace}
\def\pim    {{\ensuremath{\pion^-}}\xspace}
\def\pipm   {{\ensuremath{\pion^\pm}}\xspace}
\def\pimp   {{\ensuremath{\pion^\mp}}\xspace}

\def\rhomeson {{\ensuremath{\Prho}}\xspace}
\def\rhoz     {{\ensuremath{\rhomeson^0}}\xspace}
\def\rhop     {{\ensuremath{\rhomeson^+}}\xspace}
\def\rhom     {{\ensuremath{\rhomeson^-}}\xspace}
\def\rhopm    {{\ensuremath{\rhomeson^\pm}}\xspace}
\def\rhomp    {{\ensuremath{\rhomeson^\mp}}\xspace}

\def\kaon    {{\ensuremath{\PK}}\xspace}
%%% do NOT use ensuremath here, and keep indent
\def\Kbar    {{\ensuremath{\offsetoverline{\PK}}}\xspace}
\def\Kb      {{\ensuremath{\Kbar}}\xspace}
\def\KorKbar {\kern \thebaroffset\optbar{\kern -\thebaroffset \PK}{}\xspace}
\def\Kz      {{\ensuremath{\kaon^0}}\xspace}
\def\Kzb     {{\ensuremath{\Kbar{}^0}}\xspace}
\def\Kp      {{\ensuremath{\kaon^+}}\xspace}
\def\Km      {{\ensuremath{\kaon^-}}\xspace}
\def\Kpm     {{\ensuremath{\kaon^\pm}}\xspace}
\def\Kmp     {{\ensuremath{\kaon^\mp}}\xspace}
\def\KS      {{\ensuremath{\kaon^0_{\mathrm{S}}}}\xspace}
\def\Vzero   {{\ensuremath{V^0}}\xspace}
\def\KL      {{\ensuremath{\kaon^0_{\mathrm{L}}}}\xspace}
\def\Kstarz  {{\ensuremath{\kaon^{*0}}}\xspace}
\def\Kstarzb {{\ensuremath{\Kbar{}^{*0}}}\xspace}
\def\Kstar   {{\ensuremath{\kaon^*}}\xspace}
\def\Kstarb  {{\ensuremath{\Kbar{}^*}}\xspace}
\def\Kstarp  {{\ensuremath{\kaon^{*+}}}\xspace}
\def\Kstarm  {{\ensuremath{\kaon^{*-}}}\xspace}
\def\Kstarpm {{\ensuremath{\kaon^{*\pm}}}\xspace}
\def\Kstarmp {{\ensuremath{\kaon^{*\mp}}}\xspace}
\def\KorKbarz {\ensuremath{\KorKbar^0}\xspace}

\newcommand{\etaz}{\ensuremath{\Peta}\xspace}
\newcommand{\etapr}{\ensuremath{\Peta^{\prime}}\xspace}
\newcommand{\phiz}{\ensuremath{\Pphi}\xspace}
\newcommand{\omegaz}{\ensuremath{\Pomega}\xspace}

%% Charmed mesons

%%% do NOT use ensuremath here (and keep indent)
\def\Dbar    {{\ensuremath{\offsetoverline{\PD}}}\xspace}
\def\D       {{\ensuremath{\PD}}\xspace}
\def\Db      {{\ensuremath{\Dbar}}\xspace}
\def\DorDbar {\kern \thebaroffset\optbar{\kern -\thebaroffset \PD}\xspace}
\def\Dz      {{\ensuremath{\D^0}}\xspace}
\def\Dzb     {{\ensuremath{\Dbar{}^0}}\xspace}
\def\Dp      {{\ensuremath{\D^+}}\xspace}
\def\Dm      {{\ensuremath{\D^-}}\xspace}
\def\Dpm     {{\ensuremath{\D^\pm}}\xspace}
\def\Dmp     {{\ensuremath{\D^\mp}}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {{\ensuremath{\D^*}}\xspace}
\def\Dstarb  {{\ensuremath{\Dbar{}^*}}\xspace}
\def\Dstarz  {{\ensuremath{\D^{*0}}}\xspace}
\def\Dstarzb {{\ensuremath{\Dbar{}^{*0}}}\xspace}
\def\theDstarz{{\ensuremath{\D^{*}(2007)^{0}}}\xspace}
\def\theDstarzb{{\ensuremath{\Dbar^{*}(2007)^{0}}}\xspace}
\def\Dstarp  {{\ensuremath{\D^{*+}}}\xspace}
\def\Dstarm  {{\ensuremath{\D^{*-}}}\xspace}
\def\Dstarpm {{\ensuremath{\D^{*\pm}}}\xspace}
\def\Dstarmp {{\ensuremath{\D^{*\mp}}}\xspace}
\def\theDstarp{{\ensuremath{\D^{*}(2010)^{+}}}\xspace}
\def\theDstarm{{\ensuremath{\D^{*}(2010)^{-}}}\xspace}
\def\theDstarpm{{\ensuremath{\D^{*}(2010)^{\pm}}}\xspace}
\def\theDstarmp{{\ensuremath{\D^{*}(2010)^{\mp}}}\xspace}
\def\Ds      {{\ensuremath{\D^+_\squark}}\xspace}
\def\Dsp     {{\ensuremath{\D^+_\squark}}\xspace}
\def\Dsm     {{\ensuremath{\D^-_\squark}}\xspace}
\def\Dspm    {{\ensuremath{\D^{\pm}_\squark}}\xspace}
\def\Dsmp    {{\ensuremath{\D^{\mp}_\squark}}\xspace}
\def\Dss     {{\ensuremath{\D^{*+}_\squark}}\xspace}
\def\Dssp    {{\ensuremath{\D^{*+}_\squark}}\xspace}
\def\Dssm    {{\ensuremath{\D^{*-}_\squark}}\xspace}
\def\Dsspm   {{\ensuremath{\D^{*\pm}_\squark}}\xspace}
\def\Dssmp   {{\ensuremath{\D^{*\mp}_\squark}}\xspace}
\def\DporDsp {{\ensuremath{\D_{(\squark)}^+}}\xspace}
\def\DmorDsm {{\ensuremath{\D{}_{(\squark)}^-}}\xspace}
\def\DpmorDspm {{\ensuremath{\D{}_{(\squark)}^\pm}}\xspace}

%% Beauty mesons
\def\B       {{\ensuremath{\PB}}\xspace}
\def\Bbar    {{\ensuremath{\offsetoverline{\PB}}}\xspace}
\def\Bb      {{\ensuremath{\Bbar}}\xspace}
\def\BorBbar {\kern \thebaroffset\optbar{\kern -\thebaroffset \PB}\xspace}
\def\Bz      {{\ensuremath{\B^0}}\xspace}
\def\Bzb     {{\ensuremath{\Bbar{}^0}}\xspace}
\def\Bd      {{\ensuremath{\B^0}}\xspace}
\def\Bdb     {{\ensuremath{\Bbar{}^0}}\xspace}
\def\BdorBdbar {\kern \thebaroffset\optbar{\kern -\thebaroffset \Bd}\xspace}
\def\Bu      {{\ensuremath{\B^+}}\xspace}
\def\Bub     {{\ensuremath{\B^-}}\xspace}
\def\Bp      {{\ensuremath{\Bu}}\xspace}
\def\Bm      {{\ensuremath{\Bub}}\xspace}
\def\Bpm     {{\ensuremath{\B^\pm}}\xspace}
\def\Bmp     {{\ensuremath{\B^\mp}}\xspace}
\def\Bs      {{\ensuremath{\B^0_\squark}}\xspace}
\def\Bsb     {{\ensuremath{\Bbar{}^0_\squark}}\xspace}
\def\BsorBsbar {\kern \thebaroffset\optbar{\kern -\thebaroffset \Bs}\xspace}
\def\Bc      {{\ensuremath{\B_\cquark^+}}\xspace}
\def\Bcp     {{\ensuremath{\B_\cquark^+}}\xspace}
\def\Bcm     {{\ensuremath{\B_\cquark^-}}\xspace}
\def\Bcpm    {{\ensuremath{\B_\cquark^\pm}}\xspace}
\def\Bds     {{\ensuremath{\B_{(\squark)}^0}}\xspace}
\def\Bdsb    {{\ensuremath{\Bbar{}_{(\squark)}^0}}\xspace}
\def\BdorBs  {\Bds}
\def\BdorBsbar  {\Bdsb}

%% Onia

\def\jpsi     {{\ensuremath{{\PJ\mskip -3mu/\mskip -2mu\Ppsi}}}\xspace}
\def\psitwos  {{\ensuremath{\Ppsi{(2S)}}}\xspace}
\def\psiprpr  {{\ensuremath{\Ppsi(3770)}}\xspace}
\def\etac     {{\ensuremath{\Peta_\cquark}}\xspace}
\def\psires  {{\ensuremath{\Ppsi}}\xspace}
\def\chic     {{\ensuremath{\Pchi_\cquark}}\xspace}
\def\chiczero {{\ensuremath{\Pchi_{\cquark 0}}}\xspace}
\def\chicone  {{\ensuremath{\Pchi_{\cquark 1}}}\xspace}
\def\chictwo  {{\ensuremath{\Pchi_{\cquark 2}}}\xspace}
\def\chicJ    {{\ensuremath{\Pchi_{\cquark J}}}\xspace}
\def\Upsilonres  {{\ensuremath{\PUpsilon}}\xspace}
\def\Y#1S{\ensuremath{\PUpsilon{(#1S)}}\xspace}
\def\OneS  {{\Y1S}\xspace}
\def\TwoS  {{\Y2S}\xspace}
\def\ThreeS{{\Y3S}\xspace}
\def\FourS {{\Y4S}\xspace}
\def\FiveS {{\Y5S}\xspace}
\def\chib     {{\ensuremath{\Pchi_{b}}}\xspace}
\def\chibzero {{\ensuremath{\Pchi_{\bquark 0}}}\xspace}
\def\chibone  {{\ensuremath{\Pchi_{\bquark 1}}}\xspace}
\def\chibtwo  {{\ensuremath{\Pchi_{\bquark 2}}}\xspace}
\def\chibJ    {{\ensuremath{\Pchi_{\bquark J}}}\xspace}
\def\theX     {{\ensuremath{\Pchi_{c1}(3872)}}\xspace}

%% Light Baryons

\def\proton      {{\ensuremath{\Pp}}\xspace}
\def\antiproton  {{\ensuremath{\overline \proton}}\xspace}
\def\neutron     {{\ensuremath{\Pn}}\xspace}
\def\antineutron {{\ensuremath{\overline \neutron}}\xspace}
\def\Deltares    {{\ensuremath{\PDelta}}\xspace}
\def\Deltaresbar {{\ensuremath{\overline \Deltares}}\xspace}
%%% uds singlet
\def\Lz          {{\ensuremath{\PLambda}}\xspace}
\def\Lbar        {{\ensuremath{\offsetoverline{\PLambda}}}\xspace}
\def\LorLbar     {\kern \thebaroffset\optbar{\kern -\thebaroffset \PLambda}\xspace}
\def\Lambdares   {{\ensuremath{\PLambda}}\xspace}
\def\Lambdaresbar{{\ensuremath{\Lbar}}\xspace}
%%% uus, uds, dds
\def\Sigmares    {{\ensuremath{\PSigma}}\xspace}
\def\Sigmaz      {{\ensuremath{\Sigmares{}^0}}\xspace}
\def\Sigmap      {{\ensuremath{\Sigmares{}^+}}\xspace}
\def\Sigmam      {{\ensuremath{\Sigmares{}^-}}\xspace}
\def\Sigmaresbar {{\ensuremath{\offsetoverline{\Sigmares}}}\xspace}
\def\Sigmabarz   {{\ensuremath{\Sigmaresbar{}^0}}\xspace}
\def\Sigmabarp   {{\ensuremath{\Sigmaresbar{}^+}}\xspace}
\def\Sigmabarm   {{\ensuremath{\Sigmaresbar{}^-}}\xspace}
%%%  uss, dss
\def\Xires       {{\ensuremath{\PXi}}\xspace}
\def\Xiz         {{\ensuremath{\Xires^0}}\xspace}
\def\Xim         {{\ensuremath{\Xires^-}}\xspace}
\def\Xiresbar       {{\ensuremath{\offsetoverline{\Xires}}}\xspace}
\def\Xibarz      {{\ensuremath{\Xiresbar^0}}\xspace}
\def\Xibarp      {{\ensuremath{\Xiresbar^+}}\xspace}
%%%  sss
\def\Omegares    {{\ensuremath{\POmega}}\xspace}
\def\Omegaresbar {{\ensuremath{\offsetoverline{\POmega}}}\xspace}
\def\Omegam      {{\ensuremath{\Omegares^-}}\xspace}
\def\Omegabarp   {{\ensuremath{\Omegaresbar^+}}\xspace}

%% Charmed Baryons
\def\Lc          {{\ensuremath{\Lz^+_\cquark}}\xspace}
\def\Lcbar       {{\ensuremath{\Lbar{}^-_\cquark}}\xspace}
\def\Sigmac       {{\ensuremath{\Sigmares_\cquark}}\xspace}
\def\Sigmacp      {{\ensuremath{\Sigmares_\cquark^+}}\xspace}
\def\Sigmacz      {{\ensuremath{\Sigmares_\cquark^0}}\xspace}
\def\Sigmacpp      {{\ensuremath{\Sigmares_\cquark^{++}}}\xspace}
\def\Sigmacbar    {{\ensuremath{\Sigmaresbar_\cquark}}\xspace}
\def\Sigmacbarp   {{\ensuremath{\Sigmaresbar_\cquark^{--}}}\xspace}
\def\Sigmacbarz   {{\ensuremath{\Sigmaresbar_\cquark^0}}\xspace}
\def\Sigmacbarm   {{\ensuremath{\Sigmaresbar_\cquark^-}}\xspace}
\def\Xic         {{\ensuremath{\Xires_\cquark}}\xspace}
\def\Xicz        {{\ensuremath{\Xires^0_\cquark}}\xspace}
\def\Xicp        {{\ensuremath{\Xires^+_\cquark}}\xspace}
\def\Xicbar      {{\ensuremath{\Xiresbar{}_\cquark}}\xspace}
\def\Xicbarz     {{\ensuremath{\Xiresbar{}_\cquark^0}}\xspace}
\def\Xicbarm     {{\ensuremath{\Xiresbar{}_\cquark^-}}\xspace}
\def\Omegac      {{\ensuremath{\Omegares^0_\cquark}}\xspace}
\def\Omegacbar   {{\ensuremath{\Omegaresbar{}_\cquark^0}}\xspace}
\def\Xicc        {{\ensuremath{\Xires_{\cquark\cquark}}}\xspace}
\def\Xiccbar     {{\ensuremath{\Xiresbar{}_{\cquark\cquark}}}\xspace}
\def\Xiccp       {{\ensuremath{\Xires^+_{\cquark\cquark}}}\xspace}
\def\Xiccpp      {{\ensuremath{\Xires^{++}_{\cquark\cquark}}}\xspace}
\def\Xiccbarm    {{\ensuremath{\Xiresbar{}_{\cquark\cquark}^-}}\xspace}
\def\Xiccbarmm   {{\ensuremath{\Xiresbar{}_{\cquark\cquark}^{--}}}\xspace}
\def\Omegacc     {{\ensuremath{\Omegares^+_{\cquark\cquark}}}\xspace}
\def\Omegaccbar  {{\ensuremath{\Omegaresbar{}_{\cquark\cquark}^-}}\xspace}
\def\Omegaccc    {{\ensuremath{\Omegares^{++}_{\cquark\cquark\cquark}}}\xspace}
\def\Omegacccbar {{\ensuremath{\Omegaresbar{}_{\cquark\cquark\cquark}^{--}}}\xspace}
%% Beauty Baryons

\def\Lb           {{\ensuremath{\Lz^0_\bquark}}\xspace}
\def\Lbbar        {{\ensuremath{\Lbar{}^0_\bquark}}\xspace}
\def\Sigmab       {{\ensuremath{\Sigmares_\bquark}}\xspace}
\def\Sigmabp      {{\ensuremath{\Sigmares_\bquark^+}}\xspace}
\def\Sigmabz      {{\ensuremath{\Sigmares_\bquark^0}}\xspace}
\def\Sigmabm      {{\ensuremath{\Sigmares_\bquark^-}}\xspace}
\def\Sigmabpm     {{\ensuremath{\Sigmares_\bquark^\pm}}\xspace}
\def\Sigmabbar    {{\ensuremath{\Sigmaresbar_\bquark}}\xspace}
\def\Sigmabbarp   {{\ensuremath{\Sigmaresbar_\bquark^+}}\xspace}
\def\Sigmabbarz   {{\ensuremath{\Sigmaresbar_\bquark^0}}\xspace}
\def\Sigmabbarm   {{\ensuremath{\Sigmaresbar_\bquark^-}}\xspace}
\def\Sigmabbarpm  {{\ensuremath{\Sigmaresbar_\bquark^-}}\xspace}
\def\Xib          {{\ensuremath{\Xires_\bquark}}\xspace}
\def\Xibz         {{\ensuremath{\Xires^0_\bquark}}\xspace}
\def\Xibm         {{\ensuremath{\Xires^-_\bquark}}\xspace}
\def\Xibbar       {{\ensuremath{\Xiresbar{}_\bquark}}\xspace}
\def\Xibbarz      {{\ensuremath{\Xiresbar{}_\bquark^0}}\xspace}
\def\Xibbarp      {{\ensuremath{\Xiresbar{}_\bquark^+}}\xspace}
\def\Omegab       {{\ensuremath{\Omegares^-_\bquark}}\xspace}
\def\Omegabbar    {{\ensuremath{\Omegaresbar{}_\bquark^+}}\xspace}

%%%%%%%%%%%%%%%%%%
% Physics symbols
%%%%%%%%%%%%%%%%%

%% Decays
\def\BF         {{\ensuremath{\mathcal{B}}}\xspace}
\def\BR         {\BF}
\def\BRvis      {{\ensuremath{\BR_{\mathrm{{vis}}}}}}
\newcommand{\decay}[2]{\mbox{\ensuremath{#1\!\to #2}}\xspace} 
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}

%% Lifetimes
\newcommand{\tauBs}{{\ensuremath{\tau_{\Bs}}}\xspace}
\newcommand{\tauBd}{{\ensuremath{\tau_{\Bd}}}\xspace}
\newcommand{\tauBz}{{\ensuremath{\tau_{\Bz}}}\xspace}
\newcommand{\tauBu}{{\ensuremath{\tau_{\Bp}}}\xspace}
\newcommand{\tauDp}{{\ensuremath{\tau_{\Dp}}}\xspace}
\newcommand{\tauDz}{{\ensuremath{\tau_{\Dz}}}\xspace}
\newcommand{\tauL}{{\ensuremath{\tau_{\mathrm{ L}}}}\xspace}
\newcommand{\tauH}{{\ensuremath{\tau_{\mathrm{ H}}}}\xspace}

%% Masses
\newcommand{\mBd}{{\ensuremath{m_{\Bd}}}\xspace}
\newcommand{\mBp}{{\ensuremath{m_{\Bp}}}\xspace}
\newcommand{\mBs}{{\ensuremath{m_{\Bs}}}\xspace}
\newcommand{\mBc}{{\ensuremath{m_{\Bc}}}\xspace}
\newcommand{\mLb}{{\ensuremath{m_{\Lb}}}\xspace}

%% EW theory, groups
\def\grpsuthree {{\ensuremath{\mathrm{SU}(3)}}\xspace}
\def\grpsutw    {{\ensuremath{\mathrm{SU}(2)}}\xspace}
\def\grpuone    {{\ensuremath{\mathrm{U}(1)}}\xspace}

\def\ssqtw   {{\ensuremath{\sin^{2}\!\theta_{\mathrm{W}}}}\xspace}
\def\csqtw   {{\ensuremath{\cos^{2}\!\theta_{\mathrm{W}}}}\xspace}
\def\stw     {{\ensuremath{\sin\theta_{\mathrm{W}}}}\xspace}
\def\ctw     {{\ensuremath{\cos\theta_{\mathrm{W}}}}\xspace}
\def\ssqtwef {{\ensuremath{{\sin}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\csqtwef {{\ensuremath{{\cos}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\stwef   {{\ensuremath{\sin\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\ctwef   {{\ensuremath{\cos\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\gv      {{\ensuremath{g_{\mbox{\tiny V}}}}\xspace}
\def\ga      {{\ensuremath{g_{\mbox{\tiny A}}}}\xspace}

\def\order   {{\ensuremath{\mathcal{O}}}\xspace}
\def\ordalph {{\ensuremath{\mathcal{O}(\alpha)}}\xspace}
\def\ordalsq {{\ensuremath{\mathcal{O}(\alpha^{2})}}\xspace}
\def\ordalcb {{\ensuremath{\mathcal{O}(\alpha^{3})}}\xspace}

%% QCD parameters
\newcommand{\as}{{\ensuremath{\alpha_s}}\xspace}
\newcommand{\MSb}{{\ensuremath{\overline{\mathrm{MS}}}}\xspace}
\newcommand{\lqcd}{{\ensuremath{\Lambda_{\mathrm{QCD}}}}\xspace}
\def\qsq       {{\ensuremath{q^2}}\xspace}

%% CKM, \boldmath \CP violation

\def\eps   {{\ensuremath{\varepsilon}}\xspace}
\def\epsK  {{\ensuremath{\varepsilon_K}}\xspace}
\def\epsB  {{\ensuremath{\varepsilon_B}}\xspace}
\def\epsp  {{\ensuremath{\varepsilon^\prime_K}}\xspace}

\def\CP                {{\ensuremath{C\!P}}\xspace}
\def\CPT               {{\ensuremath{C\!PT}}\xspace}
\def\T                 {{\ensuremath{T}}\xspace}

\def\rhobar {{\ensuremath{\overline \rho}}\xspace}
\def\etabar {{\ensuremath{\overline \eta}}\xspace}

\def\Vud  {{\ensuremath{V_{\uquark\dquark}^{\phantom{\ast}}}}\xspace}
\def\Vcd  {{\ensuremath{V_{\cquark\dquark}^{\phantom{\ast}}}}\xspace}
\def\Vtd  {{\ensuremath{V_{\tquark\dquark}^{\phantom{\ast}}}}\xspace}
\def\Vus  {{\ensuremath{V_{\uquark\squark}^{\phantom{\ast}}}}\xspace}
\def\Vcs  {{\ensuremath{V_{\cquark\squark}^{\phantom{\ast}}}}\xspace}
\def\Vts  {{\ensuremath{V_{\tquark\squark}^{\phantom{\ast}}}}\xspace}
\def\Vub  {{\ensuremath{V_{\uquark\bquark}^{\phantom{\ast}}}}\xspace}
\def\Vcb  {{\ensuremath{V_{\cquark\bquark}^{\phantom{\ast}}}}\xspace}
\def\Vtb  {{\ensuremath{V_{\tquark\bquark}^{\phantom{\ast}}}}\xspace}
\def\Vuds  {{\ensuremath{V_{\uquark\dquark}^\ast}}\xspace}
\def\Vcds  {{\ensuremath{V_{\cquark\dquark}^\ast}}\xspace}
\def\Vtds  {{\ensuremath{V_{\tquark\dquark}^\ast}}\xspace}
\def\Vuss  {{\ensuremath{V_{\uquark\squark}^\ast}}\xspace}
\def\Vcss  {{\ensuremath{V_{\cquark\squark}^\ast}}\xspace}
\def\Vtss  {{\ensuremath{V_{\tquark\squark}^\ast}}\xspace}
\def\Vubs  {{\ensuremath{V_{\uquark\bquark}^\ast}}\xspace}
\def\Vcbs  {{\ensuremath{V_{\cquark\bquark}^\ast}}\xspace}
\def\Vtbs  {{\ensuremath{V_{\tquark\bquark}^\ast}}\xspace}

%% Oscillations

\newcommand{\dm}{{\ensuremath{\Delta m}}\xspace}
\newcommand{\dms}{{\ensuremath{\Delta m_{\squark}}}\xspace}
\newcommand{\dmd}{{\ensuremath{\Delta m_{\dquark}}}\xspace}
\newcommand{\DG}{{\ensuremath{\Delta\Gamma}}\xspace}
\newcommand{\DGs}{{\ensuremath{\Delta\Gamma_{\squark}}}\xspace}
\newcommand{\DGd}{{\ensuremath{\Delta\Gamma_{\dquark}}}\xspace}
\newcommand{\Gs}{{\ensuremath{\Gamma_{\squark}}}\xspace}
\newcommand{\Gd}{{\ensuremath{\Gamma_{\dquark}}}\xspace}
\newcommand{\MBq}{{\ensuremath{M_{\B_\quark}}}\xspace}
\newcommand{\DGq}{{\ensuremath{\Delta\Gamma_{\quark}}}\xspace}
\newcommand{\Gq}{{\ensuremath{\Gamma_{\quark}}}\xspace}
\newcommand{\dmq}{{\ensuremath{\Delta m_{\quark}}}\xspace}
\newcommand{\GL}{{\ensuremath{\Gamma_{\mathrm{ L}}}}\xspace}
\newcommand{\GH}{{\ensuremath{\Gamma_{\mathrm{ H}}}}\xspace}
\newcommand{\DGsGs}{{\ensuremath{\Delta\Gamma_{\squark}/\Gamma_{\squark}}}\xspace}
\newcommand{\Delm}{{\mbox{$\Delta m $}}\xspace}
\newcommand{\ACP}{{\ensuremath{{\mathcal{A}}^{\CP}}}\xspace}
\newcommand{\Adir}{{\ensuremath{{\mathcal{A}}^{\mathrm{ dir}}}}\xspace}
\newcommand{\Amix}{{\ensuremath{{\mathcal{A}}^{\mathrm{ mix}}}}\xspace}
\newcommand{\ADelta}{{\ensuremath{{\mathcal{A}}^\Delta}}\xspace}
\newcommand{\phid}{{\ensuremath{\phi_{\dquark}}}\xspace}
\newcommand{\sinphid}{{\ensuremath{\sin\!\phid}}\xspace}
\newcommand{\phis}{{\ensuremath{\phi_{\squark}}}\xspace}
\newcommand{\betas}{{\ensuremath{\beta_{\squark}}}\xspace}
\newcommand{\sbetas}{{\ensuremath{\sigma(\beta_{\squark})}}\xspace}
\newcommand{\stbetas}{{\ensuremath{\sigma(2\beta_{\squark})}}\xspace}
\newcommand{\stphis}{{\ensuremath{\sigma(\phi_{\squark})}}\xspace}
\newcommand{\sinphis}{{\ensuremath{\sin\!\phis}}\xspace}

%% Tagging
\newcommand{\edet}{{\ensuremath{\varepsilon_{\mathrm{ det}}}}\xspace}
\newcommand{\erec}{{\ensuremath{\varepsilon_{\mathrm{ rec/det}}}}\xspace}
\newcommand{\esel}{{\ensuremath{\varepsilon_{\mathrm{ sel/rec}}}}\xspace}
\newcommand{\etrg}{{\ensuremath{\varepsilon_{\mathrm{ trg/sel}}}}\xspace}
\newcommand{\etot}{{\ensuremath{\varepsilon_{\mathrm{ tot}}}}\xspace}

\newcommand{\mistag}{\ensuremath{\omega}\xspace}
\newcommand{\wcomb}{\ensuremath{\omega^{\mathrm{comb}}}\xspace}
\newcommand{\etag}{{\ensuremath{\varepsilon_{\mathrm{tag}}}}\xspace}
\newcommand{\etagcomb}{{\ensuremath{\varepsilon_{\mathrm{tag}}^{\mathrm{comb}}}}\xspace}
\newcommand{\effeff}{\ensuremath{\varepsilon_{\mathrm{eff}}}\xspace}
\newcommand{\effeffcomb}{\ensuremath{\varepsilon_{\mathrm{eff}}^{\mathrm{comb}}}\xspace}
\newcommand{\efftag}{{\ensuremath{\etag(1-2\omega)^2}}\xspace}
\newcommand{\effD}{{\ensuremath{\etag D^2}}\xspace}

\newcommand{\etagprompt}{{\ensuremath{\varepsilon_{\mathrm{ tag}}^{\mathrm{Pr}}}}\xspace}
\newcommand{\etagLL}{{\ensuremath{\varepsilon_{\mathrm{ tag}}^{\mathrm{LL}}}}\xspace}

%% Key decay channels

\def\BdToKstmm    {\decay{\Bd}{\Kstarz\mup\mun}}
\def\BdbToKstmm   {\decay{\Bdb}{\Kstarzb\mup\mun}}

\def\BsToJPsiPhi  {\decay{\Bs}{\jpsi\phi}}
\def\BdToJPsiKst  {\decay{\Bd}{\jpsi\Kstarz}}
\def\BdbToJPsiKst {\decay{\Bdb}{\jpsi\Kstarzb}}

\def\BsPhiGam     {\decay{\Bs}{\phi \g}}
\def\BdKstGam     {\decay{\Bd}{\Kstarz \g}}

\def\BTohh        {\decay{\B}{\Ph^+ \Ph'^-}}
\def\BdTopipi     {\decay{\Bd}{\pip\pim}}
\def\BdToKpi      {\decay{\Bd}{\Kp\pim}}
\def\BsToKK       {\decay{\Bs}{\Kp\Km}}
\def\BsTopiK      {\decay{\Bs}{\pip\Km}}
\def\Cpipi        {\ensuremath{C_{\pip\pim}}\xspace}
\def\Spipi        {\ensuremath{S_{\pip\pim}}\xspace}
\def\CKK          {\ensuremath{C_{\Kp\Km}}\xspace}
\def\SKK          {\ensuremath{S_{\Kp\Km}}\xspace}
\def\ADGKK        {\ensuremath{A^{\DG}_{\Kp\Km}}\xspace}

%% Rare decays
\def\BdKstee  {\decay{\Bd}{\Kstarz\epem}}
\def\BdbKstee {\decay{\Bdb}{\Kstarzb\epem}}
\def\bsll     {\decay{\bquark}{\squark \ell^+ \ell^-}}
\def\AFB      {\ensuremath{A_{\mathrm{FB}}}\xspace}
\def\FL       {\ensuremath{F_{\mathrm{L}}}\xspace}
\def\AT#1     {\ensuremath{A_{\mathrm{T}}^{#1}}\xspace}           % 2
\def\btosgam  {\decay{\bquark}{\squark \g}}
\def\btodgam  {\decay{\bquark}{\dquark \g}}
\def\Bsmm     {\decay{\Bs}{\mup\mun}}
\def\Bdmm     {\decay{\Bd}{\mup\mun}}
\def\Bsee     {\decay{\Bs}{\epem}}
\def\Bdee     {\decay{\Bd}{\epem}}
\def\ctl       {\ensuremath{\cos{\theta_\ell}}\xspace}
\def\ctk       {\ensuremath{\cos{\theta_K}}\xspace}

%% Wilson coefficients and operators
\def\C#1      {\ensuremath{\mathcal{C}_{#1}}\xspace}                       % 9
\def\Cp#1     {\ensuremath{\mathcal{C}_{#1}^{'}}\xspace}                    % 7
\def\Ceff#1   {\ensuremath{\mathcal{C}_{#1}^{\mathrm{(eff)}}}\xspace}        % 9  
\def\Cpeff#1  {\ensuremath{\mathcal{C}_{#1}^{'\mathrm{(eff)}}}\xspace}       % 7
\def\Ope#1    {\ensuremath{\mathcal{O}_{#1}}\xspace}                       % 2
\def\Opep#1   {\ensuremath{\mathcal{O}_{#1}^{'}}\xspace}                    % 7

%% Charm

\def\xprime     {\ensuremath{x^{\prime}}\xspace}
\def\yprime     {\ensuremath{y^{\prime}}\xspace}
\def\ycp        {\ensuremath{y_{\CP}}\xspace}
\def\agamma     {\ensuremath{A_{\Gamma}}\xspace}
%%%\def\kpi        {\ensuremath{\PK\Ppi}\xspace}
%%%\def\kk         {\ensuremath{\PK\PK}\xspace}
%%%\def\dkpi       {\decay{\PD}{\PK\Ppi}}
%%%\def\dkk        {\decay{\PD}{\PK\PK}}
\def\dkpicf     {\decay{\Dz}{\Km\pip}}

%% QM
\newcommand{\bra}[1]{\ensuremath{\langle #1|}}             % {a}
\newcommand{\ket}[1]{\ensuremath{|#1\rangle}}              % {b}
\newcommand{\braket}[2]{\ensuremath{\langle #1|#2\rangle}} % {a}{b}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Units (these macros add a small space in front)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\nospaceunit}[1]{\ensuremath{\text{#1}}}       
\newcommand{\aunit}[1]{\ensuremath{\text{\,#1}}}       
%%% the following conflicts with siunitx package
%%% \newcommand{\unit}[1]{\aunit{#1}\xspace}                   % {kg}   

%% Energy and momentum 
\newcommand{\tev}{\aunit{Te\kern -0.1em V}\xspace}
\newcommand{\gev}{\aunit{Ge\kern -0.1em V}\xspace}
\newcommand{\mev}{\aunit{Me\kern -0.1em V}\xspace}
\newcommand{\kev}{\aunit{ke\kern -0.1em V}\xspace}
\newcommand{\ev}{\aunit{e\kern -0.1em V}\xspace}
\newcommand{\gevgev}{\ensuremath{\gev^2}\xspace} 
\newcommand{\mevc}{\ensuremath{\aunit{Me\kern -0.1em V\!/}c}\xspace}
\newcommand{\gevc}{\ensuremath{\aunit{Ge\kern -0.1em V\!/}c}\xspace}
\newcommand{\mevcc}{\ensuremath{\aunit{Me\kern -0.1em V\!/}c^2}\xspace}
\newcommand{\gevcc}{\ensuremath{\aunit{Ge\kern -0.1em V\!/}c^2}\xspace}
\newcommand{\gevgevcc}{\ensuremath{\gev^2\!/c^2}\xspace} % for \pt^2 in CEP
\newcommand{\gevgevcccc}{\ensuremath{\gev^2\!/c^4}\xspace} % for q^2

%% Distance and area (these macros add a small space)
\def\km   {\aunit{km}\xspace}
\def\m    {\aunit{m}\xspace}
\def\ma   {\ensuremath{\aunit{m}^2}\xspace}
\def\cm   {\aunit{cm}\xspace}
\def\cma  {\ensuremath{\aunit{cm}^2}\xspace}
\def\mm   {\aunit{mm}\xspace}
\def\mma  {\ensuremath{\aunit{mm}^2}\xspace}
\def\mum  {\ensuremath{\,\upmu\nospaceunit{m}}\xspace}
\def\muma {\ensuremath{\,\upmu\nospaceunit{m}^2}\xspace}
\def\nm   {\aunit{nm}\xspace}
\def\fm   {\aunit{fm}\xspace}
\def\barn{\aunit{b}\xspace}
%%%\def\barnhyph{\ensuremath{\mathrm{ -b}}
\def\mbarn{\aunit{mb}\xspace}
\def\mub{\ensuremath{\,\upmu\nospaceunit{b}}\xspace}
%%%\def\mbarnhyph{\ensuremath{\mathrm{ -mb}}
\def\nb {\aunit{nb}\xspace}
\def\invnb {\ensuremath{\nb^{-1}}\xspace}
\def\pb {\aunit{pb}\xspace}
\def\invpb {\ensuremath{\pb^{-1}}\xspace}
\def\fb   {\ensuremath{\aunit{fb}}\xspace}
\def\invfb   {\ensuremath{\fb^{-1}}\xspace}
\def\ab   {\ensuremath{\aunit{ab}}\xspace}
\def\invab   {\ensuremath{\ab^{-1}}\xspace}

%% Time 
\def\sec  {\ensuremath{\aunit{s}}\xspace}
\def\ms   {\ensuremath{\aunit{ms}}\xspace}
\def\mus  {\ensuremath{\,\upmu\nospaceunit{s}}\xspace}
\def\ns   {\ensuremath{\aunit{ns}}\xspace}
\def\ps   {\ensuremath{\aunit{ps}}\xspace}
\def\fs   {\aunit{fs}}

\def\mhz  {\ensuremath{\aunit{MHz}}\xspace}
\def\khz  {\ensuremath{\aunit{kHz}}\xspace}
\def\hz   {\ensuremath{\aunit{Hz}}\xspace}

\def\invps{\ensuremath{\ps^{-1}}\xspace}
\def\invns{\ensuremath{\ns^{-1}}\xspace}

\def\yr   {\aunit{yr}\xspace}
\def\hr   {\aunit{hr}\xspace}

%% Temperature
\def\degc {\ensuremath{^\circ}{\text{C}}\xspace}
\def\degk {\aunit{K}\xspace}

%% Material lengths, radiation
\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{\rm int}}\xspace}
\def\mip {MIP\xspace}
\def\neutroneq {\ensuremath{n_\nospaceunit{eq}}\xspace}
\def\neqcmcm {\ensuremath{\neutroneq/\nospaceunit{cm}^2}\xspace}
\def\kRad {\aunit{kRad}\xspace}
\def\MRad {\aunit{MRad}\xspace}
\def\ci {\aunit{Ci}\xspace}
\def\mci {\aunit{mCi}\xspace}

%% Uncertainties
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    

\newcommand{\stat}{\aunit{(stat)}\xspace}
\newcommand{\syst}{\aunit{(syst)}\xspace}
\newcommand{\lumi}{\aunit{(lumi)}\xspace}

%% Maths

\def\order{{\ensuremath{\mathcal{O}}}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\chisqndf}{\ensuremath{\chi^2/\mathrm{ndf}}\xspace}
\newcommand{\chisqip}{\ensuremath{\chi^2_{\text{IP}}}\xspace}
\newcommand{\chisqfd}{\ensuremath{\chi^2_{\text{FD}}}\xspace}
\newcommand{\chisqvs}{\ensuremath{\chi^2_{\text{VS}}}\xspace}
\newcommand{\chisqvtx}{\ensuremath{\chi^2_{\text{vtx}}}\xspace}
\newcommand{\chisqvtxndf}{\ensuremath{\chi^2_{\text{vtx}}/\mathrm{ndf}}\xspace}

\def\deriv {\ensuremath{\mathrm{d}}}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\newcommand{\mean}[1]{\ensuremath{\left\langle #1 \right\rangle}} % {x}
\newcommand{\abs}[1]{\ensuremath{\left\|#1\right\|}} % {x}
\newcommand{\Real}{\ensuremath{\mathcal{R}e}\xspace}
\newcommand{\Imag}{\ensuremath{\mathcal{I}m}\xspace}

\def\PDF {PDF\xspace}

\def\sPlot{\mbox{\em sPlot}\xspace}
\def\sFit{\mbox{\em sFit}\xspace}
%%%\def\sWeight{\mbox{\em sWeight}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Kinematics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Energy, Momenta
\def\Ebeam {\ensuremath{E_{\mbox{\tiny BEAM}}}\xspace}
\def\sqs   {\ensuremath{\protect\sqrt{s}}\xspace}
\def\sqsnn {\ensuremath{\protect\sqrt{s_{\scriptscriptstyle\text{NN}}}}\xspace}
\def\pt         {\ensuremath{p_{\mathrm{T}}}\xspace}
\def\ptsq       {\ensuremath{p_{\mathrm{T}}^2}\xspace}
\def\ptot       {\ensuremath{p}\xspace}
\def\et         {\ensuremath{E_{\mathrm{T}}}\xspace}
\def\mt         {\ensuremath{M_{\mathrm{T}}}\xspace}
\def\dpp        {\ensuremath{\Delta p/p}\xspace}
\def\msq        {\ensuremath{m^2}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
%% PID
\def\dllkpi     {\ensuremath{\mathrm{DLL}_{\kaon\pion}}\xspace}
\def\dllppi     {\ensuremath{\mathrm{DLL}_{\proton\pion}}\xspace}
\def\dllepi     {\ensuremath{\mathrm{DLL}_{\electron\pion}}\xspace}
\def\dllmupi    {\ensuremath{\mathrm{DLL}_{\muon\pi}}\xspace}
%% Geometry
%%%\def\mphi       {\mbox{$\phi$}\xspace}
%%%\def\mtheta     {\mbox{$\theta$}\xspace}
%%%\def\ctheta     {\mbox{$\cos\theta$}\xspace}
%%%\def\stheta     {\mbox{$\sin\theta$}\xspace}
%%%\def\ttheta     {\mbox{$\tan\theta$}\xspace}

\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\murad{\ensuremath{\,\upmu\nospaceunit{rad}}\xspace}
\def\mrad{\aunit{mrad}\xspace}
\def\rad{\aunit{rad}\xspace}

%% Accelerator
\def\betastar {\ensuremath{\beta^*}}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}
\newcommand{\intlum}[1]{\ensuremath{\int\lum=#1}\xspace}  % {2 \,\invfb}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Software
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Programs
%%%\def\ansys      {\mbox{\textsc{Ansys}}\xspace}
\def\bcvegpy    {\mbox{\textsc{Bcvegpy}}\xspace}
\def\boole      {\mbox{\textsc{Boole}}\xspace}
\def\brunel     {\mbox{\textsc{Brunel}}\xspace}
\def\davinci    {\mbox{\textsc{DaVinci}}\xspace}
\def\dirac      {\mbox{\textsc{Dirac}}\xspace}
%%%\def\erasmus    {\mbox{\textsc{Erasmus}}\xspace}
\def\evtgen     {\mbox{\textsc{EvtGen}}\xspace}
\def\fewz       {\mbox{\textsc{Fewz}}\xspace}
\def\fluka      {\mbox{\textsc{Fluka}}\xspace}
\def\ganga      {\mbox{\textsc{Ganga}}\xspace}
%%%\def\garfield   {\mbox{\textsc{Garfield}}\xspace}
\def\gaudi      {\mbox{\textsc{Gaudi}}\xspace}
\def\gauss      {\mbox{\textsc{Gauss}}\xspace}
\def\geant      {\mbox{\textsc{Geant4}}\xspace}
\def\lamarr     {\mbox{\textsc{Lamarr}}\xspace}
\def\hepmc      {\mbox{\textsc{HepMC}}\xspace}
\def\herwig     {\mbox{\textsc{Herwig}}\xspace}
\def\moore      {\mbox{\textsc{Moore}}\xspace}
\def\neurobayes {\mbox{\textsc{NeuroBayes}}\xspace}
\def\photos     {\mbox{\textsc{Photos}}\xspace}
\def\powheg     {\mbox{\textsc{Powheg}}\xspace}
%%%\def\pyroot     {\mbox{\textsc{PyRoot}}\xspace}
\def\pythia     {\mbox{\textsc{Pythia}}\xspace}
\def\resbos     {\mbox{\textsc{ResBos}}\xspace}
\def\roofit     {\mbox{\textsc{RooFit}}\xspace}
\def\root       {\mbox{\textsc{Root}}\xspace}
\def\spice      {\mbox{\textsc{Spice}}\xspace}
%%%\def\tosca      {\mbox{\textsc{Tosca}}\xspace}
\def\tensorflow {\mbox{\textsc{TensorFlow}}\xspace}
\def\urania     {\mbox{\textsc{Urania}}\xspace}

%% Languages
\def\cpp        {\mbox{\textsc{C\raisebox{0.1em}{{\footnotesize{++}}}}}\xspace}
%%%\def\python     {\mbox{\textsc{Python}}\xspace}
\def\ruby       {\mbox{\textsc{Ruby}}\xspace}
\def\fortran    {\mbox{\textsc{Fortran}}\xspace}
\def\svn        {\mbox{\textsc{svn}}\xspace}
\def\git        {\mbox{\textsc{git}}\xspace}
\def\latex      {\mbox{\LaTeX}\xspace}

%% Data processing
\def\kbit          {\aunit{kbit}\xspace}
\def\kbps        {\aunit{kbit/s}\xspace}
\def\kbytes     {\aunit{kB}\xspace}
\def\kbyps      {\aunit{kB/s}\xspace}
\def\mbit          {\aunit{Mbit}\xspace}
\def\mbps        {\aunit{Mbit/s}\xspace}
\def\mbytes     {\aunit{MB}\xspace}
\def\mbyps      {\aunit{MB/s}\xspace}
\def\gbit          {\aunit{Gbit}\xspace}
\def\gbps        {\aunit{Gbit/s}\xspace}
\def\gbytes     {\aunit{GB}\xspace}
\def\gbyps      {\aunit{GB/s}\xspace}
\def\tbit          {\aunit{Tbit}\xspace}
\def\tbps        {\aunit{Tbit/s}\xspace}
\def\tbytes     {\aunit{TB}\xspace}
\def\tbyps      {\aunit{TB/s}\xspace}
\def\dst        {DST\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Detector related
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Detector technologies
\def\nonn {\ensuremath{\mathrm{{ \mathit{n^+}} \mbox{-} on\mbox{-}{ \mathit{n}}}}\xspace}
\def\ponn {\ensuremath{\mathrm{{ \mathit{p^+}} \mbox{-} on\mbox{-}{ \mathit{n}}}}\xspace}
\def\nonp {\ensuremath{\mathrm{{ \mathit{n^+}} \mbox{-} on\mbox{-}{ \mathit{p}}}}\xspace}
\def\cvd  {CVD\xspace}
\def\mwpc {MWPC\xspace}
\def\gem  {GEM\xspace}

%% Detector components, electronics
\def\tell1  {TELL1\xspace}
\def\ukl1   {UKL1\xspace}
\def\beetle {Beetle\xspace}
\def\otis   {OTIS\xspace}
\def\croc   {CROC\xspace}
\def\carioca {CARIOCA\xspace}
\def\dialog {DIALOG\xspace}
\def\sync   {SYNC\xspace}
\def\cardiac {CARDIAC\xspace}
\def\gol    {GOL\xspace}
\def\vcsel  {VCSEL\xspace}
\def\ttc    {TTC\xspace}
\def\ttcrx  {TTCrx\xspace}
\def\hpd    {HPD\xspace}
\def\pmt    {PMT\xspace}
\def\specs  {SPECS\xspace}
\def\elmb   {ELMB\xspace}
\def\fpga   {FPGA\xspace}
\def\plc    {PLC\xspace}
\def\rasnik {RASNIK\xspace}
\def\elmb   {ELMB\xspace}
\def\can    {CAN\xspace}
\def\lvds   {LVDS\xspace}
\def\ntc    {NTC\xspace}
\def\adc    {ADC\xspace}
\def\led    {LED\xspace}
\def\ccd    {CCD\xspace}
\def\hv     {HV\xspace}
\def\lv     {LV\xspace}
\def\pvss   {PVSS\xspace}
\def\cmos   {CMOS\xspace}
\def\fifo   {FIFO\xspace}
\def\ccpc   {CCPC\xspace}

%% Chemical symbols
\def\cfourften     {\ensuremath{\mathrm{ C_4 F_{10}}}\xspace}
\def\cffour        {\ensuremath{\mathrm{ CF_4}}\xspace}
\def\cotwo         {\ensuremath{\mathrm{ CO_2}}\xspace} 
\def\csixffouteen  {\ensuremath{\mathrm{ C_6 F_{14}}}\xspace} 
\def\mgftwo     {\ensuremath{\mathrm{ Mg F_2}}\xspace} 
\def\siotwo     {\ensuremath{\mathrm{ SiO_2}}\xspace} 

%%%%%%%%%%%%%%%
%% Special Text 
%%%%%%%%%%%%%%%
\newcommand{\eg}{\mbox{\itshape e.g.}\xspace}
\newcommand{\ie}{\mbox{\itshape i.e.}\xspace}
\newcommand{\etal}{\mbox{\itshape et al.}\xspace}
\newcommand{\etc}{\mbox{\itshape etc.}\xspace}
\newcommand{\cf}{\mbox{\itshape cf.}\xspace}
\newcommand{\ffp}{\mbox{\itshape ff.}\xspace}
\newcommand{\vs}{\mbox{\itshape vs.}\xspace}
%%%%%%%%%%%%%%%
%% Helpful to align numbers in tables
%%%%%%%%%%%%%%%
\newcommand{\phz}{\phantom{0}}
\newcommand{\lhcborcid}[1]{\href{https://orcid.org/#1}{\hspace*{0.1em}\raisebox{-0.45ex}{\includegraphics[width=1em]{figs/orcidIcon.pdf}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                                                                    %
%%% !!!!!!!!!!!!!!!!!!! DO NOT EDIT THIS FILE !!!!!!!!!!!!!!!!!!!!!!!! %
%%%                                                                    %
%%% THE EB MAY OVERWRITE IT TO REFLECT LATEST CHANGES IN THE TEMPLATE  %
%%%                                                                    %
%%% You may define your own macros and packages in main.tex or add     %
%%% additional local files                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
% Special Text 
%%%%%%%%%%%%%%%

\def\Mz     {{\ensuremath{M^0}}\xspace}
\def\Mp     {{\ensuremath{M^{+}}}\xspace}
\def\Mzg    {{\ensuremath{\Mz}{\g}}\xspace}
\def\Mpg    {{\ensuremath{\Mp}{\g}}\xspace}
\def\DzX    {{\ensuremath{\Dz}{X}}\xspace}
\def\Dspg   {{\ensuremath{\Dsp}{\g}}\xspace}
\def\Dsmg   {{\ensuremath{\Dsm}{\g}}\xspace}
\def\Dsg    {{\ensuremath{\Dspm}{\g}}\xspace}
\def\DsgFull{{\ensuremath{\Dspm(\to\Kp\Km\pip)}{\g}}\xspace}
\def\Dzg    {{\ensuremath{\Dz}{\g}}\xspace}
\def\DzgFull{{\ensuremath{\Dz(\to\Km\pip)}{\g}}\xspace}
\def\Jpg    {{\ensuremath{\jpsi}{\g}}\xspace}
\def\Upg    {{\ensuremath{\OneS}{\g}}\xspace}
\def\Phg    {{\ensuremath{\Pphi}{\g}}\xspace}
\def\Rhg    {{\ensuremath{\Prho}{\g}}\xspace} 
\def\gg     {{\ensuremath{\g}{\g}}\xspace}
\def\munu   {{\ensuremath{\mupm}{\neu}}\xspace}
\def\mpnu   {{\ensuremath{\mup}{\neu}}\xspace}
\def\mmnu   {{\ensuremath{\mun}{\neu}}\xspace}
\def\taumu  {{\ensuremath{\tauon}{\nu}}\xspace}

\def\DsFull{{\ensuremath{\Dspm\to\Kp\Km\pip}}\xspace}
\def\DzFull{{\ensuremath{\Dz\to\Km\pip}}\xspace}

\def\HMzg    {\decay{H}{\Mzg}}
\def\ZMzg    {\decay{\Z}{\Mzg}}
\def\WMpg    {\decay{\Wp}{\Mpg}}
\def\ZDzX    {\decay{\Z}{\DzX}}
\def\WDspg   {\decay{\Wp}{\Dspg}}
\def\WDsmg   {\decay{\Wm}{\Dsmg}}
\def\WDsg    {\decay{\Wpm}{\Dsg}}
\def\WDsgFull{{\Wpm}\to{\Dspm{(\to\Kp\Km\pip)}}{\g}\xspace}
%\def\WDsgFull{\decay{\Wpm}{\DsgFull}
\def\ZDzg    {\decay{\Z}{\Dzg}}
\def\ZDzgFull{{\Z}\to{\Dz{(\to\Km\pip)}}{\g}\xspace}
%\def\ZDzgFull{\decay{\Z}{\DzgFull}}
\def\ZJpg    {\decay{\Z}{\Jpg}}
\def\ZUpg    {\decay{\Z}{\Upg}}
\def\ZPhg    {\decay{\Z}{\Phg}}
\def\ZRhg    {\decay{\Z}{\Rhg}}
\def\Zgg     {\decay{\Z}{\gg}}
\def\Zmm     {\decay{\Z}{\mumu}} 
\def\Zm     {\decay{\Z}{\mu}} 
\def\wm     {\decay{\W}{\mu}} 
\def\Wmn     {\decay{\Wpm}{\munu}}
\def\Wmpn    {\decay{\Wp}{\mpnu}}
\def\Wmnn    {\decay{\Wm}{\mmnu}}
\def\Wtm     {\decay{\Wpm}{\taumu}}
\def\Ztt     {\decay{\Z}{\tautau}}
\def\bbxm    {\decay{\bbbar}{X\muon}}
\def\ccxm    {\decay{\ccbar}{X\muon}}
\def\ggtt    {\decay{\Pg\Pg}{\ttbar}}
\def\qqtt    {\decay{\quark\quark}{\ttbar}}
\def\imu     {I_{\mu}\xspace}

\def\PDeltap {\ensuremath{\Delta p}\xspace} 
\def\jet   {\text{jet}\xspace}
\def\cjet   {\ensuremath{\cquark\mathrm{\text{-jet}}}\xspace}
\def\bjet   {\ensuremath{\bquark\mathrm{\text{-jet}}}\xspace}
\def\mubpt {$p(\vec{j_{b}} + \vec{j_{\mu}})_{T}$}
\def\jmu    {$j_{\mu}$}
\def\jpb    {\ensuremath{P_{b}}\xspace}
\def\jpc    {\ensuremath{P_{c}}\xspace}
\def\jpq    {\ensuremath{P_{q}}\xspace}
%{\ensuremath{E_{\mathrm{T}}}\xspace}

==> lhcb_text/lhcb-symbols-list.tex <==
% This is an automatically generated appendix to template.tex. 
% When included it will show all the symbols defined in lhcb-symbols-def.tex.
%
% To regenerate with the latest definitions run the script python listsymbols.py

\section{List of all symbols}
\label{sec:listofsymbols}
\subsection{Experiments}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash lhcb} & \lhcb & \texttt{\textbackslash atlas} & \atlas & \texttt{\textbackslash cms} & \cms \\
\texttt{\textbackslash alice} & \alice & \texttt{\textbackslash babar} & \babar & \texttt{\textbackslash belle} & \belle \\
\texttt{\textbackslash belletwo} & \belletwo & \texttt{\textbackslash besiii} & \besiii & \texttt{\textbackslash cleo} & \cleo \\
\texttt{\textbackslash cdf} & \cdf & \texttt{\textbackslash dzero} & \dzero & \texttt{\textbackslash aleph} & \aleph \\
\texttt{\textbackslash delphi} & \delphi & \texttt{\textbackslash opal} & \opal & \texttt{\textbackslash lthree} & \lthree \\
\texttt{\textbackslash sld} & \sld & \texttt{\textbackslash cern} & \cern & \texttt{\textbackslash lhc} & \lhc \\
\texttt{\textbackslash lep} & \lep & \texttt{\textbackslash tevatron} & \tevatron & \texttt{\textbackslash bfactories} & \bfactories \\
\texttt{\textbackslash bfactory} & \bfactory & \texttt{\textbackslash upgradeone} & \upgradeone & \texttt{\textbackslash upgradetwo} & \upgradetwo \\
\end{tabular*}

\subsubsection{LHCb sub-detectors and sub-systems}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash velo} & \velo & \texttt{\textbackslash rich} & \rich & \texttt{\textbackslash richone} & \richone \\
\texttt{\textbackslash richtwo} & \richtwo & \texttt{\textbackslash ttracker} & \ttracker & \texttt{\textbackslash intr} & \intr \\
\texttt{\textbackslash st} & \st & \texttt{\textbackslash ot} & \ot & \texttt{\textbackslash herschel} & \herschel \\
\texttt{\textbackslash spd} & \spd & \texttt{\textbackslash presh} & \presh & \texttt{\textbackslash ecal} & \ecal \\
\texttt{\textbackslash hcal} & \hcal & \texttt{\textbackslash MagUp} & \MagUp & \texttt{\textbackslash MagDown} & \MagDown \\
\texttt{\textbackslash ode} & \ode & \texttt{\textbackslash daq} & \daq & \texttt{\textbackslash tfc} & \tfc \\
\texttt{\textbackslash ecs} & \ecs & \texttt{\textbackslash lone} & \lone & \texttt{\textbackslash hlt} & \hlt \\
\texttt{\textbackslash hltone} & \hltone & \texttt{\textbackslash hlttwo} & \hlttwo &  \\
\end{tabular*}

\subsection{Particles}
\subsubsection{Leptons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash electron} & \electron & \texttt{\textbackslash en} & \en & \texttt{\textbackslash ep} & \ep \\
\texttt{\textbackslash epm} & \epm & \texttt{\textbackslash emp} & \emp & \texttt{\textbackslash epem} & \epem \\
\texttt{\textbackslash muon} & \muon & \texttt{\textbackslash mup} & \mup & \texttt{\textbackslash mun} & \mun \\
\texttt{\textbackslash mupm} & \mupm & \texttt{\textbackslash mump} & \mump & \texttt{\textbackslash mumu} & \mumu \\
\texttt{\textbackslash tauon} & \tauon & \texttt{\textbackslash taup} & \taup & \texttt{\textbackslash taum} & \taum \\
\texttt{\textbackslash taupm} & \taupm & \texttt{\textbackslash taump} & \taump & \texttt{\textbackslash tautau} & \tautau \\
\texttt{\textbackslash lepton} & \lepton & \texttt{\textbackslash ellm} & \ellm & \texttt{\textbackslash ellp} & \ellp \\
\texttt{\textbackslash ellpm} & \ellpm & \texttt{\textbackslash ellmp} & \ellmp & \texttt{\textbackslash ellell} & \ellell \\
\texttt{\textbackslash neu} & \neu & \texttt{\textbackslash neub} & \neub & \texttt{\textbackslash neue} & \neue \\
\texttt{\textbackslash neueb} & \neueb & \texttt{\textbackslash neum} & \neum & \texttt{\textbackslash neumb} & \neumb \\
\texttt{\textbackslash neut} & \neut & \texttt{\textbackslash neutb} & \neutb & \texttt{\textbackslash neul} & \neul \\
\texttt{\textbackslash neulb} & \neulb &  \\
\end{tabular*}

\subsubsection{Gauge bosons and scalars}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash g} & \g & \texttt{\textbackslash H} & \H & \texttt{\textbackslash Hp} & \Hp \\
\texttt{\textbackslash Hm} & \Hm & \texttt{\textbackslash Hpm} & \Hpm & \texttt{\textbackslash W} & \W \\
\texttt{\textbackslash Wp} & \Wp & \texttt{\textbackslash Wm} & \Wm & \texttt{\textbackslash Wpm} & \Wpm \\
\texttt{\textbackslash Z} & \Z &  \\
\end{tabular*}

\subsubsection{Quarks}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash quark} & \quark & \texttt{\textbackslash quarkbar} & \quarkbar & \texttt{\textbackslash qqbar} & \qqbar \\
\texttt{\textbackslash uquark} & \uquark & \texttt{\textbackslash uquarkbar} & \uquarkbar & \texttt{\textbackslash uubar} & \uubar \\
\texttt{\textbackslash dquark} & \dquark & \texttt{\textbackslash dquarkbar} & \dquarkbar & \texttt{\textbackslash ddbar} & \ddbar \\
\texttt{\textbackslash squark} & \squark & \texttt{\textbackslash squarkbar} & \squarkbar & \texttt{\textbackslash ssbar} & \ssbar \\
\texttt{\textbackslash cquark} & \cquark & \texttt{\textbackslash cquarkbar} & \cquarkbar & \texttt{\textbackslash ccbar} & \ccbar \\
\texttt{\textbackslash bquark} & \bquark & \texttt{\textbackslash bquarkbar} & \bquarkbar & \texttt{\textbackslash bbbar} & \bbbar \\
\texttt{\textbackslash tquark} & \tquark & \texttt{\textbackslash tquarkbar} & \tquarkbar & \texttt{\textbackslash ttbar} & \ttbar \\
\end{tabular*}

\subsubsection{Light mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash hadron} & \hadron & \texttt{\textbackslash pion} & \pion & \texttt{\textbackslash piz} & \piz \\
\texttt{\textbackslash pip} & \pip & \texttt{\textbackslash pim} & \pim & \texttt{\textbackslash pipm} & \pipm \\
\texttt{\textbackslash pimp} & \pimp & \texttt{\textbackslash rhomeson} & \rhomeson & \texttt{\textbackslash rhoz} & \rhoz \\
\texttt{\textbackslash rhop} & \rhop & \texttt{\textbackslash rhom} & \rhom & \texttt{\textbackslash rhopm} & \rhopm \\
\texttt{\textbackslash rhomp} & \rhomp & \texttt{\textbackslash kaon} & \kaon & \texttt{\textbackslash Kbar} & \Kbar \\
\texttt{\textbackslash Kb} & \Kb & \texttt{\textbackslash KorKbar} & \KorKbar & \texttt{\textbackslash Kz} & \Kz \\
\texttt{\textbackslash Kzb} & \Kzb & \texttt{\textbackslash Kp} & \Kp & \texttt{\textbackslash Km} & \Km \\
\texttt{\textbackslash Kpm} & \Kpm & \texttt{\textbackslash Kmp} & \Kmp & \texttt{\textbackslash KS} & \KS \\
\texttt{\textbackslash Vzero} & \Vzero & \texttt{\textbackslash KL} & \KL & \texttt{\textbackslash Kstarz} & \Kstarz \\
\texttt{\textbackslash Kstarzb} & \Kstarzb & \texttt{\textbackslash Kstar} & \Kstar & \texttt{\textbackslash Kstarb} & \Kstarb \\
\texttt{\textbackslash Kstarp} & \Kstarp & \texttt{\textbackslash Kstarm} & \Kstarm & \texttt{\textbackslash Kstarpm} & \Kstarpm \\
\texttt{\textbackslash Kstarmp} & \Kstarmp & \texttt{\textbackslash KorKbarz} & \KorKbarz & \texttt{\textbackslash etaz} & \etaz \\
\texttt{\textbackslash etapr} & \etapr & \texttt{\textbackslash phiz} & \phiz & \texttt{\textbackslash omegaz} & \omegaz \\
\end{tabular*}

\subsubsection{Charmed mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Dbar} & \Dbar & \texttt{\textbackslash D} & \D & \texttt{\textbackslash Db} & \Db \\
\texttt{\textbackslash DorDbar} & \DorDbar & \texttt{\textbackslash Dz} & \Dz & \texttt{\textbackslash Dzb} & \Dzb \\
\texttt{\textbackslash Dp} & \Dp & \texttt{\textbackslash Dm} & \Dm & \texttt{\textbackslash Dpm} & \Dpm \\
\texttt{\textbackslash Dmp} & \Dmp & \texttt{\textbackslash DpDm} & \DpDm & \texttt{\textbackslash Dstar} & \Dstar \\
\texttt{\textbackslash Dstarb} & \Dstarb & \texttt{\textbackslash Dstarz} & \Dstarz & \texttt{\textbackslash Dstarzb} & \Dstarzb \\
\texttt{\textbackslash theDstarz} & \theDstarz & \texttt{\textbackslash theDstarzb} & \theDstarzb & \texttt{\textbackslash Dstarp} & \Dstarp \\
\texttt{\textbackslash Dstarm} & \Dstarm & \texttt{\textbackslash Dstarpm} & \Dstarpm & \texttt{\textbackslash Dstarmp} & \Dstarmp \\
\texttt{\textbackslash theDstarp} & \theDstarp & \texttt{\textbackslash theDstarm} & \theDstarm & \texttt{\textbackslash theDstarpm} & \theDstarpm \\
\texttt{\textbackslash theDstarmp} & \theDstarmp & \texttt{\textbackslash Ds} & \Ds & \texttt{\textbackslash Dsp} & \Dsp \\
\texttt{\textbackslash Dsm} & \Dsm & \texttt{\textbackslash Dspm} & \Dspm & \texttt{\textbackslash Dsmp} & \Dsmp \\
\texttt{\textbackslash Dss} & \Dss & \texttt{\textbackslash Dssp} & \Dssp & \texttt{\textbackslash Dssm} & \Dssm \\
\texttt{\textbackslash Dsspm} & \Dsspm & \texttt{\textbackslash Dssmp} & \Dssmp & \texttt{\textbackslash DporDsp} & \DporDsp \\
\texttt{\textbackslash DmorDsm} & \DmorDsm & \texttt{\textbackslash DpmorDspm} & \DpmorDspm &  \\
\end{tabular*}

\subsubsection{Beauty mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash B} & \B & \texttt{\textbackslash Bbar} & \Bbar & \texttt{\textbackslash Bb} & \Bb \\
\texttt{\textbackslash BorBbar} & \BorBbar & \texttt{\textbackslash Bz} & \Bz & \texttt{\textbackslash Bzb} & \Bzb \\
\texttt{\textbackslash Bd} & \Bd & \texttt{\textbackslash Bdb} & \Bdb & \texttt{\textbackslash BdorBdbar} & \BdorBdbar \\
\texttt{\textbackslash Bu} & \Bu & \texttt{\textbackslash Bub} & \Bub & \texttt{\textbackslash Bp} & \Bp \\
\texttt{\textbackslash Bm} & \Bm & \texttt{\textbackslash Bpm} & \Bpm & \texttt{\textbackslash Bmp} & \Bmp \\
\texttt{\textbackslash Bs} & \Bs & \texttt{\textbackslash Bsb} & \Bsb & \texttt{\textbackslash BsorBsbar} & \BsorBsbar \\
\texttt{\textbackslash Bc} & \Bc & \texttt{\textbackslash Bcp} & \Bcp & \texttt{\textbackslash Bcm} & \Bcm \\
\texttt{\textbackslash Bcpm} & \Bcpm & \texttt{\textbackslash Bds} & \Bds & \texttt{\textbackslash Bdsb} & \Bdsb \\
\texttt{\textbackslash BdorBs} & \BdorBs & \texttt{\textbackslash BdorBsbar} & \BdorBsbar &  \\
\end{tabular*}

\subsubsection{Onia}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash jpsi} & \jpsi & \texttt{\textbackslash psitwos} & \psitwos & \texttt{\textbackslash psiprpr} & \psiprpr \\
\texttt{\textbackslash etac} & \etac & \texttt{\textbackslash psires} & \psires & \texttt{\textbackslash chic} & \chic \\
\texttt{\textbackslash chiczero} & \chiczero & \texttt{\textbackslash chicone} & \chicone & \texttt{\textbackslash chictwo} & \chictwo \\
\texttt{\textbackslash chicJ} & \chicJ & \texttt{\textbackslash Upsilonres} & \Upsilonres & \texttt{\textbackslash OneS} & \OneS \\
\texttt{\textbackslash TwoS} & \TwoS & \texttt{\textbackslash ThreeS} & \ThreeS & \texttt{\textbackslash FourS} & \FourS \\
\texttt{\textbackslash FiveS} & \FiveS & \texttt{\textbackslash chib} & \chib & \texttt{\textbackslash chibzero} & \chibzero \\
\texttt{\textbackslash chibone} & \chibone & \texttt{\textbackslash chibtwo} & \chibtwo & \texttt{\textbackslash chibJ} & \chibJ \\
\texttt{\textbackslash theX} & \theX &  \\
\end{tabular*}

\subsubsection{Light Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash proton} & \proton & \texttt{\textbackslash antiproton} & \antiproton & \texttt{\textbackslash neutron} & \neutron \\
\texttt{\textbackslash antineutron} & \antineutron & \texttt{\textbackslash Deltares} & \Deltares & \texttt{\textbackslash Deltaresbar} & \Deltaresbar \\
\texttt{\textbackslash Lz} & \Lz & \texttt{\textbackslash Lbar} & \Lbar & \texttt{\textbackslash LorLbar} & \LorLbar \\
\texttt{\textbackslash Lambdares} & \Lambdares & \texttt{\textbackslash Lambdaresbar} & \Lambdaresbar & \texttt{\textbackslash Sigmares} & \Sigmares \\
\texttt{\textbackslash Sigmaz} & \Sigmaz & \texttt{\textbackslash Sigmap} & \Sigmap & \texttt{\textbackslash Sigmam} & \Sigmam \\
\texttt{\textbackslash Sigmaresbar} & \Sigmaresbar & \texttt{\textbackslash Sigmabarz} & \Sigmabarz & \texttt{\textbackslash Sigmabarp} & \Sigmabarp \\
\texttt{\textbackslash Sigmabarm} & \Sigmabarm & \texttt{\textbackslash Xires} & \Xires & \texttt{\textbackslash Xiz} & \Xiz \\
\texttt{\textbackslash Xim} & \Xim & \texttt{\textbackslash Xiresbar} & \Xiresbar & \texttt{\textbackslash Xibarz} & \Xibarz \\
\texttt{\textbackslash Xibarp} & \Xibarp & \texttt{\textbackslash Omegares} & \Omegares & \texttt{\textbackslash Omegaresbar} & \Omegaresbar \\
\texttt{\textbackslash Omegam} & \Omegam & \texttt{\textbackslash Omegabarp} & \Omegabarp &  \\
\end{tabular*}

\subsubsection{Charmed Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Lc} & \Lc & \texttt{\textbackslash Lcbar} & \Lcbar & \texttt{\textbackslash Sigmac} & \Sigmac \\
\texttt{\textbackslash Sigmacp} & \Sigmacp & \texttt{\textbackslash Sigmacz} & \Sigmacz & \texttt{\textbackslash Sigmacpp} & \Sigmacpp \\
\texttt{\textbackslash Sigmacbar} & \Sigmacbar & \texttt{\textbackslash Sigmacbarp} & \Sigmacbarp & \texttt{\textbackslash Sigmacbarz} & \Sigmacbarz \\
\texttt{\textbackslash Sigmacbarm} & \Sigmacbarm & \texttt{\textbackslash Xic} & \Xic & \texttt{\textbackslash Xicz} & \Xicz \\
\texttt{\textbackslash Xicp} & \Xicp & \texttt{\textbackslash Xicbar} & \Xicbar & \texttt{\textbackslash Xicbarz} & \Xicbarz \\
\texttt{\textbackslash Xicbarm} & \Xicbarm & \texttt{\textbackslash Omegac} & \Omegac & \texttt{\textbackslash Omegacbar} & \Omegacbar \\
\texttt{\textbackslash Xicc} & \Xicc & \texttt{\textbackslash Xiccbar} & \Xiccbar & \texttt{\textbackslash Xiccp} & \Xiccp \\
\texttt{\textbackslash Xiccpp} & \Xiccpp & \texttt{\textbackslash Xiccbarm} & \Xiccbarm & \texttt{\textbackslash Xiccbarmm} & \Xiccbarmm \\
\texttt{\textbackslash Omegacc} & \Omegacc & \texttt{\textbackslash Omegaccbar} & \Omegaccbar & \texttt{\textbackslash Omegaccc} & \Omegaccc \\
\texttt{\textbackslash Omegacccbar} & \Omegacccbar &  \\
\end{tabular*}

\subsubsection{Beauty Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Lb} & \Lb & \texttt{\textbackslash Lbbar} & \Lbbar & \texttt{\textbackslash Sigmab} & \Sigmab \\
\texttt{\textbackslash Sigmabp} & \Sigmabp & \texttt{\textbackslash Sigmabz} & \Sigmabz & \texttt{\textbackslash Sigmabm} & \Sigmabm \\
\texttt{\textbackslash Sigmabpm} & \Sigmabpm & \texttt{\textbackslash Sigmabbar} & \Sigmabbar & \texttt{\textbackslash Sigmabbarp} & \Sigmabbarp \\
\texttt{\textbackslash Sigmabbarz} & \Sigmabbarz & \texttt{\textbackslash Sigmabbarm} & \Sigmabbarm & \texttt{\textbackslash Sigmabbarpm} & \Sigmabbarpm \\
\texttt{\textbackslash Xib} & \Xib & \texttt{\textbackslash Xibz} & \Xibz & \texttt{\textbackslash Xibm} & \Xibm \\
\texttt{\textbackslash Xibbar} & \Xibbar & \texttt{\textbackslash Xibbarz} & \Xibbarz & \texttt{\textbackslash Xibbarp} & \Xibbarp \\
\texttt{\textbackslash Omegab} & \Omegab & \texttt{\textbackslash Omegabbar} & \Omegabbar &  \\
\end{tabular*}

\subsection{Physics symbols}
\subsubsection{Decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BF} & \BF & \texttt{\textbackslash BR} & \BR & \texttt{\textbackslash BRvis} & \BRvis \\
\texttt{\textbackslash ra} & \ra & \texttt{\textbackslash to} & \to &  \\
\end{tabular*}

\subsubsection{Lifetimes}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tauBs} & \tauBs & \texttt{\textbackslash tauBd} & \tauBd & \texttt{\textbackslash tauBz} & \tauBz \\
\texttt{\textbackslash tauBu} & \tauBu & \texttt{\textbackslash tauDp} & \tauDp & \texttt{\textbackslash tauDz} & \tauDz \\
\texttt{\textbackslash tauL} & \tauL & \texttt{\textbackslash tauH} & \tauH &  \\
\end{tabular*}

\subsubsection{Masses}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash mBd} & \mBd & \texttt{\textbackslash mBp} & \mBp & \texttt{\textbackslash mBs} & \mBs \\
\texttt{\textbackslash mBc} & \mBc & \texttt{\textbackslash mLb} & \mLb &  \\
\end{tabular*}

\subsubsection{EW theory, groups}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash grpsuthree} & \grpsuthree & \texttt{\textbackslash grpsutw} & \grpsutw & \texttt{\textbackslash grpuone} & \grpuone \\
\texttt{\textbackslash ssqtw} & \ssqtw & \texttt{\textbackslash csqtw} & \csqtw & \texttt{\textbackslash stw} & \stw \\
\texttt{\textbackslash ctw} & \ctw & \texttt{\textbackslash ssqtwef} & \ssqtwef & \texttt{\textbackslash csqtwef} & \csqtwef \\
\texttt{\textbackslash stwef} & \stwef & \texttt{\textbackslash ctwef} & \ctwef & \texttt{\textbackslash gv} & \gv \\
\texttt{\textbackslash ga} & \ga & \texttt{\textbackslash order} & \order & \texttt{\textbackslash ordalph} & \ordalph \\
\texttt{\textbackslash ordalsq} & \ordalsq & \texttt{\textbackslash ordalcb} & \ordalcb &  \\
\end{tabular*}

\subsubsection{QCD parameters}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash as} & \as & \texttt{\textbackslash MSb} & \MSb & \texttt{\textbackslash lqcd} & \lqcd \\
\texttt{\textbackslash qsq} & \qsq &  \\
\end{tabular*}

\subsubsection{CKM, \boldmath \CP violation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eps} & \eps & \texttt{\textbackslash epsK} & \epsK & \texttt{\textbackslash epsB} & \epsB \\
\texttt{\textbackslash epsp} & \epsp & \texttt{\textbackslash CP} & \CP & \texttt{\textbackslash CPT} & \CPT \\
\texttt{\textbackslash T} & \T & \texttt{\textbackslash rhobar} & \rhobar & \texttt{\textbackslash etabar} & \etabar \\
\texttt{\textbackslash Vud} & \Vud & \texttt{\textbackslash Vcd} & \Vcd & \texttt{\textbackslash Vtd} & \Vtd \\
\texttt{\textbackslash Vus} & \Vus & \texttt{\textbackslash Vcs} & \Vcs & \texttt{\textbackslash Vts} & \Vts \\
\texttt{\textbackslash Vub} & \Vub & \texttt{\textbackslash Vcb} & \Vcb & \texttt{\textbackslash Vtb} & \Vtb \\
\texttt{\textbackslash Vuds} & \Vuds & \texttt{\textbackslash Vcds} & \Vcds & \texttt{\textbackslash Vtds} & \Vtds \\
\texttt{\textbackslash Vuss} & \Vuss & \texttt{\textbackslash Vcss} & \Vcss & \texttt{\textbackslash Vtss} & \Vtss \\
\texttt{\textbackslash Vubs} & \Vubs & \texttt{\textbackslash Vcbs} & \Vcbs & \texttt{\textbackslash Vtbs} & \Vtbs \\
\end{tabular*}

\subsubsection{Oscillations}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dm} & \dm & \texttt{\textbackslash dms} & \dms & \texttt{\textbackslash dmd} & \dmd \\
\texttt{\textbackslash DG} & \DG & \texttt{\textbackslash DGs} & \DGs & \texttt{\textbackslash DGd} & \DGd \\
\texttt{\textbackslash Gs} & \Gs & \texttt{\textbackslash Gd} & \Gd & \texttt{\textbackslash MBq} & \MBq \\
\texttt{\textbackslash DGq} & \DGq & \texttt{\textbackslash Gq} & \Gq & \texttt{\textbackslash dmq} & \dmq \\
\texttt{\textbackslash GL} & \GL & \texttt{\textbackslash GH} & \GH & \texttt{\textbackslash DGsGs} & \DGsGs \\
\texttt{\textbackslash Delm} & \Delm & \texttt{\textbackslash ACP} & \ACP & \texttt{\textbackslash Adir} & \Adir \\
\texttt{\textbackslash Amix} & \Amix & \texttt{\textbackslash ADelta} & \ADelta & \texttt{\textbackslash phid} & \phid \\
\texttt{\textbackslash sinphid} & \sinphid & \texttt{\textbackslash phis} & \phis & \texttt{\textbackslash betas} & \betas \\
\texttt{\textbackslash sbetas} & \sbetas & \texttt{\textbackslash stbetas} & \stbetas & \texttt{\textbackslash stphis} & \stphis \\
\texttt{\textbackslash sinphis} & \sinphis &  \\
\end{tabular*}

\subsubsection{Tagging}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash edet} & \edet & \texttt{\textbackslash erec} & \erec & \texttt{\textbackslash esel} & \esel \\
\texttt{\textbackslash etrg} & \etrg & \texttt{\textbackslash etot} & \etot & \texttt{\textbackslash mistag} & \mistag \\
\texttt{\textbackslash wcomb} & \wcomb & \texttt{\textbackslash etag} & \etag & \texttt{\textbackslash etagcomb} & \etagcomb \\
\texttt{\textbackslash effeff} & \effeff & \texttt{\textbackslash effeffcomb} & \effeffcomb & \texttt{\textbackslash efftag} & \efftag \\
\texttt{\textbackslash effD} & \effD & \texttt{\textbackslash etagprompt} & \etagprompt & \texttt{\textbackslash etagLL} & \etagLL \\
\end{tabular*}

\subsubsection{Key decay channels}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdToKstmm} & \BdToKstmm & \texttt{\textbackslash BdbToKstmm} & \BdbToKstmm & \texttt{\textbackslash BsToJPsiPhi} & \BsToJPsiPhi \\
\texttt{\textbackslash BdToJPsiKst} & \BdToJPsiKst & \texttt{\textbackslash BdbToJPsiKst} & \BdbToJPsiKst & \texttt{\textbackslash BsPhiGam} & \BsPhiGam \\
\texttt{\textbackslash BdKstGam} & \BdKstGam & \texttt{\textbackslash BTohh} & \BTohh & \texttt{\textbackslash BdTopipi} & \BdTopipi \\
\texttt{\textbackslash BdToKpi} & \BdToKpi & \texttt{\textbackslash BsToKK} & \BsToKK & \texttt{\textbackslash BsTopiK} & \BsTopiK \\
\texttt{\textbackslash Cpipi} & \Cpipi & \texttt{\textbackslash Spipi} & \Spipi & \texttt{\textbackslash CKK} & \CKK \\
\texttt{\textbackslash SKK} & \SKK & \texttt{\textbackslash ADGKK} & \ADGKK &  \\
\end{tabular*}

\subsubsection{Rare decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdKstee} & \BdKstee & \texttt{\textbackslash BdbKstee} & \BdbKstee & \texttt{\textbackslash bsll} & \bsll \\
\texttt{\textbackslash AFB} & \AFB & \texttt{\textbackslash FL} & \FL & \texttt{\textbackslash AT\#1 \textbackslash AT2} & \AT2 \\
\texttt{\textbackslash btosgam} & \btosgam & \texttt{\textbackslash btodgam} & \btodgam & \texttt{\textbackslash Bsmm} & \Bsmm \\
\texttt{\textbackslash Bdmm} & \Bdmm & \texttt{\textbackslash Bsee} & \Bsee & \texttt{\textbackslash Bdee} & \Bdee \\
\texttt{\textbackslash ctl} & \ctl & \texttt{\textbackslash ctk} & \ctk &  \\
\end{tabular*}

\subsubsection{Wilson coefficients and operators}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash C\#1 \textbackslash C9} & \C9 & \texttt{\textbackslash Cp\#1 \textbackslash Cp7} & \Cp7 & \texttt{\textbackslash Ceff\#1 \textbackslash Ceff9  } & \Ceff9   \\
\texttt{\textbackslash Cpeff\#1 \textbackslash Cpeff7} & \Cpeff7 & \texttt{\textbackslash Ope\#1 \textbackslash Ope2} & \Ope2 & \texttt{\textbackslash Opep\#1 \textbackslash Opep7} & \Opep7 \\
\end{tabular*}

\subsubsection{Charm}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash xprime} & \xprime & \texttt{\textbackslash yprime} & \yprime & \texttt{\textbackslash ycp} & \ycp \\
\texttt{\textbackslash agamma} & \agamma & \texttt{\textbackslash dkpicf} & \dkpicf &  \\
\end{tabular*}

\subsubsection{QM}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bra[1] \textbackslash bra\{a\}} & \bra{a} & \texttt{\textbackslash ket[1] \textbackslash ket\{b\}} & \ket{b} & \texttt{\textbackslash braket[2] \textbackslash braket\{a\}\{b\}} & \braket{a}{b} \\
\end{tabular*}

\subsubsection{Units (these macros add a small space in front)}
\subsubsection{Energy and momentum }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tev} & \tev & \texttt{\textbackslash gev} & \gev & \texttt{\textbackslash mev} & \mev \\
\texttt{\textbackslash kev} & \kev & \texttt{\textbackslash ev} & \ev & \texttt{\textbackslash gevgev} & \gevgev \\
\texttt{\textbackslash mevc} & \mevc & \texttt{\textbackslash gevc} & \gevc & \texttt{\textbackslash mevcc} & \mevcc \\
\texttt{\textbackslash gevcc} & \gevcc & \texttt{\textbackslash gevgevcc} & \gevgevcc & \texttt{\textbackslash gevgevcccc} & \gevgevcccc \\
\end{tabular*}

\subsubsection{Distance and area (these macros add a small space)}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash km} & \km & \texttt{\textbackslash m} & \m & \texttt{\textbackslash ma} & \ma \\
\texttt{\textbackslash cm} & \cm & \texttt{\textbackslash cma} & \cma & \texttt{\textbackslash mm} & \mm \\
\texttt{\textbackslash mma} & \mma & \texttt{\textbackslash mum} & \mum & \texttt{\textbackslash muma} & \muma \\
\texttt{\textbackslash nm} & \nm & \texttt{\textbackslash fm} & \fm & \texttt{\textbackslash barn} & \barn \\
\texttt{\textbackslash mbarn} & \mbarn & \texttt{\textbackslash mub} & \mub & \texttt{\textbackslash nb} & \nb \\
\texttt{\textbackslash invnb} & \invnb & \texttt{\textbackslash pb} & \pb & \texttt{\textbackslash invpb} & \invpb \\
\texttt{\textbackslash fb} & \fb & \texttt{\textbackslash invfb} & \invfb & \texttt{\textbackslash ab} & \ab \\
\texttt{\textbackslash invab} & \invab &  \\
\end{tabular*}

\subsubsection{Time }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sec} & \sec & \texttt{\textbackslash ms} & \ms & \texttt{\textbackslash mus} & \mus \\
\texttt{\textbackslash ns} & \ns & \texttt{\textbackslash ps} & \ps & \texttt{\textbackslash fs} & \fs \\
\texttt{\textbackslash mhz} & \mhz & \texttt{\textbackslash khz} & \khz & \texttt{\textbackslash hz} & \hz \\
\texttt{\textbackslash invps} & \invps & \texttt{\textbackslash invns} & \invns & \texttt{\textbackslash yr} & \yr \\
\texttt{\textbackslash hr} & \hr &  \\
\end{tabular*}

\subsubsection{Temperature}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degc} & \degc & \texttt{\textbackslash degk} & \degk &  \\
\end{tabular*}

\subsubsection{Material lengths, radiation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Xrad} & \Xrad & \texttt{\textbackslash NIL} & \NIL & \texttt{\textbackslash mip} & \mip \\
\texttt{\textbackslash neutroneq} & \neutroneq & \texttt{\textbackslash neqcmcm} & \neqcmcm & \texttt{\textbackslash kRad} & \kRad \\
\texttt{\textbackslash MRad} & \MRad & \texttt{\textbackslash ci} & \ci & \texttt{\textbackslash mci} & \mci \\
\end{tabular*}

\subsubsection{Uncertainties}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sx} & \sx & \texttt{\textbackslash sy} & \sy & \texttt{\textbackslash sz} & \sz \\
\texttt{\textbackslash stat} & \stat & \texttt{\textbackslash syst} & \syst & \texttt{\textbackslash lumi} & \lumi \\
\end{tabular*}

\subsubsection{Maths}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash order} & \order & \texttt{\textbackslash chisq} & \chisq & \texttt{\textbackslash chisqndf} & \chisqndf \\
\texttt{\textbackslash chisqip} & \chisqip & \texttt{\textbackslash chisqfd} & \chisqfd & \texttt{\textbackslash chisqvs} & \chisqvs \\
\texttt{\textbackslash chisqvtx} & \chisqvtx & \texttt{\textbackslash chisqvtxndf} & \chisqvtxndf & \texttt{\textbackslash deriv} & \deriv \\
\texttt{\textbackslash gsim} & \gsim & \texttt{\textbackslash lsim} & \lsim & \texttt{\textbackslash mean[1] \textbackslash mean\{x\}} & \mean{x} \\
\texttt{\textbackslash abs[1] \textbackslash abs\{x\}} & \abs{x} & \texttt{\textbackslash Real} & \Real & \texttt{\textbackslash Imag} & \Imag \\
\texttt{\textbackslash PDF} & \PDF & \texttt{\textbackslash sPlot} & \sPlot & \texttt{\textbackslash sFit} & \sFit \\
\end{tabular*}

\subsection{Kinematics}
\subsubsection{Energy, Momenta}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Ebeam} & \Ebeam & \texttt{\textbackslash sqs} & \sqs & \texttt{\textbackslash sqsnn} & \sqsnn \\
\texttt{\textbackslash pt} & \pt & \texttt{\textbackslash ptsq} & \ptsq & \texttt{\textbackslash ptot} & \ptot \\
\texttt{\textbackslash et} & \et & \texttt{\textbackslash mt} & \mt & \texttt{\textbackslash dpp} & \dpp \\
\texttt{\textbackslash msq} & \msq & \texttt{\textbackslash dedx} & \dedx &  \\
\end{tabular*}

\subsubsection{PID}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dllkpi} & \dllkpi & \texttt{\textbackslash dllppi} & \dllppi & \texttt{\textbackslash dllepi} & \dllepi \\
\texttt{\textbackslash dllmupi} & \dllmupi &  \\
\end{tabular*}

\subsubsection{Geometry}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degrees} & \degrees & \texttt{\textbackslash murad} & \murad & \texttt{\textbackslash mrad} & \mrad \\
\texttt{\textbackslash rad} & \rad &  \\
\end{tabular*}

\subsubsection{Accelerator}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash betastar} & \betastar & \texttt{\textbackslash lum} & \lum & \texttt{\textbackslash intlum[1] \textbackslash intlum\{2 \,\invfb\}} & \intlum{2 \,\invfb} \\
\end{tabular*}

\subsection{Software}
\subsubsection{Programs}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bcvegpy} & \bcvegpy & \texttt{\textbackslash boole} & \boole & \texttt{\textbackslash brunel} & \brunel \\
\texttt{\textbackslash davinci} & \davinci & \texttt{\textbackslash dirac} & \dirac & \texttt{\textbackslash evtgen} & \evtgen \\
\texttt{\textbackslash fewz} & \fewz & \texttt{\textbackslash fluka} & \fluka & \texttt{\textbackslash ganga} & \ganga \\
\texttt{\textbackslash gaudi} & \gaudi & \texttt{\textbackslash gauss} & \gauss & \texttt{\textbackslash geant} & \geant \\
\texttt{\textbackslash lamarr} & \lamarr & \texttt{\textbackslash hepmc} & \hepmc & \texttt{\textbackslash herwig} & \herwig \\
\texttt{\textbackslash moore} & \moore & \texttt{\textbackslash neurobayes} & \neurobayes & \texttt{\textbackslash photos} & \photos \\
\texttt{\textbackslash powheg} & \powheg & \texttt{\textbackslash pythia} & \pythia & \texttt{\textbackslash resbos} & \resbos \\
\texttt{\textbackslash roofit} & \roofit & \texttt{\textbackslash root} & \root & \texttt{\textbackslash spice} & \spice \\
\texttt{\textbackslash tensorflow} & \tensorflow & \texttt{\textbackslash urania} & \urania &  \\
\end{tabular*}

\subsubsection{Languages}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cpp} & \cpp & \texttt{\textbackslash ruby} & \ruby & \texttt{\textbackslash fortran} & \fortran \\
\texttt{\textbackslash svn} & \svn & \texttt{\textbackslash git} & \git & \texttt{\textbackslash latex} & \latex \\
\end{tabular*}

\subsubsection{Data processing}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash kbit} & \kbit & \texttt{\textbackslash kbps} & \kbps & \texttt{\textbackslash kbytes} & \kbytes \\
\texttt{\textbackslash kbyps} & \kbyps & \texttt{\textbackslash mbit} & \mbit & \texttt{\textbackslash mbps} & \mbps \\
\texttt{\textbackslash mbytes} & \mbytes & \texttt{\textbackslash mbyps} & \mbyps & \texttt{\textbackslash gbit} & \gbit \\
\texttt{\textbackslash gbps} & \gbps & \texttt{\textbackslash gbytes} & \gbytes & \texttt{\textbackslash gbyps} & \gbyps \\
\texttt{\textbackslash tbit} & \tbit & \texttt{\textbackslash tbps} & \tbps & \texttt{\textbackslash tbytes} & \tbytes \\
\texttt{\textbackslash tbyps} & \tbyps & \texttt{\textbackslash dst} & \dst &  \\
\end{tabular*}

\subsection{Detector related}
\subsubsection{Detector technologies}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash nonn} & \nonn & \texttt{\textbackslash ponn} & \ponn & \texttt{\textbackslash nonp} & \nonp \\
\texttt{\textbackslash cvd} & \cvd & \texttt{\textbackslash mwpc} & \mwpc & \texttt{\textbackslash gem} & \gem \\
\end{tabular*}

\subsubsection{Detector components, electronics}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tell1} & \tell1 & \texttt{\textbackslash ukl1} & \ukl1 & \texttt{\textbackslash beetle} & \beetle \\
\texttt{\textbackslash otis} & \otis & \texttt{\textbackslash croc} & \croc & \texttt{\textbackslash carioca} & \carioca \\
\texttt{\textbackslash dialog} & \dialog & \texttt{\textbackslash sync} & \sync & \texttt{\textbackslash cardiac} & \cardiac \\
\texttt{\textbackslash gol} & \gol & \texttt{\textbackslash vcsel} & \vcsel & \texttt{\textbackslash ttc} & \ttc \\
\texttt{\textbackslash ttcrx} & \ttcrx & \texttt{\textbackslash hpd} & \hpd & \texttt{\textbackslash pmt} & \pmt \\
\texttt{\textbackslash specs} & \specs & \texttt{\textbackslash elmb} & \elmb & \texttt{\textbackslash fpga} & \fpga \\
\texttt{\textbackslash plc} & \plc & \texttt{\textbackslash rasnik} & \rasnik & \texttt{\textbackslash elmb} & \elmb \\
\texttt{\textbackslash can} & \can & \texttt{\textbackslash lvds} & \lvds & \texttt{\textbackslash ntc} & \ntc \\
\texttt{\textbackslash adc} & \adc & \texttt{\textbackslash led} & \led & \texttt{\textbackslash ccd} & \ccd \\
\texttt{\textbackslash hv} & \hv & \texttt{\textbackslash lv} & \lv & \texttt{\textbackslash pvss} & \pvss \\
\texttt{\textbackslash cmos} & \cmos & \texttt{\textbackslash fifo} & \fifo & \texttt{\textbackslash ccpc} & \ccpc \\
\end{tabular*}

\subsubsection{Chemical symbols}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cfourften} & \cfourften & \texttt{\textbackslash cffour} & \cffour & \texttt{\textbackslash cotwo} & \cotwo \\
\texttt{\textbackslash csixffouteen} & \csixffouteen & \texttt{\textbackslash mgftwo} & \mgftwo & \texttt{\textbackslash siotwo} & \siotwo \\
\end{tabular*}

\subsubsection{Special Text }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eg} & \eg & \texttt{\textbackslash ie} & \ie & \texttt{\textbackslash etal} & \etal \\
\texttt{\textbackslash etc} & \etc & \texttt{\textbackslash cf} & \cf & \texttt{\textbackslash ffp} & \ffp \\
\texttt{\textbackslash vs} & \vs &  \\
\end{tabular*}

\subsubsection{Helpful to align numbers in tables}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash phz} & \phz &  \\
\end{tabular*}



==> lhcb_text/preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
% !!!!!!!!!!!!!!!!!!! DO NOT EDIT THIS FILE !!!!!!!!!!!!!!!!!!!!!!!! %
%                                                                    %
% THE EB MAY OVERWRITE IT TO REFLECT LATEST CHANGES IN THE TEMPLATE  %
%                                                                    %
% You may define your own macros and packages in main.tex or add     %
% additional local files                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THis file contains all the default packages and modifications for
% LHCb formatting

%% %%%%%%%%%%%%%%%%%%
%%  Page formatting
%% %%%%%%%%%%%%%%%%%%
%%\usepackage[margin=1in]{geometry}
\usepackage[top=1in, bottom=1.25in, left=1in, right=1in]{geometry}

% fallback for manual settings... uncomment if the geometry package is not available
%
%\voffset=-11mm
%\textheight=220mm
%\textwidth=160mm
%\oddsidemargin=0mm
%\evensidemargin=0mm

\columnsep=5mm
\addtolength{\belowcaptionskip}{0.5em}

\renewcommand{\textfraction}{0.01}
\renewcommand{\floatpagefraction}{0.8} % changed from 0.99
\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.9}

% Allow the page size to vary a bit ...
\raggedbottom
% To avoid Latex to be too fussy with line breaking ...
\sloppy

%% %%%%%%%%%%%%%%%%%%%%%%%
%% Packages to be used
%% %%%%%%%%%%%%%%%%%%%%%%% 
\usepackage{microtype}
\usepackage{lineno}  % for line numbering during review
\usepackage{xspace} % To avoid problems with missing or double spaces after
                    % predefined symbold
\usepackage{caption} %these three command get the figure and table captions automatically small
\renewcommand{\captionfont}{\small}
\renewcommand{\captionlabelfont}{\small}

%% Graphics
\usepackage{graphicx}  % to include figures (can also use other packages)
\usepackage{color}
\usepackage{colortbl}
\graphicspath{{./figs/}} % Make Latex search fig subdir for figures
% \DeclareGraphicsExtensions{.pdf,.PDF,.png,.PNG}   % not needed

%% Math
\usepackage{amsmath} % Adds a large collection of math symbols
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{upgreek} % Adds in support for greek letters in roman typeset

%% fix to allow peaceful coexistence of line numbering and
%% mathematical objects
%% http://www.latex-community.org/forum/viewtopic.php?f=5&t=163
%%
\newcommand*\patchAmsMathEnvironmentForLineno[1]{%
\expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
\expandafter\let\csname oldend#1\expandafter\endcsname\csname
end#1\endcsname
 \renewenvironment{#1}%
   {\linenomath\csname old#1\endcsname}%
   {\csname oldend#1\endcsname\endlinenomath}%
}
\newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
  \patchAmsMathEnvironmentForLineno{#1}%
  \patchAmsMathEnvironmentForLineno{#1*}%
}
\AtBeginDocument{%
\patchBothAmsMathEnvironmentsForLineno{equation}%
\patchBothAmsMathEnvironmentsForLineno{align}%
\patchBothAmsMathEnvironmentsForLineno{flalign}%
\patchBothAmsMathEnvironmentsForLineno{alignat}%
\patchBothAmsMathEnvironmentsForLineno{gather}%
\patchBothAmsMathEnvironmentsForLineno{multline}%
\patchBothAmsMathEnvironmentsForLineno{eqnarray}%
}

% Get hyperlinks to captions and in references.
% These do not work with revtex. Use "hypertext" as class option instead.

\iffalse
\usepackage[pdftex,
            pdfauthor={\paperauthors},
            pdftitle={\paperasciititle},
            pdfkeywords={\paperkeywords},
            pdfcopyright={Copyright (C) \papercopyright},
            pdflicenseurl={\paperlicenceurl}]{hyperref}
% if you have a mysterious compilation error at this line, check there are only ascii characters in \paperasciititle (main.tex)
\fi
% overleaf comments
\usepackage[colorinlistoftodos,textsize=scriptsize]{todonotes}

% get footnotes below floats
\usepackage[bottom,flushmargin,hang,multiple]{footmisc}

%\usepackage[all]{hypcap} % Internal hyperlinks to floats.

\input{lhcb_text/lhcb-symbols-def} % Add in the predefined LHCb symbols

\iffalse
% substitute the boxes in the links by coloured text: (the boxes often overlap with the text inside)
\hypersetup{
  colorlinks   = true, %Colours links instead of ugly boxes
  urlcolor     = blue, %Colour for external hyperlinks
  linkcolor    = blue, %Colour of internal links
  citecolor    = red   %Colour of citations
}

\fi
\ifEnableSectionTOCLinks
    \usepackage[explicit]{titlesec} % to change headings
    
    % renew \contentsline for toc to include hypertarget
    \let\oldcontentsline\contentsline
    \renewcommand\contentsline[4]{\hypertarget{toc#4}{}\oldcontentsline{#1}{#2}{#3}{#4}}

    % renew \section to link to the toc
    \titleformat{\section}{\normalfont\Large\bf}{\hyperlink{tocsection.\thesection}{{\thesection} \parbox[t]{\dimexpr\textwidth-1pc}{#1}}}{1pc}{}

    % renew \subsection to link to the toc
    \titleformat{\subsection}{\normalfont\bf}{\hyperlink{tocsubsection.\thesubsection}{{\thesubsection} \parbox[t]{\dimexpr\textwidth-1pc}{#1}}}{1pc}{}

    %% Add 'Contents' title in TOC
    \titleformat{name=\section,numberless}[display]{}{}{0pt}{\normalfont\Huge\bfseries #1}
\fi

\usepackage{hyperref}    % Hyperlinks in references
\usepackage[all]{hypcap} % Internal hyperlinks to floats.
% Make this the last packages you include before the \begin{document}
\usepackage{cite} % Allows for ranges in citations
\usepackage{mciteplus}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
% !!!!!!!!!!!!!!!!!!! DO NOT EDIT THIS FILE !!!!!!!!!!!!!!!!!!!!!!!! %
%                                                                    %
% THE EB MAY OVERWRITE IT TO REFLECT LATEST CHANGES IN THE TEMPLATE  %
%                                                                    %
% You may define your own macros and packages in main.tex or add     %
% additional local files                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> mainbbl.tex <==
\ifx\mcitethebibliography\mciteundefinedmacro
\PackageError{LHCb.bst}{mciteplus.sty has not been loaded}
{This bibstyle requires the use of the mciteplus package.}\fi
\providecommand{\href}[2]{#2}
\begin{mcitethebibliography}{10}
\mciteSetBstSublistMode{n}
\mciteSetBstMaxWidthForm{subitem}{\alph{mcitesubitemcount})}
\mciteSetBstSublistLabelBeginEnd{\mcitemaxwidthsubitemform\space}
{\relax}{\relax}

\bibitem{PDG2024}
Particle Data Group, S.~Navas {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{\href{http://pdg.lbl.gov/}{Review of particle physics}}}, }{}\href{https://doi.org/10.1103/PhysRevD.110.030001}{Phys.\ Rev.\  \textbf{D110} (2024) 030001}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Kagan:2011pnt}
A.~L. Kagan, J.~F. Kamenik, G.~Perez, and S.~Stone, \ifthenelse{\boolean{articletitles}}{\emph{{Probing new top physics at the LHCb experiment}}, }{}\href{https://doi.org/10.1103/PhysRevLett.107.082003}{Phys.\ Rev.\ Lett.\  \textbf{107} (2011) 082003}, \href{http://arxiv.org/abs/1103.3747}{{\normalfont\ttfamily arXiv:1103.3747}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Gauld:2013aja}
R.~Gauld, \ifthenelse{\boolean{articletitles}}{\emph{{Feasibility of top quark measurements at LHCb and constraints on the large-$x$ gluon PDF}}, }{}\href{https://doi.org/10.1007/JHEP02(2014)126}{JHEP \textbf{02} (2014) 126}, \href{http://arxiv.org/abs/1311.1810}{{\normalfont\ttfamily arXiv:1311.1810}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Gauld:2014pxa}
R.~Gauld, \ifthenelse{\boolean{articletitles}}{\emph{{Leptonic top quark asymmetry predictions at LHCb}}, }{}\href{https://doi.org/10.1103/PhysRevD.91.054029}{Phys.\ Rev.\  \textbf{D91} (2015) 054029}, \href{http://arxiv.org/abs/1409.8631}{{\normalfont\ttfamily arXiv:1409.8631}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ttbar}
J.~M. Campbell, R.~K. Ellis, P.~Nason, and E.~Re, \ifthenelse{\boolean{articletitles}}{\emph{{Top-Pair Production and Decay at NLO Matched with Parton Showers}}, }{}\href{https://doi.org/10.1007/JHEP04(2015)114}{JHEP \textbf{04} (2015) 114}, \href{http://arxiv.org/abs/1412.1828}{{\normalfont\ttfamily arXiv:1412.1828}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ST_sch}
S.~Alioli, P.~Nason, C.~Oleari, and E.~Re, \ifthenelse{\boolean{articletitles}}{\emph{{NLO single-top production matched with shower in POWHEG: s- and t-channel contributions}}, }{}\href{https://doi.org/10.1088/1126-6708/2009/09/111}{JHEP \textbf{09} (2009) 111}, \href{http://arxiv.org/abs/0907.4076}{{\normalfont\ttfamily arXiv:0907.4076}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Wt}
E.~Re, \ifthenelse{\boolean{articletitles}}{\emph{{Single-top Wt-channel production matched with parton showers using the POWHEG method}}, }{}\href{https://doi.org/10.1140/epjc/s10052-011-1547-z}{Eur.\ Phys.\ J.\  \textbf{C71} (2011) 1547}, \href{http://arxiv.org/abs/1009.2450}{{\normalfont\ttfamily arXiv:1009.2450}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{gluonpdf}
M.~Czakon, M.~L. Mangano, A.~Mitov, and J.~Rojo, \ifthenelse{\boolean{articletitles}}{\emph{{Constraints on the gluon PDF from top quark pair production at hadron colliders}}, }{}\href{https://doi.org/10.1007/JHEP07(2013)167}{JHEP \textbf{07} (2013) 167}, \href{http://arxiv.org/abs/1303.7215}{{\normalfont\ttfamily arXiv:1303.7215}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Alekhin:2024bhs}
S.~Alekhin, M.~V. Garzelli, S.-O. Moch, and O.~Zenaiev, \ifthenelse{\boolean{articletitles}}{\emph{{NNLO PDFs driven by top-quark data}}, }{}\href{https://doi.org/10.1140/epjc/s10052-025-13832-8}{Eur.\ Phys.\ J.\  \textbf{C85} (2025) 162}, \href{http://arxiv.org/abs/2407.00545}{{\normalfont\ttfamily arXiv:2407.00545}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ablat:2023tiy}
A.~Ablat {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Exploring the impact of high-precision top-quark pair production data on the structure of the proton at the LHC}}, }{}\href{https://doi.org/10.1103/PhysRevD.109.054027}{Phys.\ Rev.\  \textbf{D109} (2024) 054027}, \href{http://arxiv.org/abs/2307.11153}{{\normalfont\ttfamily arXiv:2307.11153}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Bernreuther:2012sx}
W.~Bernreuther and Z.-G. Si, \ifthenelse{\boolean{articletitles}}{\emph{{Top quark and leptonic charge asymmetries for the Tevatron and LHC}}, }{}\href{https://doi.org/10.1103/PhysRevD.86.034026}{Phys.\ Rev.\  \textbf{D86} (2012) 034026}, \href{http://arxiv.org/abs/1205.6580}{{\normalfont\ttfamily arXiv:1205.6580}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CMS:2012hcu}
CMS collaboration, S.~Chatrchyan {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the $t\bar{t}$ production cross section in $pp$ collisions at $\sqrt{s}=7$ TeV with lepton + jets final states}}, }{}\href{https://doi.org/10.1016/j.physletb.2013.02.021}{Phys.\ Lett.\  \textbf{B720} (2013) 83}, \href{http://arxiv.org/abs/1212.6682}{{\normalfont\ttfamily arXiv:1212.6682}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CMS:2012xhh}
CMS collaboration, S.~Chatrchyan {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the single-top-quark $t$-channel cross section in $pp$ collisions at $\sqrt{s}=7$ TeV}}, }{}\href{https://doi.org/10.1007/JHEP12(2012)035}{JHEP \textbf{12} (2012) 035}, \href{http://arxiv.org/abs/1209.4533}{{\normalfont\ttfamily arXiv:1209.4533}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CMS:2013yjt}
CMS collaboration, S.~Chatrchyan {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the $t\bar{t}$ production cross section in the all-jet final state in pp collisions at $\sqrt{s}$ = 7 TeV}}, }{}\href{https://doi.org/10.1007/JHEP05(2013)065}{JHEP \textbf{05} (2013) 065}, \href{http://arxiv.org/abs/1302.0508}{{\normalfont\ttfamily arXiv:1302.0508}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ATLAS:2014sxe}
ATLAS collaboration, G.~Aad {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Comprehensive measurements of $t$-channel single top-quark production cross sections at $\sqrt{s} = 7$ TeV with the ATLAS detector}}, }{}\href{https://doi.org/10.1103/PhysRevD.90.112006}{Phys.\ Rev.\  \textbf{D90} (2014) 112006}, \href{http://arxiv.org/abs/1406.7844}{{\normalfont\ttfamily arXiv:1406.7844}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CMS:2014mgj}
CMS collaboration, V.~Khachatryan {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the t-channel single-top-quark production cross section and of the $\mid V_{tb} \mid$ CKM matrix element in pp collisions at $\sqrt{s}$= 8 TeV}}, }{}\href{https://doi.org/10.1007/JHEP06(2014)090}{JHEP \textbf{06} (2014) 090}, \href{http://arxiv.org/abs/1403.7366}{{\normalfont\ttfamily arXiv:1403.7366}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ATLAS:2014nxi}
ATLAS collaboration, G.~Aad {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the $t\bar{t}$ production cross-section using $e\mu $ events with b-tagged jets in pp collisions at $\sqrt{s}$ = 7 and 8 $\,\mathrm{TeV}$ with the ATLAS detector}}, }{}\href{https://doi.org/10.1140/epjc/s10052-016-4501-2}{Eur.\ Phys.\ J.\  \textbf{C74} (2014) 3109}, Addendum \href{https://doi.org/10.1140/epjc/s10052-016-4501-2}{ibid.\   \textbf{76} (2016) 642}, \href{http://arxiv.org/abs/1406.5375}{{\normalfont\ttfamily arXiv:1406.5375}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CMS:2015auz}
CMS collaboration, V.~Khachatryan {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the $t\bar{t}$ production cross section in the all-jets final state in pp collisions at $\sqrt{s}=8$ $\,\text {TeV}$}}, }{}\href{https://doi.org/10.1140/epjc/s10052-016-3956-5}{Eur.\ Phys.\ J.\  \textbf{C76} (2016) 128}, \href{http://arxiv.org/abs/1509.06076}{{\normalfont\ttfamily arXiv:1509.06076}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ATLAS:2016qhd}
ATLAS collaboration, M.~Aaboud {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the inclusive cross-sections of single top-quark and top-antiquark $t$-channel production in $pp$ collisions at $\sqrt{s}$ = 13 TeV with the ATLAS detector}}, }{}\href{https://doi.org/10.1007/JHEP04(2017)086}{JHEP \textbf{04} (2017) 086}, \href{http://arxiv.org/abs/1609.03920}{{\normalfont\ttfamily arXiv:1609.03920}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CMS:2016yys}
CMS collaboration, V.~Khachatryan {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the $\ttbar$ production cross section in the $e\mu$ channel in proton-proton collisions at $\sqrt{s} =$ 7 and 8 TeV}}, }{}\href{https://doi.org/10.1007/JHEP08(2016)029}{JHEP \textbf{08} (2016) 029}, \href{http://arxiv.org/abs/1603.02303}{{\normalfont\ttfamily arXiv:1603.02303}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CMS:2016csa}
CMS collaboration, V.~Khachatryan {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurements of the $t\bar{t}$ production cross section in lepton+jets final states in pp collisions at 8 $\,\text {TeV}$ and ratio of 8 to 7 $\,\text {TeV}$ cross sections}}, }{}\href{https://doi.org/10.1140/epjc/s10052-016-4504-z}{Eur.\ Phys.\ J.\  \textbf{C77} (2017) 15}, \href{http://arxiv.org/abs/1602.09024}{{\normalfont\ttfamily arXiv:1602.09024}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ATLAS:2017jkf}
ATLAS collaboration, M.~Aaboud {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the $t\bar{t}$ production cross section in the $\tau$ + jets final state in $pp$ collisions at $\sqrt{s}=8$ TeV using the ATLAS detector}}, }{}\href{https://doi.org/10.1103/PhysRevD.95.072003}{Phys.\ Rev.\  \textbf{D95} (2017) 072003}, \href{http://arxiv.org/abs/1702.08839}{{\normalfont\ttfamily arXiv:1702.08839}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ATLAS:2017wvi}
ATLAS collaboration, M.~Aaboud {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the inclusive and fiducial $t\bar{t}$ production cross-sections in the lepton+jets channel in $pp$ collisions at $\sqrt{s} = 8$ TeV with the ATLAS detector}}, }{}\href{https://doi.org/10.1140/epjc/s10052-018-5904-z}{Eur.\ Phys.\ J.\  \textbf{C78} (2018) 487}, \href{http://arxiv.org/abs/1712.06857}{{\normalfont\ttfamily arXiv:1712.06857}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ATLAS:2017rso}
ATLAS collaboration, M.~Aaboud {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Fiducial, total and differential cross-section measurements of $t$-channel single top-quark production in $pp$ collisions at 8 TeV using data collected by the ATLAS detector}}, }{}\href{https://doi.org/10.1140/epjc/s10052-017-5061-9}{Eur.\ Phys.\ J.\  \textbf{C77} (2017) 531}, \href{http://arxiv.org/abs/1702.02859}{{\normalfont\ttfamily arXiv:1702.02859}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CMS:2018fks}
CMS collaboration, A.~M. Sirunyan {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the $t\bar{t}$ production cross section, the top quark mass, and the strong coupling constant using dilepton events in pp collisions at $\sqrt{s} =$ 13 TeV}}, }{}\href{https://doi.org/10.1140/epjc/s10052-019-6863-8}{Eur.\ Phys.\ J.\  \textbf{C79} (2019) 368}, \href{http://arxiv.org/abs/1812.10505}{{\normalfont\ttfamily arXiv:1812.10505}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CMS:2018lgn}
CMS collaboration, A.~M. Sirunyan {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the single top quark and antiquark production cross sections in the $t$ channel and their ratio in proton-proton collisions at $\sqrt{s}=$ 13 TeV}}, }{}\href{https://doi.org/10.1016/j.physletb.2019.135042}{Phys.\ Lett.\  \textbf{B800} (2020) 135042}, \href{http://arxiv.org/abs/1812.10514}{{\normalfont\ttfamily arXiv:1812.10514}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CMS:2019snc}
CMS collaboration, A.~M. Sirunyan {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the top quark pair production cross section in dilepton final states containing one $\tau$ lepton in pp collisions at $\sqrt{s}=$ 13 TeV}}, }{}\href{https://doi.org/10.1007/JHEP02(2020)191}{JHEP \textbf{02} (2020) 191}, \href{http://arxiv.org/abs/1911.13204}{{\normalfont\ttfamily arXiv:1911.13204}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ATLAS:2020ccu}
ATLAS collaboration, G.~Aad {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurements of top-quark pair single- and double-differential cross-sections in the all-hadronic channel in $pp$ collisions at $\sqrt{s}=13~\textrm{TeV}$ using the ATLAS detector}}, }{}\href{https://doi.org/10.1007/JHEP01(2021)033}{JHEP \textbf{01} (2021) 033}, \href{http://arxiv.org/abs/2006.09274}{{\normalfont\ttfamily arXiv:2006.09274}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CMS:2021gwv}
CMS collaboration, A.~Tumasyan {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the inclusive $t\bar{t}$ production cross section in proton-proton collisions at $ \sqrt{s} $ = 5.02 TeV}}, }{}\href{https://doi.org/10.1007/JHEP04(2022)144}{JHEP \textbf{04} (2022) 144}, \href{http://arxiv.org/abs/2112.09114}{{\normalfont\ttfamily arXiv:2112.09114}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CMS:2021vhb}
CMS collaboration, A.~Tumasyan {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of differential $t\bar{t}$ production cross sections in the full kinematic range using lepton+jets events from proton-proton collisions at $\sqrt {s}$ = 13\,\,TeV}}, }{}\href{https://doi.org/10.1103/PhysRevD.104.092013}{Phys.\ Rev.\  \textbf{D104} (2021) 092013}, \href{http://arxiv.org/abs/2108.02803}{{\normalfont\ttfamily arXiv:2108.02803}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ATLAS:2022aof}
ATLAS, CMS collaborations, G.~Aad {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Combination of inclusive top-quark pair production cross-section measurements using ATLAS and CMS data at $ \sqrt{s} $ = 7 and 8 TeV}}, }{}\href{https://doi.org/10.1007/JHEP07(2023)213}{JHEP \textbf{07} (2023) 213}, \href{http://arxiv.org/abs/2205.13830}{{\normalfont\ttfamily arXiv:2205.13830}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ATLAS:2022jbj}
ATLAS collaboration, G.~Aad {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the $ t\overline{t} $ production cross-section in pp collisions at $ \sqrt{s} $ = 5.02 TeV with the ATLAS detector}}, }{}\href{https://doi.org/10.1007/JHEP06(2023)138}{JHEP \textbf{06} (2023) 138}, \href{http://arxiv.org/abs/2207.01354}{{\normalfont\ttfamily arXiv:2207.01354}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ATLAS:2022opp}
ATLAS collaboration, M.~Aaboud {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the inclusive $t\bar{t}$ production cross section in the lepton+jets channel in pp collisions at $\sqrt{s} =$7{\,}{\,}TeV with the ATLAS detector using support vector machines}}, }{}\href{https://doi.org/10.1103/PhysRevD.108.032014}{Phys.\ Rev.\  \textbf{D108} (2023) 032014}, \href{http://arxiv.org/abs/2212.00571}{{\normalfont\ttfamily arXiv:2212.00571}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ATLAS:2023gsl}
ATLAS collaboration, G.~Aad {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Inclusive and differential cross-sections for dilepton $ t\overline{t} $ production measured in $ \sqrt{s} $ = 13 TeV pp collisions with the ATLAS detector}}, }{}\href{https://doi.org/10.1007/JHEP07(2023)141}{JHEP \textbf{07} (2023) 141}, \href{http://arxiv.org/abs/2303.15340}{{\normalfont\ttfamily arXiv:2303.15340}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ATLAS:2023slx}
ATLAS collaboration, G.~Aad {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the $t\bar{t}$ cross section and its ratio to the $Z$ production cross section using $pp$ collisions at $\sqrt{s} =$13.6 TeV with the ATLAS detector}}, }{}\href{https://doi.org/10.1016/j.physletb.2023.138376}{Phys.\ Lett.\  \textbf{B848} (2024) 138376}, \href{http://arxiv.org/abs/2308.09529}{{\normalfont\ttfamily arXiv:2308.09529}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CMS:2023qyl}
CMS collaboration, A.~Tumasyan {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{First measurement of the top quark pair production cross section in proton-proton collisions at $ \sqrt{s} $ = 13.6 TeV}}, }{}\href{https://doi.org/10.1007/JHEP08(2023)204}{JHEP \textbf{08} (2023) 204}, \href{http://arxiv.org/abs/2303.10680}{{\normalfont\ttfamily arXiv:2303.10680}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CMS:2024ghc}
CMS collaboration, A.~Hayrapetyan {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the inclusive $t\bar{t}$ cross section in final states with at least one lepton and additional jets with 302 pb$^{-1}$ of pp collisions at $\sqrt{s}$ = 5.02 TeV}}, }{}\href{https://doi.org/10.1007/JHEP04(2025)099}{JHEP \textbf{04} (2025) 099}, \href{http://arxiv.org/abs/2410.21631}{{\normalfont\ttfamily arXiv:2410.21631}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2015-022}
LHCb collaboration, R.~Aaij {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{First observation of top quark production in the forward region}}, }{}\href{https://doi.org/10.1103/PhysRevLett.115.112001}{Phys.\ Rev.\ Lett.\  \textbf{115} (2015) 112001}, \href{http://arxiv.org/abs/1506.00903}{{\normalfont\ttfamily arXiv:1506.00903}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2016-038}
LHCb collaboration, R.~Aaij {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of forward $\ttbar$, $W + \bbbar$ and $W + \ccbar$ production in \proton\proton collisions at \mbox{$\sqs=$8~\tev}}}, }{}\href{https://doi.org/10.1016/j.physletb.2017.01.044}{Phys.\ Lett.\  \textbf{B767} (2017) 110}, \href{http://arxiv.org/abs/1610.08142}{{\normalfont\ttfamily arXiv:1610.08142}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2017-050}
LHCb collaboration, R.~Aaij {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of forward top pair production in the dilepton channel in \proton\proton collisions at $\sqs=13~\tev$}}, }{}\href{https://doi.org/10.1007/JHEP08(2018)174}{JHEP \textbf{08} (2018) 174}, \href{http://arxiv.org/abs/1803.05188}{{\normalfont\ttfamily arXiv:1803.05188}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CDF:2011xdt}
CDF collaboration, T.~Aaltonen {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Evidence for a mass dependent forward-backward asymmetry in top quark pair production}}, }{}\href{https://doi.org/10.1103/PhysRevD.83.112003}{Phys.\ Rev.\  \textbf{D83} (2011) 112003}, \href{http://arxiv.org/abs/1101.0034}{{\normalfont\ttfamily arXiv:1101.0034}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{D0:2015alu}
D0 collaboration, V.~M. Abazov {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Simultaneous measurement of forward-backward asymmetry and top polarization in dilepton final states from $t\bar t$ production at the Tevatron}}, }{}\href{https://doi.org/10.1103/PhysRevD.92.052007}{Phys.\ Rev.\  \textbf{D92} (2015) 052007}, \href{http://arxiv.org/abs/1507.05666}{{\normalfont\ttfamily arXiv:1507.05666}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CDF:2012ctl}
CDF collaboration, T.~Aaltonen {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the top quark forward-backward production asymmetry and its dependence on event kinematic properties}}, }{}\href{https://doi.org/10.1103/PhysRevD.87.092002}{Phys.\ Rev.\  \textbf{D87} (2013) 092002}, \href{http://arxiv.org/abs/1211.1003}{{\normalfont\ttfamily arXiv:1211.1003}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Czakon:2014xsa}
M.~Czakon, P.~Fiedler, and A.~Mitov, \ifthenelse{\boolean{articletitles}}{\emph{{Resolving the Tevatron top quark forward-backward asymmetry puzzle: fully differential next-to-next-to-leading-order calculation}}, }{}\href{https://doi.org/10.1103/PhysRevLett.115.052001}{Phys.\ Rev.\ Lett.\  \textbf{115} (2015) 052001}, \href{http://arxiv.org/abs/1411.3007}{{\normalfont\ttfamily arXiv:1411.3007}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{D0:2014cda}
D0 collaboration, V.~M. Abazov {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the forward-backward asymmetry in top quark-antiquark production in $p\bar{p}$ collisions using the lepton+jets channel}}, }{}\href{https://doi.org/10.1103/PhysRevD.90.072011}{Phys.\ Rev.\  \textbf{D90} (2014) 072011}, \href{http://arxiv.org/abs/1405.0421}{{\normalfont\ttfamily arXiv:1405.0421}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Kidonakis:2015ona}
N.~Kidonakis, \ifthenelse{\boolean{articletitles}}{\emph{{Top quark forward-backward asymmetry at approximate N$^3$LO}}, }{}\href{https://doi.org/10.1103/PhysRevD.91.071502}{Phys.\ Rev.\  \textbf{D91} (2015) 071502(R)}, \href{http://arxiv.org/abs/1501.01581}{{\normalfont\ttfamily arXiv:1501.01581}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CDF:2017cvy}
CDF, D0 collaborations, T.~A. Aaltonen {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Combined forward-backward asymmetry measurements in top-antitop quark production at the Tevatron}}, }{}\href{https://doi.org/10.1103/PhysRevLett.120.042001}{Phys.\ Rev.\ Lett.\  \textbf{120} (2018) 042001}, \href{http://arxiv.org/abs/1709.04894}{{\normalfont\ttfamily arXiv:1709.04894}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ATLAS:2013buu}
ATLAS collaboration, G.~Aad {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the top quark pair production charge asymmetry in proton-proton collisions at $\sqrt{s}$ = 7 TeV using the ATLAS detector}}, }{}\href{https://doi.org/10.1007/JHEP02(2014)107}{JHEP \textbf{02} (2014) 107}, \href{http://arxiv.org/abs/1311.6724}{{\normalfont\ttfamily arXiv:1311.6724}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ATLAS:2015ysm}
ATLAS collaboration, G.~Aad {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the charge asymmetry in dileptonic decays of top quark pairs in $pp$ collisions at $\sqrt{s}=7$ TeV using the ATLAS detector}}, }{}\href{https://doi.org/10.1007/JHEP05(2015)061}{JHEP \textbf{05} (2015) 061}, \href{http://arxiv.org/abs/1501.07383}{{\normalfont\ttfamily arXiv:1501.07383}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ATLAS:2015jgj}
ATLAS collaboration, G.~Aad {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the charge asymmetry in top-quark pair production in the lepton-plus-jets final state in pp collision data at $\sqrt{s}=8\,\mathrm TeV{}$ with the ATLAS detector}}, }{}\href{https://doi.org/10.1140/epjc/s10052-016-3910-6}{Eur.\ Phys.\ J.\  \textbf{C76} (2016) 87}, Erratum \href{https://doi.org/10.1140/epjc/s10052-017-5089-x}{ibid.\   \textbf{C77} (2017) 564}, \href{http://arxiv.org/abs/1509.02358}{{\normalfont\ttfamily arXiv:1509.02358}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ATLAS:2015sex}
ATLAS collaboration, G.~Aad {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the charge asymmetry in highly boosted top-quark pair production in $\sqrt{s} =$ 8 TeV $pp$ collision data collected by the ATLAS experiment}}, }{}\href{https://doi.org/10.1016/j.physletb.2016.02.055}{Phys.\ Lett.\  \textbf{B756} (2016) 52}, \href{http://arxiv.org/abs/1512.06092}{{\normalfont\ttfamily arXiv:1512.06092}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ATLAS:2022wec}
ATLAS collaboration, G.~Aad {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the charge asymmetry in top-quark pair production in association with a photon with the ATLAS experiment}}, }{}\href{https://doi.org/10.1016/j.physletb.2023.137848}{Phys.\ Lett.\  \textbf{B843} (2023) 137848}, \href{http://arxiv.org/abs/2212.10552}{{\normalfont\ttfamily arXiv:2212.10552}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ATLAS:2022waa}
ATLAS collaboration, G.~Aad {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Evidence for the charge asymmetry in pp {\textrightarrow} $ t\overline{t} $ production at $ \sqrt{s} $ = 13 TeV with the ATLAS detector}}, }{}\href{https://doi.org/10.1007/JHEP08(2023)077}{JHEP \textbf{08} (2023) 077}, \href{http://arxiv.org/abs/2208.12095}{{\normalfont\ttfamily arXiv:2208.12095}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CMS:2012oht}
CMS collaboration, S.~Chatrchyan {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Inclusive and differential measurements of the $t \bar{t}$ charge asymmetry in proton-proton collisions at $\sqrt{s} =$ 7 TeV}}, }{}\href{https://doi.org/10.1016/j.physletb.2012.09.028}{Phys.\ Lett.\  \textbf{B717} (2012) 129}, \href{http://arxiv.org/abs/1207.0065}{{\normalfont\ttfamily arXiv:1207.0065}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CMS:2014rdf}
CMS collaboration, S.~Chatrchyan {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurements of the $t\bar{t}$ charge asymmetry using the dilepton decay channel in pp collisions at $\sqrt{s} =$ 7 TeV}}, }{}\href{https://doi.org/10.1007/JHEP04(2014)191}{JHEP \textbf{04} (2014) 191}, \href{http://arxiv.org/abs/1402.3803}{{\normalfont\ttfamily arXiv:1402.3803}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CMS:2015fvy}
CMS collaboration, V.~Khachatryan {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the charge asymmetry in top quark pair production in pp collisions at $\sqrt{s} =$ 8 TeV using a template method}}, }{}\href{https://doi.org/10.1103/PhysRevD.93.034014}{Phys.\ Rev.\  \textbf{D93} (2016) 034014}, \href{http://arxiv.org/abs/1508.03862}{{\normalfont\ttfamily arXiv:1508.03862}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CMS:2015pob}
CMS collaboration, V.~Khachatryan {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Inclusive and differential measurements of the $t\bar{t}$ charge asymmetry in pp collisions at $\sqrt{s} =$ 8 TeV}}, }{}\href{https://doi.org/10.1016/j.physletb.2016.03.060}{Phys.\ Lett.\  \textbf{B757} (2016) 154}, \href{http://arxiv.org/abs/1507.03119}{{\normalfont\ttfamily arXiv:1507.03119}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{CMS:2016ypc}
CMS collaboration, V.~Khachatryan {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurements of $t \bar t$ charge asymmetry using dilepton final states in pp collisions at $\sqrt s=8$ TeV}}, }{}\href{https://doi.org/10.1016/j.physletb.2016.07.006}{Phys.\ Lett.\  \textbf{B760} (2016) 365}, \href{http://arxiv.org/abs/1603.06221}{{\normalfont\ttfamily arXiv:1603.06221}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{antiKt}
M.~Cacciari, G.~P. Salam, and G.~Soyez, \ifthenelse{\boolean{articletitles}}{\emph{{The anti-$k_t$ jet clustering algorithm}}, }{}\href{https://doi.org/10.1088/1126-6708/2008/04/063}{JHEP \textbf{04} (2008) 063}, \href{http://arxiv.org/abs/0802.1189}{{\normalfont\ttfamily arXiv:0802.1189}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2013-058}
LHCb collaboration, R.~Aaij {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Study of forward \Z+jet production in \proton\proton collisions at $\sqs = $7~\tev}}, }{}\href{https://doi.org/10.1007/JHEP01(2014)033}{JHEP \textbf{01} (2014) 033}, \href{http://arxiv.org/abs/1310.8197}{{\normalfont\ttfamily arXiv:1310.8197}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-DP-2008-001}
LHCb collaboration, A.~A. Alves~Jr.\ {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{The \lhcb detector at the LHC}}, }{}\href{https://doi.org/10.1088/1748-0221/3/08/S08005}{JINST \textbf{3} (2008) S08005}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-DP-2014-002}
LHCb collaboration, R.~Aaij {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{LHCb detector performance}}, }{}\href{https://doi.org/10.1142/S0217751X15300227}{Int.\ J.\ Mod.\ Phys.\  \textbf{A30} (2015) 1530022}, \href{http://arxiv.org/abs/1412.6352}{{\normalfont\ttfamily arXiv:1412.6352}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-DP-2014-001}
R.~Aaij {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Performance of the LHCb Vertex Locator}}, }{}\href{https://doi.org/10.1088/1748-0221/9/09/P09007}{JINST \textbf{9} (2014) P09007}, \href{http://arxiv.org/abs/1405.7808}{{\normalfont\ttfamily arXiv:1405.7808}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-DP-2017-001}
P.~d'Argent {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Improved performance of the LHCb Outer Tracker in LHC Run 2}}, }{}\href{https://doi.org/10.1088/1748-0221/12/11/P11016}{JINST \textbf{12} (2017) P11016}, \href{http://arxiv.org/abs/1708.00819}{{\normalfont\ttfamily arXiv:1708.00819}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-DP-2012-003}
M.~Adinolfi {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Performance of the \lhcb RICH detector at the LHC}}, }{}\href{https://doi.org/10.1140/epjc/s10052-013-2431-9}{Eur.\ Phys.\ J.\  \textbf{C73} (2013) 2431}, \href{http://arxiv.org/abs/1211.6759}{{\normalfont\ttfamily arXiv:1211.6759}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-DP-2012-002}
A.~A. Alves~Jr.\ {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Performance of the LHCb muon system}}, }{}\href{https://doi.org/10.1088/1748-0221/8/02/P02022}{JINST \textbf{8} (2013) P02022}, \href{http://arxiv.org/abs/1211.1346}{{\normalfont\ttfamily arXiv:1211.1346}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-DP-2012-004}
R.~Aaij {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{The \lhcb trigger and its performance in 2011}}, }{}\href{https://doi.org/10.1088/1748-0221/8/04/P04022}{JINST \textbf{8} (2013) P04022}, \href{http://arxiv.org/abs/1211.3055}{{\normalfont\ttfamily arXiv:1211.3055}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-DP-2019-001}
R.~Aaij {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Design and performance of the LHCb trigger and full real-time reconstruction in Run 2 of the LHC}}, }{}\href{https://doi.org/10.1088/1748-0221/14/04/P04013}{JINST \textbf{14} (2019) P04013}, \href{http://arxiv.org/abs/1812.10790}{{\normalfont\ttfamily arXiv:1812.10790}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Sjostrand:2007gs}
T.~Sj\"{o}strand, S.~Mrenna, and P.~Skands, \ifthenelse{\boolean{articletitles}}{\emph{{A brief introduction to PYTHIA 8.1}}, }{}\href{https://doi.org/10.1016/j.cpc.2008.01.036}{Comput.\ Phys.\ Commun.\  \textbf{178} (2008) 852}, \href{http://arxiv.org/abs/0710.3820}{{\normalfont\ttfamily arXiv:0710.3820}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Sjostrand:2006za}
T.~Sj\"{o}strand, S.~Mrenna, and P.~Skands, \ifthenelse{\boolean{articletitles}}{\emph{{PYTHIA 6.4 physics and manual}}, }{}\href{https://doi.org/10.1088/1126-6708/2006/05/026}{JHEP \textbf{05} (2006) 026}, \href{http://arxiv.org/abs/hep-ph/0603175}{{\normalfont\ttfamily arXiv:hep-ph/0603175}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PROC-2010-056}
I.~Belyaev {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Handling of the generation of primary events in Gauss, the LHCb simulation framework}}, }{}\href{https://doi.org/10.1088/1742-6596/331/3/032047}{J.\ Phys.\ Conf.\ Ser.\  \textbf{331} (2011) 032047}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{davidson2015photos}
N.~Davidson, T.~Przedzinski, and Z.~Was, \ifthenelse{\boolean{articletitles}}{\emph{{PHOTOS interface in C++: Technical and physics documentation}}, }{}\href{https://doi.org/https://doi.org/10.1016/j.cpc.2015.09.013}{Comp.\ Phys.\ Comm.\  \textbf{199} (2016) 86}, \href{http://arxiv.org/abs/1011.0937}{{\normalfont\ttfamily arXiv:1011.0937}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Allison:2006ve}
Geant4 collaboration, J.~Allison {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Geant4 developments and applications}}, }{}\href{https://doi.org/10.1109/TNS.2006.869826}{IEEE Trans.\ Nucl.\ Sci.\  \textbf{53} (2006) 270}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Agostinelli:2002hh}
Geant4 collaboration, S.~Agostinelli {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Geant4: A simulation toolkit}}, }{}\href{https://doi.org/10.1016/S0168-9002(03)01368-8}{Nucl.\ Instrum.\ Meth.\  \textbf{A506} (2003) 250}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PROC-2011-006}
M.~Clemencic {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{The \lhcb simulation application, Gauss: Design, evolution and experience}}, }{}\href{https://doi.org/10.1088/1742-6596/331/3/032023}{J.\ Phys.\ Conf.\ Ser.\  \textbf{331} (2011) 032023}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Nason:2004rx}
P.~Nason, \ifthenelse{\boolean{articletitles}}{\emph{{A new method for combining NLO QCD with shower Monte Carlo algorithms}}, }{}\href{https://doi.org/10.1088/1126-6708/2004/11/040}{JHEP \textbf{11} (2004) 040}, \href{http://arxiv.org/abs/hep-ph/0409146}{{\normalfont\ttfamily arXiv:hep-ph/0409146}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Frixione:2007vw}
S.~Frixione, P.~Nason, and C.~Oleari, \ifthenelse{\boolean{articletitles}}{\emph{{Matching NLO QCD computations with parton shower simulations: the POWHEG method}}, }{}\href{https://doi.org/10.1088/1126-6708/2007/11/070}{JHEP \textbf{11} (2007) 070}, \href{http://arxiv.org/abs/0709.2092}{{\normalfont\ttfamily arXiv:0709.2092}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Alioli:2010xd}
S.~Alioli, P.~Nason, C.~Oleari, and E.~Re, \ifthenelse{\boolean{articletitles}}{\emph{{A general framework for implementing NLO calculations in shower Monte Carlo programs: the POWHEG BOX}}, }{}\href{https://doi.org/10.1007/JHEP06(2010)043}{JHEP \textbf{06} (2010) 043}, \href{http://arxiv.org/abs/1002.2581}{{\normalfont\ttfamily arXiv:1002.2581}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Mg5}
J.~Alwall {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{The automated computation of tree-level and next-to-leading order differential cross sections, and their matching to parton shower simulations}}, }{}\href{https://doi.org/10.1007/JHEP07(2014)079}{JHEP \textbf{07} (2014) 079}, \href{http://arxiv.org/abs/1405.0301}{{\normalfont\ttfamily arXiv:1405.0301}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2016-011}
LHCb collaboration, R.~Aaij {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of forward $\W$ and $\Z$ boson production in association with jets in proton-proton collisions at \mbox{$\sqs=$8~\tev}}}, }{}\href{https://doi.org/10.1007/JHEP05(2016)131}{JHEP \textbf{05} (2016) 131}, \href{http://arxiv.org/abs/1605.00951}{{\normalfont\ttfamily arXiv:1605.00951}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{deepjet}
E.~Bols {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Jet flavour classification using DeepJet}}, }{}\href{https://doi.org/10.1088/1748-0221/15/12/P12012}{JINST \textbf{15} (2020) P12012}, \href{http://arxiv.org/abs/2008.10519}{{\normalfont\ttfamily arXiv:2008.10519}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2025-034}
LHCb collaboration, R.~Aaij {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Search for $H \to b \Bar{b}$ and $H \to c \Bar{c}$ in $\sqrt{s}=13$ TeV $pp$ collisions at LHCb using machine learning techniques}}, }{} {LHCb-PAPER-2025-034}, {in preparation, to be submitted to JHEP}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{ABCD_ATLAS}
ATLAS collaboration, G.~Aad {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the inclusive isolated prompt photon cross section in $pp$ collisions at $\sqrt{s}=7$ TeV with the ATLAS detector}}, }{}\href{https://doi.org/10.1103/PhysRevD.83.052005}{Phys.\ Rev.\  \textbf{D83} (2011) 052005}, \href{http://arxiv.org/abs/1012.4389}{{\normalfont\ttfamily arXiv:1012.4389}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCB-PAPER-2021-037}
LHCb collaboration, R.~Aaij {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Precision measurement of forward \Z boson production in proton-proton collisions at $\sqrt{s} = 13$~\tev}}, }{}\href{https://doi.org/10.1007/JHEP07(2022)026}{JHEP \textbf{07} (2022) 026}, \href{http://arxiv.org/abs/2112.07458}{{\normalfont\ttfamily arXiv:2112.07458}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCB-PAPER-2014-033}
LHCb collaboration, R.~Aaij {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the forward \W boson production cross-section in \proton\proton collisions at \mbox{$\sqs=$7~\tev}}}, }{}\href{https://doi.org/10.1007/JHEP12(2014)079}{JHEP \textbf{12} (2014) 079}, \href{http://arxiv.org/abs/1408.4354}{{\normalfont\ttfamily arXiv:1408.4354}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCB-PAPER-2015-001}
LHCb collaboration, R.~Aaij {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of the forward \Z boson cross-section in \proton\proton collisions at \mbox{$\sqs=$7~\tev}}}, }{}\href{https://doi.org/10.1007/JHEP08(2015)039}{JHEP \textbf{08} (2015) 039}, \href{http://arxiv.org/abs/1505.07024}{{\normalfont\ttfamily arXiv:1505.07024}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCB-PAPER-2015-049}
LHCb collaboration, R.~Aaij {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of forward \W and \Z boson production in \proton\proton collisions at \mbox{$\sqs=$8~\tev}}}, }{}\href{https://doi.org/10.1007/JHEP01(2016)155}{JHEP \textbf{01} (2016) 155}, \href{http://arxiv.org/abs/1511.08039}{{\normalfont\ttfamily arXiv:1511.08039}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-018}
LHCb collaboration, R.~Aaij {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Measurement of differential $\bquark \bquarkbar$ and $\cquark \cquarkbar$ dijet cross-sections in the forward region of $pp$ collisions at $\sqrt{s} = 13$~\tev}}, }{}\href{https://doi.org/10.1007/JHEP02(2021)023}{JHEP \textbf{02} (2021) 023}, \href{http://arxiv.org/abs/2010.09437}{{\normalfont\ttfamily arXiv:2010.09437}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2015-021}
LHCb collaboration, R.~Aaij {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Study of \W boson production in association with beauty and charm}}, }{}\href{https://doi.org/10.1103/PhysRevD.92.052001}{Phys.\ Rev.\  \textbf{D92} (2015) 052012}, \href{http://arxiv.org/abs/1505.04051}{{\normalfont\ttfamily arXiv:1505.04051}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{theoryerr}
LHC Higgs Cross Section Working Group, S.~Dittmaier {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Handbook of LHC Higgs cross sections: 1. inclusive observables}}, }{}doi:~\href{https://doi.org/10.5170/CERN-2011-002}{10.5170/CERN-2011-002} \href{http://arxiv.org/abs/1101.0593}{{\normalfont\ttfamily arXiv:1101.0593}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{lumi}
LHCb collaboration, R.~Aaij {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Precision luminosity measurements at LHCb}}, }{}\href{https://doi.org/10.1088/1748-0221/9/12/P12005}{JINST \textbf{9} (2014) P12005}, \href{http://arxiv.org/abs/1410.0149}{{\normalfont\ttfamily arXiv:1410.0149}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{POWHEG}
T.~Je\v{z}o and P.~Nason, \ifthenelse{\boolean{articletitles}}{\emph{{On the treatment of resonances in next-to-leading order calculations matched to a parton shower}}, }{}\href{https://doi.org/10.1007/JHEP12(2015)065}{JHEP \textbf{12} (2015) 065}, \href{http://arxiv.org/abs/1509.09071}{{\normalfont\ttfamily arXiv:1509.09071}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Hou:2019efy}
T.-J. Hou {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{New CTEQ global analysis of quantum chromodynamics with high-precision data from the LHC}}, }{}\href{https://doi.org/10.1103/PhysRevD.103.014013}{Phys.\ Rev.\  \textbf{D103} (2021) 014013}, \href{http://arxiv.org/abs/1912.10053}{{\normalfont\ttfamily arXiv:1912.10053}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ball2017}
NNPDF collaboration, R.~D. Ball {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Parton distributions from high-precision collider data}}, }{}\href{https://doi.org/10.1140/epjc/s10052-017-5199-5}{Eur.\ Phys.\ J.\  \textbf{C77} (2017) 663}, \href{http://arxiv.org/abs/1706.00428}{{\normalfont\ttfamily arXiv:1706.00428}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{bourilkov2006}
D.~Bourilkov, R.~C. Group, and M.~R. Whalley, \ifthenelse{\boolean{articletitles}}{\emph{{LHAPDF: PDF use from the Tevatron to the LHC}}, }{} in {\em {TeV4LHC Workshop - 4th meeting}}, 2006, \href{http://arxiv.org/abs/hep-ph/0605240}{{\normalfont\ttfamily arXiv:hep-ph/0605240}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{james_paper}
J.~V. Mead, \ifthenelse{\boolean{articletitles}}{\emph{{A measurement of top quark production at $ \sqrt{s} $ = 13 TeV with LHCb data}}, }{} 2021.
\newblock \href{https://cds.cern.ch/record/2780780} {CERN-THESIS-2021-130}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\end{mcitethebibliography}


==> section/prl_justification.tex <==
\clearpage
\centerline{\large\normalfont\bfseries PRL Justification}

We present the first measurement of the top-quark charge asymmetry and differential production cross-sections in the forward region in proton-proton collisions at \mbox{$\sqrt{s}=13$ TeV}, using 5.4 fb$^{-1}$ of data collected by the LHCb experiment. This probes a unique phase space dominated by valence-sea-quark interactions, where sensitivity to QCD effects and potential Beyond the Standard Model contributions are enhanced.

The asymmetry observable, previously studied only at central rapidities, is measured here with unprecedented precision in the forward region, offering complementary information to existing ATLAS and CMS results. Alongside this, we present the most precise measurements to date of forward \tquark and \tquarkbar cross-sections, both inclusively and differentially in muon pseudorapidity intervals.

The analysis employs robust data-driven techniques, with systematic uncertainties carefully evaluated, and results are compared to NLO predictions with modern PDFs. These measurements provide important inputs for SM tests and global fits, and will be of broad interest to the high-energy physics community.

\section*{Word count}

\begin{itemize}
  \item Text: 3223
  \item Figures: $(20 + 150/1.688) + (20 + 150/1.333) $ $\;\Rightarrow\;$ 242
  \item Maths: four single-column equations: $5 \times 16 = 80$
  \item Tables: $(13 + 6.5 \times 12) + (13 + 6.5 \times 4) + (13 + 6.5 \times 5) = 175.5$
\end{itemize}

\noindent
Total: $3223 + 80 + 175.5 + 109 + 133 \approx 3721$ words


\clearpage

==> title-LHCb-PAPER.tex <==
% ===============================================================================
% Purpose: LHCb-PAPER journal paper title page template
% Author: 
% Created on: 2010-09-25
% ===============================================================================

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  TITLE PAGE  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{titlepage}
\pagenumbering{roman}

% Header ---------------------------------------------------
\vspace*{-1.5cm}
\centerline{\large EUROPEAN ORGANIZATION FOR NUCLEAR RESEARCH (CERN)}
\vspace*{1.5cm}
\noindent
\begin{tabular*}{\linewidth}{lc@{\extracolsep{\fill}}r@{\extracolsep{0pt}}}
\ifthenelse{\boolean{pdflatex}}% Logo format choice
{\vspace*{-1.5cm}\mbox{\!\!\!\includegraphics[width=.14\textwidth]{figs/lhcb-logo.pdf}} & &}%
{\vspace*{-1.2cm}\mbox{\!\!\!\includegraphics[width=.12\textwidth]{figs/lhcb-logo.eps}} & &}%
\\
 & & CERN-EP-2025-274 \\  % ID 
 & & LHCb-PAPER-2025-057 \\  % ID 
 & & April 21, 2026  \\ % Date - Can also hardwire e.g.: 23 March 2010
 & & \\
% not in paper \hline
\end{tabular*}

\vspace*{1.50cm}

% Title --------------------------------------------------
{\normalfont\bfseries\boldmath\huge
\begin{center}
% DO NOT EDIT HERE. Instead edit macro in main.tex to keep metadata correct
\papertitle
\end{center}
}
\vspace*{1.5cm}
% Authors -------------------------------------------------
\begin{center}
%In the footnote, replace 'paper' by 'Letter' in case of submission to PRL or PLB 
% Edit macro in main.tex to keep metadata correct
\paperauthors\footnote{Authors are listed at the end of this paper.}
\end{center}

\vspace{\fill}

% Abstract -----------------------------------------------
\begin{abstract}
  \noindent
The first measurements of the top- and antitop-quark differential production cross-sections and the top-quark charge asymmetry in the forward region are presented, using proton-proton collision data collected by the \lhcb experiment at a center-of-mass energy of 13\tev corresponding to an integrated luminosity of 5.4\invfb. The total production cross-sections of top and antitop quarks are also determined. 
Measurements are performed using the $\mu+\bjet$ final state within a fiducial region defined by \bjet $\jetpt>50\gev$ and pseudorapidity $2.2<\jeteta<4.0$, with the muon from the \W-boson decay required to have $\mupt>25\gev$ and $2.0<\mueta<4.5$. The muon and \bjet system must satisfy $\pt(\mu+\jet) > 20\gev$.
The measured integrated production cross-sections for the top and antitop quarks are
\begin{equation*}
\begin{split}
 \sigma_{\tquark} = \xs \pm \xsstat \pm \xssyst  \pm \xslumi \   \pb, \\
 \sigma_{\tquarkbar} = \tbarxs \pm \tbarxsstat  \pm \tbarxssyst  \pm \tbarxslumi \   \pb,
 \end{split}
\end{equation*}
 where the first uncertainty is statistical, the second systematic, and the third accounts for the luminosity uncertainty. The top-quark charge asymmetry is measured to be
\begin{equation*}
 \asy = \ay \pm \aystat  \pm \aysyst ,
\end{equation*}
 where the first uncertainty is statistical and the second is systematic. 
These results are consistent with next-to-leading order Standard Model predictions.
\end{abstract}
\vspace*{1.0cm}
\begin{center}
  Submitted to
  % JHEP /
  % Phys.~Rev.~D /
  Phys.~Rev.~Lett.
%  Phys.~Lett.~B /
  % Eur.~Phys.~J.~C /
  % %  Nucl.~Phys.~B /
  % Chin.~Phys.~C /
  % Nature~Physics /
  % sciPost~Physics /
  % J. Instr. /
  % Instruments 
\end{center}

\vspace{\fill}

{\footnotesize 
% Edit macro in main.tex to keep metadata correct
\centerline{\copyright~\papercopyright. \href{\paperlicenceurl}{\paperlicence}.}}
\vspace*{2mm}

\end{titlepage}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  EOD OF TITLE PAGE  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  empty page follows the title page ----
\newpage
\setcounter{page}{2}
\mbox{~}
%\newpage
%
%% Author List ----------------------------
%%  You need to get a new author list!
%\input{LHCb_authorlist.tex}
%
%The author list for journal publications is provided by the Membership Committee shortly after 'approval to go to paper' has been given.
%%It will be made available on the page
%%\verb!http://www.physik.uzh.ch/~strauman/forMemCo/LHCb-PAPER-XXXX-XXX/! .
%It will be sent to you by email shortly after a paper number has beens assigned.
%The author list should be included already at first circulation, 
%to allow new members of the collaboration to verify whether they have been included correctly.
%Occasionally a misspelled name is corrected or associated institutions become full members.
%In that case, a new author list will be sent to you.
%In case line numbering doesn't work well after including the authorlist, try moving the \verb!\bigskip! after the last author to a separate line.
%
%
%The authorship for Conference Reports should be ``The LHCb
%  collaboration'', with a footnote giving the name(s) of the contact
%  author(s), but without the full list of collaboration names.












